Reuse Detector: Improving the Management of STT-RAM SLLCs

Various constraints of Static Random Access Memory (SRAM) are leading to consider new memory technologies as candidates for building on-chip shared last-level caches (SLLCs). Spin-Transfer Torque RAM (STT-RAM) is currently postulated as the prime contender due to its better energy efficiency, smaller die footprint and higher scalability. However, STT-RAM also exhibits some drawbacks, like slow and energy-hungry write operations, that need to be mitigated. In this work we address these shortcomings by leveraging a new management mechanism for STT-RAM SLLCs. This approach is based on the previous observation that the stream of references arriving at the SLLC of a Chip MultiProcessor (CMP) exhibits reuse locality, i.e., those blocks referenced several times manifest high probability of forthcoming reuse. In this paper, we employ a cache management mechanism that selects the contents of the SLLC aimed to exploit reuse locality instead of temporal locality. Specifically, our proposal consists in the inclusion of a Reuse Detector between private cache levels and the STT-RAM SLLC to detect blocks that do not exhibit reuse, in order to avoid their insertion in the SLLC, hence reducing the number of write operations and the energy consumption in the STT-RAM. Our evaluation reveals that our scheme reports on average, energy reductions in the SLLC in the range of 37-30\%, additional energy savings in the main memory in the range of 6-8\% and performance improvements of 3\% up to 14\% (16-core) compared to an STT-RAM SLLC baseline where no reuse detector is employed. More importantly, our approach outperforms DASCA, the state-of-the-art STT-RAM SLLC management, reporting SLLC energy savings in the range of 4-11\% higher than those of DASCA, delivering higher performance in the range of 1.5-14\%, and additional improvements in DRAM energy consumption in the range of 2-9\% higher than DASCA.

==> Makefile <==
DOCS = compJournal
ALLTEXFILES = $(wildcard *.tex)
TEXFILES = $(patsubst %,%.tex,$(DOCS))
DVIFILES = $(patsubst %,%.dvi,$(DOCS))
PSFILES = $(patsubst %,%.ps,$(DOCS))
PDFFILES = $(patsubst %,%.pdf,$(DOCS))
TEXCODE = 
#$(patsubst code/%.c, code/%.tex, $(wildcard code/*.c))

#all: $(TEXCODE) $(DVIFILES) $(PSFILES) $(PDFFILES)
all: $(DVIFILES) $(PSFILES) $(PDFFILES)

%.dvi: $(ALLTEXFILES)
	latex $*
	bibtex $*
	latex $*
	latex $*

%.ps: %.dvi
	dvips -t a4 -X 1200 -Y 1200 $< -o $@

%.pdf: %.ps
#	lpr -P APDF $<
#	sleep 5
#	mv $(HOME)/PDF/$@ .
	ps2pdf -sPAPERSIZE=a4 -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 -dSubsetFonts=true -dEmbedAllFonts=true $<

wc: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  wc $$tex; \
	done;

spellcheck: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  ispell -t -d american $$tex; \
	done;	

clean:
	@rm -f *.out *.bbl *.blg *.dvi *~ *.ps *.aux *.log *.pdf code/*.tex code/*~ *.bak




==> Makefile_eps <==
DOCS = compJournal
ALLTEXFILES = $(wildcard *.tex)
TEXFILES = $(patsubst %,%.tex,$(DOCS))
DVIFILES = $(patsubst %,%.dvi,$(DOCS))
PSFILES = $(patsubst %,%.ps,$(DOCS))
PDFFILES = $(patsubst %,%.pdf,$(DOCS))
TEXCODE = 
#$(patsubst code/%.c, code/%.tex, $(wildcard code/*.c))

#all: $(TEXCODE) $(DVIFILES) $(PSFILES) $(PDFFILES)
all: $(DVIFILES) $(PSFILES) $(PDFFILES)

%.dvi: $(ALLTEXFILES)
	latex $*
	bibtex $*
	latex $*
	latex $*

%.ps: %.dvi
	dvips -t a4 -X 1200 -Y 1200 $< -o $@

%.pdf: %.ps
#	lpr -P APDF $<
#	sleep 5
#	mv $(HOME)/PDF/$@ .
	ps2pdf -sPAPERSIZE=a4 -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 -dSubsetFonts=true -dEmbedAllFonts=true $<

wc: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  wc $$tex; \
	done;

spellcheck: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  ispell -t -d american $$tex; \
	done;	

clean:
	@rm -f *.out *.bbl *.blg *.dvi *~ *.ps *.aux *.log *.pdf code/*.tex code/*~ *.bak




==> Makefile_old <==
DOCS = acmsmall-sample
IEEE = bare_conf
CJ = compJournal.tex
ELSEVIER = ecrc-template.tex
ALLTEXFILES = $(wildcard *.tex)
TEXFILES = $(patsubst %,%.tex,$(DOCS))
PDFFILES = $(patsubst %,%.pdf,$(DOCS))
PDFFILESIEEE = $(patsubst %,%.pdf,$(IEEE))
PDFFILESCJ = $(patsubst %,%.pdf,$(CJ))
PDFFILESELSEVIER = $(patsubst %,%.pdf,$(ELSEVIER))

TEXCODE = 
#$(patsubst code/%.c, code/%.tex, $(wildcard code/*.c))

#all: $(TEXCODE) $(DVIFILES) $(PSFILES) $(PDFFILES)
all: $(PDFFILESCJ)

elsevier: $(PDFFILESELSEVIER)
taco: $(PDFFILES)
ieee: $(PDFFILESIEEE)

%.pdf: $(ALLTEXFILES)
#	lualatex $*
	latexmk -pdf -dvi- -ps- -f $*
#	pdflatex $*
#	bibtex  $*
#	pdflatex  $*
#	pdflatex  $*

#%.ps: %.dvi
#	dvips  -X 1200 -Y 1200 $< -o $@

#%.pdf: %.ps
#	lpr -P APDF $<
#	sleep 5
#	mv $(HOME)/PDF/$@ .
#	ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.2 -dSubsetFonts=true -dEmbedAllFonts=true $<

wc: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  wc $$tex; \
	done;

spellcheck: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  ispell -t -d american $$tex; \
	done;	

clean:
	@rm -f $(PDFFILES) *.out *.bbl *.blg *.dvi *~ *.ps *.aux *.log  code/*.tex code/*~ *.bak *.fdb_latexmk *.fls *.lof *.pdf *.toc *.lot *.ilg *.idx */*.pdf 


==> Makefile_pdf <==
DOCS = compJournal
ALLTEXFILES = $(wildcard *.tex)
TEXFILES = $(patsubst %,%.tex,$(DOCS))
PDFFILES = $(patsubst %,%.pdf,$(DOCS))
TEXCODE = 
#$(patsubst code/%.c, code/%.tex, $(wildcard code/*.c))

#all: $(TEXCODE) $(DVIFILES) $(PSFILES) $(PDFFILES)
all: $(PDFFILES)

%.pdf: $(ALLTEXFILES)
	pdflatex $*
	bibtex  $*
	pdflatex  $*
	pdflatex  $*

#%.ps: %.dvi
#	dvips  -X 1200 -Y 1200 $< -o $@

#%.pdf: %.ps
#	lpr -P APDF $<
#	sleep 5
#	mv $(HOME)/PDF/$@ .
#	ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.2 -dSubsetFonts=true -dEmbedAllFonts=true $<

wc: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  wc $$tex; \
	done;

spellcheck: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  ispell -t -d american $$tex; \
	done;	

clean:
	@rm -f $(PDFFILES) *.out *.bbl *.blg *.dvi *~ *.ps *.aux *.log  code/*.tex code/*~ *.bak


==> evaluation_con_pgfplots.tex <==
\section{Evaluation}
\label{sec:eval}

This section compares how well RD and DASCA behave when managing an STT-RAM LLC, both in terms of performance and energy consumption of LLC and main memory. Single, four and eight-core systems are discussed in Sections~\ref{subsec:sc},~\ref{subsec:mc}, and~\ref{subsec:8_mc}, respectively. Finally, in Section~\ref{subsec:putting}, we show the results derived from the evaluation in a 16-core CMP and we analyze the performance of both approaches as the number of cores augments.

\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0,
				ymax=1.01,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.89,0.98)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={perlbench,bzip2,gcc,bwaves,mcf,milc,zeusmp,gromacs,cactusADM,leslie3d,namd,gobmk,soplex,calculix,hmmer,GemsFDTD,libquantum,h264ref,tonto,lbm,omnetpp,astar,wrf,sphinx3,xalancbmk,GMEAN,HIGH}, 
				symbolic x coords={perlbench,bzip2,gcc,bwaves,mcf,milc,zeusmp,gromacs,cactusADM,leslie3d,namd,gobmk,soplex,calculix,hmmer,GemsFDTD,libquantum,h264ref,tonto,lbm,omnetpp,astar,wrf,sphinx3,xalancbmk,AVG,HIGH}, 
				xtick=data, 
 			    x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				%\addplot [LineFillYellowTiny]coordinates {(perlbench,0.22) (bzip2,0.44) (gcc,0.65) (bwaves,0.01) (mcf,0.43) (milc,0.64) (zeusmp,0.17) (gromacs,0.74) (cactusADM,0.09) (leslie3d,0.15) (namd,0.28) (gobmk,0.21) (soplex,0.65) (calculix,0.40) (hmmer,0.86) (GemsFDTD,1.00) (libquantum,1.00) (h264ref,0.86) (tonto,0.92) (lbm,0.23) (omnetpp,1.00) (astar,0.38) (wrf,0.10) (sphinx3,0.14) (xalancbmk,0.47) (GMEAN,0.344)(HIGH,0.19465)};
				\addplot [LineFillYellowTiny]coordinates {(perlbench,0.22) (bzip2,0.44) (gcc,0.65) (bwaves,0.01) (mcf,0.43) (milc,0.64) (zeusmp,0.17) (gromacs,0.74) (cactusADM,0.09) (leslie3d,0.15) (namd,0.28) (gobmk,0.21) (soplex,0.65) (calculix,0.40) (hmmer,0.86) (GemsFDTD,1.00) (libquantum,1.00) (h264ref,0.86) (tonto,0.92) (lbm,0.23) (omnetpp,1.00) (astar,0.38) (wrf,0.10) (sphinx3,0.14) (xalancbmk,0.47) (AVG,0.482)(HIGH,0.3405)};
			%\addplot [LineFillBlueTiny]coordinates {(perlbench,0.15) (bzip2,0.54) (gcc,0.37) (bwaves,0.00) (mcf,0.32) (milc,0.02) (zeusmp,0.09) (gromacs,0.60) (cactusADM,0.15) (leslie3d,0.05) (namd,0.01) (gobmk,0.15) (soplex,0.62) (calculix,0.45) (hmmer,0.97) (GemsFDTD,0.22) (libquantum,1.00) (h264ref,0.73) (tonto,0.78) (lbm,0.00) (omnetpp,0.60) (astar,0.43) (wrf,0.07) (sphinx3,0.01) (xalancbmk,0.40) (GMEAN,0.105)(HIGH,0.01781)};
			\addplot [LineFillBlueTiny]coordinates {(perlbench,0.15) (bzip2,0.54) (gcc,0.37) (bwaves,0.00) (mcf,0.32) (milc,0.02) (zeusmp,0.09) (gromacs,0.60) (cactusADM,0.15) (leslie3d,0.05) (namd,0.01) (gobmk,0.15) (soplex,0.62) (calculix,0.45) (hmmer,0.97) (GemsFDTD,0.22) (libquantum,1.00) (h264ref,0.73) (tonto,0.78) (lbm,0.00) (omnetpp,0.60) (astar,0.43) (wrf,0.07) (sphinx3,0.01) (xalancbmk,0.40) (AVG,0.348)(HIGH,0.2041)};
%\addplot [LineFillRedTiny]coordinates {(400.perlbench,) (401.bzip2,) (403.gcc,) (410.bwaves,) (429.mcf,) (433.milc,) (434.zeusmp,) (435.gromacs,) (436.cactusADM,) (437.leslie3d,) (444.namd,) (445.gobmk,) (450.soplex,) (454.calculix,) (456.hmmer,) (459.GemsFDTD,) (462.libquantum,) (464.h264ref,) (465.tonto,) (470.lbm,) (471.omnetpp,) (473.astar,) (481.wrf,) (482.sphinx3,) (483.xalancbmk,) (GMEAN,)(HIGH,)};
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Number of writes to the STT-RAM LLC normalized to the baseline: SPEC CPU2006 suite.}
\label{fig:writes_sc}
\end{figure*}
  
\subsection{Evaluation in a single-core scenario}
\label{subsec:sc}

First, we show the number of writes to the LLC that each evaluated proposal involves as well as the performance delivered. Then, we focus on the involved energy consumption in both the STT-RAM and the main memory according to the model detailed in Section \ref{sec:sim}. Finally, we discuss the obtained results. All the graphs shown in this section report individual data for each benchmark, adding at the right end the arithmetic mean considering all data (labeled as \emph{AVG}) or the geometric mean (labeled as \emph{GMEAN}) in the case of the performance metric, and also the arithmetic mean of the eight most write-intensive benchmarks according to Table~\ref{tab:writeperinst} or the corresponding geometric mean for the performance metric (labeled as \emph{HIGH} in both cases).


\subsubsection{Write filtering}
\label{subsubsec:wr_sc}

Figure~\ref{fig:writes_sc} illustrates the number of writes to the STT-RAM LLC generated by the DASCA scheme and our proposal (using a RD of 8K entries) normalized to a baseline system without any write reduction/filtering scheme.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Escrituras

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As shown, our proposal significantly outperforms DASCA. Notably, in 20 out of 25 benchmarks evaluated the Reuse Detector exhibits higher ability in cutting the write traffic to the STT-RAM LLC. Overall, the block bypassing decisions commanded by RD reduce the number of LLC writes in the baseline system around 65\% whereas DASCA just achieves a 52\% reduction. In addition, if we zoom just in the 8 programs with highest WPKI numbers (those labeled as \emph{high} in Table~\ref{tab:writeperinst}), RD reduces the number of LLC writes by around 80\% with respect to the baseline, while DASCA cuts the write traffic by 66\%.


\subsubsection{Performance}
\label{subsubsec:perf_sc}

Apart from the goal of decreasing the STT-RAM LLC energy consumption (quantified later in this section), it is clear that energy efficiency should not come at the expense of a performance drop. Thus, to further evaluate the benefits of RD, Figure~\ref{fig:perf_sc} shows the performance (IPC) delivered.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Rendimiento
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.95,
				ymax=1.08,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.89,0.98)}, 
				anchor=north,legend columns=5}, 
				symbolic x coords={perlbench,bzip2,gcc,bwaves,mcf,milc,zeusmp,gromacs,cactusADM,leslie3d,namd,gobmk,soplex,calculix,hmmer,GemsFDTD,libquantum,h264ref,tonto,lbm,omnetpp,astar,wrf,sphinx3,xalancbmk,GMEAN,HIGH}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				\addplot [LineFillYellowTiny]coordinates {(perlbench,1.02098) (bzip2,0.96002) (gcc,1.01039) (bwaves,1.00180) (mcf,1.03903) (milc,1.01837) (zeusmp,1.01339) (gromacs,0.99536) (cactusADM,1.00360) (leslie3d,1.01689) (namd,0.99986) (gobmk,1.00110) (soplex,1.00776) (calculix,0.99590) (hmmer,0.97387) (GemsFDTD,1.00000) (libquantum,0.99935) (h264ref,0.99910) (tonto,0.99837) (lbm,1.01832) (omnetpp,0.99990) (astar,0.99900) (wrf,0.98918) (sphinx3,0.99951) (xalancbmk,1.01450) (GMEAN,1.00291)(HIGH,1.013773885)};
		\addplot [LineFillBlueTiny]coordinates {(perlbench,1.01114) (bzip2,1.00619) (gcc,1.02764) (bwaves,1.00172) (mcf,1.18219) (milc,1.04057) (zeusmp,1.00664) (gromacs,0.99306) (cactusADM,1.07121) (leslie3d,1.01627) (namd,0.99983) (gobmk,0.99854) (soplex,1.00252) (calculix,0.99467) (hmmer,1.01914) (GemsFDTD,0.99996) (libquantum,1.06866) (h264ref,0.99767) (tonto,0.99714) (lbm,1.02030) (omnetpp,0.99945) (astar,1.01665) (wrf,0.99479) (sphinx3,0.99931) (xalancbmk,1.01909) (GMEAN,1.01868)(HIGH,1.049550784)};
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Performance (Instructions per Cycle) normalized to the baseline: SPEC CPU2006 suite.}
\label{fig:perf_sc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Overall our scheme performs moderately better than DASCA: RD delivers 1.9\% performance improvement compared to the baseline while DASCA just improves IPC by 0.3\%.
% Also, it is worth to note that in 18 out of 25 benchmarks evaluated our proposal is able to outperform DASCA.
If we focus on the write-intensive applications RD clearly outperforms DASCA, achieving performance improvements of 5\% and 1.4\%, respectively. This reveals, as we will confirm later in the multi-core environment, that our approach works especially well for those applications for which the number of writes performed to the LLC is high.
%, both in terms of writes reduction and performance improvement. 

\subsubsection{Energy savings}
\label{subsubsec:energy_sc}

Figure~\ref{fig:energy_sc} shows the total energy savings (adding both the dynamic and the static components) in the LLC. 
%Since our proposal and DASCA exhibit quite similar performance numbers, this graph almost match the trend observed in the write reduction figure. 
Overall, our proposal reports 34.5\% energy reduction compared to the baseline while DASCA reports 29.5\%. Considering only the write-intensive programs, the numbers are 60\% and 49\%, respectively. If we split the total energy savings with respect to the baseline into the dynamic and static parts, our proposal achieves 50\% of reduction in the dynamic part considering all the applications (68\% for the \emph{high} programs), while DASCA obtains 42\% (57\% for the \emph{high} benchmarks). As for the static part RD is able to obtain 2\% energy savings (around 5\% for the \emph{high programs}) while DASCA just achieves 0.3\% (1.4\% for the write-intensive applications). Note that avoiding LLC writes reduces dynamic energy, whereas increasing performance translates into static energy savings. It is also worth noting that, as Figure~\ref{fig:energysc_llc_break} illustrates, the dynamic energy consumption in the LLC of the baseline system is, for most of the applications evaluated, significantly higher than the static contribution. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.2,
%				ymax=1.05,
				ymax=1,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.1,0.98)}, 
				anchor=north,legend columns=5}, 
%				symbolic x coords={perlbench,bzip2,gcc,bwaves,mcf,milc,zeusmp,gromacs,cactusADM,leslie3d,namd,gobmk,soplex,calculix,hmmer,GemsFDTD,libquantum,h264ref,tonto,lbm,omnetpp,astar,wrf,sphinx3,xalancbmk,GMEAN,HIGH}, 
symbolic x coords={perlbench,bzip2,gcc,bwaves,mcf,milc,zeusmp,gromacs,cactusADM,leslie3d,namd,gobmk,soplex,calculix,hmmer,GemsFDTD,libquantum,h264ref,tonto,lbm,omnetpp,astar,wrf,sphinx3,xalancbmk,AVG,HIGH}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.09em,
				bar width=0.25em,		
				ymajorgrids,
				] 
				%\addplot [LineFillYellowTiny]coordinates {(perlbench,0.59) (bzip2,0.63) (gcc,0.79) (bwaves,0.29) (mcf,0.57) (milc,0.72) (zeusmp,0.38) (gromacs,0.88) (cactusADM,0.33) (leslie3d,0.37) (namd,0.88) (gobmk,0.61) (soplex,0.81) (calculix,0.86) (hmmer,0.90) (GemsFDTD,1.00) (libquantum,1.00) (h264ref,0.97) (tonto,0.98) (lbm,0.41) (omnetpp,1.00) (astar,0.64) (wrf,0.39) (sphinx3,0.88) (xalancbmk,0.73) (GMEAN,0.65947)(HIGH,0.4658542809)};
				\addplot [LineFillYellowTiny]coordinates {(perlbench,0.59) (bzip2,0.63) (gcc,0.79) (bwaves,0.29) (mcf,0.57) (milc,0.72) (zeusmp,0.38) (gromacs,0.88) (cactusADM,0.33) (leslie3d,0.37) (namd,0.88) (gobmk,0.61) (soplex,0.81) (calculix,0.86) (hmmer,0.90) (GemsFDTD,1.00) (libquantum,1.00) (h264ref,0.97) (tonto,0.98) (lbm,0.41) (omnetpp,1.00) (astar,0.64) (wrf,0.39) (sphinx3,0.88) (xalancbmk,0.73) (AVG,0.70496)(HIGH,0.50765)};
			%	\addplot [LineFillBlueTiny]coordinates {(perlbench,0.56) (bzip2,0.69) (gcc,0.62) (bwaves,0.28) (mcf,0.48) (milc,0.25) (zeusmp,0.31) (gromacs,0.82) (cactusADM,0.38) (leslie3d,0.30) (namd,0.84) (gobmk,0.58) (soplex,0.79) (calculix,0.87) (hmmer,0.98) (GemsFDTD,1.00) (libquantum,1.00) (h264ref,0.94) (tonto,0.95) (lbm,0.23) (omnetpp,0.92) (astar,0.67) (wrf,0.37) (sphinx3,0.86) (xalancbmk,0.70) (GMEAN,0.59284)(HIGH,0.3575202976)};
				\addplot [LineFillBlueTiny]coordinates {(perlbench,0.56) (bzip2,0.69) (gcc,0.62) (bwaves,0.28) (mcf,0.48) (milc,0.25) (zeusmp,0.31) (gromacs,0.82) (cactusADM,0.38) (leslie3d,0.30) (namd,0.84) (gobmk,0.58) (soplex,0.79) (calculix,0.87) (hmmer,0.98) (GemsFDTD,1.00) (libquantum,1.00) (h264ref,0.94) (tonto,0.95) (lbm,0.23) (omnetpp,0.92) (astar,0.67) (wrf,0.37) (sphinx3,0.86) (xalancbmk,0.70) (AVG,0.65509)(HIGH,0.40225)};
%\addplot [LineFillYellowTiny]coordinates {(400.perlbench,0.87) (401.bzip2,0.87) (403.gcc,0.93) (410.bwaves,0.71) (429.mcf,0.76) (433.milc,0.86) (434.zeusmp,0.70) (435.gromacs,0.98) (436.cactusADM,0.72) (437.leslie3d,0.72) (444.namd,0.98) (445.gobmk,0.90) (450.soplex,0.94) (454.calculix,0.98) (456.hmmer,0.97) (459.GemsFDTD,1.00) (462.libquantum,1.00) (464.h264ref,1.00) (465.tonto,1.00) (470.lbm,0.71) (471.omnetpp,1.00) (473.astar,0.90) (481.wrf,0.79) (482.sphinx3,0.98) (483.xalancbmk,0.91) (GMEAN,0.88115)(HIGH,0.769016434)};
%		\addplot [LineFillBlueTiny]coordinates {(400.perlbench,0.87) (401.bzip2,0.88) (403.gcc,0.87) (410.bwaves,0.71) (429.mcf,0.70) (433.milc,0.62) (434.zeusmp,0.67) (435.gromacs,0.96) (436.cactusADM,0.72) (437.leslie3d,0.68) (444.namd,0.98) (445.gobmk,0.90) (450.soplex,0.93) (454.calculix,0.98) (456.hmmer,0.99) (459.GemsFDTD,1.00) (462.libquantum,0.98) (464.h264ref,0.99) (465.tonto,0.99) (470.lbm,0.63) (471.omnetpp,0.99) (473.astar,0.89) (481.wrf,0.78) (482.sphinx3,0.98) (483.xalancbmk,0.90)(GMEAN,0.85413)(HIGH,0.708788074)};
%\addplot [LineFillOrangeTiny]coordinates {(400.perlbench,1.01218) (401.bzip2,1.02261) (403.gcc,0.98457) (410.bwaves,0.98333) (429.mcf,0.93681) (433.milc,0.97469) (434.zeusmp,0.96298) (435.gromacs,0.98766) (436.cactusADM,0.94657) (437.leslie3d,0.99543) (444.namd,1.01640) (445.gobmk,0.99046) (450.soplex,0.97306) (454.calculix,0.98271) (456.hmmer,0.98617) (459.GemsFDTD,1.00000) (462.libquantum,0.98933) (464.h264ref,0.97932) (465.tonto,0.98745) (470.lbm,0.93740) (471.omnetpp,0.99905) (473.astar,1.02984) (481.wrf,1.00221) (482.sphinx3,0.99756) (483.xalancbmk,0.95408) (gmean,0.98499)};
%\addplot [LineFillGreenTiny]coordinates {(400.perlbench,0.98916) (401.bzip2,1.00464) (403.gcc,0.97681) (410.bwaves,0.98506) (429.mcf,0.87247) (433.milc,0.94358) (434.zeusmp,0.98881) (435.gromacs,0.99588) (436.cactusADM,0.98608) (437.leslie3d,0.99388) (444.namd,0.98823) (445.gobmk,0.99934) (450.soplex,0.99747) (454.calculix,0.98911) (456.hmmer,0.91441) (459.GemsFDTD,0.99715) (462.libquantum,0.99014) (464.h264ref,0.97981) (465.tonto,0.98474) (470.lbm,0.92943) (471.omnetpp,0.93513) (473.astar,0.99815) (481.wrf,0.99310) (482.sphinx3,0.99741) (483.xalancbmk,0.95459) (gmean,0.97484)};
%				\legend{DASCA LLC,RD LLC, DASCA Mem, RD Mem} 
			  	\legend{DASCA,RD}
			\end{axis}
		\end{tikzpicture}	
%\caption{Energy savings in the LLC and main memory normalized to the baseline: SPEC CPU2006 suite.}
\caption{Energy consumption in the STT-RAM LLC normalized to the baseline: SPEC CPU2006 suite.}
\label{fig:energy_sc}
\end{figure*}

\begin{figure}[h!]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				%height=15em,width=35em,
				height=15em,width=25em,
				ybar stacked, 
				ymin=0,
				ymax=1,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.3)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			symbolic x coords={perlbench,bzip2,gcc,bwaves,mcf,milc,zeusmp,gromacs,cactusADM,leslie3d,namd,gobmk,soplex,calculix,hmmer,GemsFDTD,libquantum,h264ref,tonto,lbm,omnetpp,astar,wrf,sphinx3,xalancbmk,AVG,HIGH}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.35em,
				ymajorgrids,
				] 
				\addplot [LineFillOrangeTinyND]coordinates {(perlbench,0.28) (bzip2,0.17) (gcc,0.23) (bwaves,0.17) (mcf,0.09) (milc,0.11) (zeusmp,0.12) (gromacs,0.39) (cactusADM,0.16) (leslie3d,0.14) (namd,0.81) (gobmk,0.35) (soplex,0.23) (calculix,0.70) (hmmer,0.17) (GemsFDTD,0.99) (libquantum,0.05) (h264ref,0.68) (tonto,0.66) (lbm,0.12) (omnetpp,0.69) (astar,0.27) (wrf,0.22) (sphinx3,0.84) (xalancbmk,0.20) (AVG,0.35) (HIGH,0.12)};
				\addplot [LineFillGreenTinyND]coordinates {(perlbench,0.72) (bzip2,0.83) (gcc,0.77) (bwaves,0.83) (mcf,0.91) (milc,0.89) (zeusmp,0.88) (gromacs,0.61) (cactusADM,0.84) (leslie3d,0.86) (namd,0.19) (gobmk,0.65) (soplex,0.77) (calculix,0.30) (hmmer,0.83) (GemsFDTD,0.01) (libquantum,0.95) (h264ref,0.32) (tonto,0.34) (lbm,0.88) (omnetpp,0.31) (astar,0.73) (wrf,0.78) (sphinx3,0.16) (xalancbmk,0.80) (AVG,0.65) (HIGH,0.88)};
				\legend{Static,Dynamic} 
			\end{axis}
		\end{tikzpicture}	
\caption{Breakdown of energy consumption in the LLC into the static and dynamic contributions for the baseline in the single-core system.}
\label{fig:energysc_llc_break}
\end{figure}


Finally, we have also explored the impact on the energy consumption in the DRAM main memory. For the sake of simplicity, we do not show the results for all the applications. However, as expected, the DRAM energy reduction follows the trend of performance improvement. Overall, our proposal manages to reduce the DRAM energy consumption by 2\% (4.7\% for the write-intensive programs) with respect to the baseline while DASCA just improves the memory energy consumption by 0.2\% (1.1\% for the \emph{high} applications). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Discussion}
\label{subsubsec:disc_sc}

If we zoom into specific benchmarks, there are some special cases that deserve further detail to get a deeper insight. Note that globally, the relative trend shown in the amount of writes to the LLC between our approach and DASCA for each benchmark, is mainly held in the energy consumption differences, although modulated with the relative performance numbers. However, there are some few exceptions such as \emph{namd}, \emph{GemsFDTD} or \emph{omnetpp}, where RD is able to reduce the amount of LLC writes significantly more than DASCA but the energy savings and also the performance improvements obtained by both techniques are almost the same (and quite low compared to the baseline) in all these three cases. The reason is that these programs are three of the four benchmarks that exhibit the lowest values of WPKI, so although the write reductions that RD achieves in relative terms compared to DASCA is significant for these applications, the corresponding reduction in absolute values are very modest, and therefore the impact on the energy is almost negligible.

Also, in other applications such as \emph{mcf}, \emph{cactusADM} or \emph{hmmer}, our approach is able to report IPC numbers significantly higher than in DASCA, while both techniques exhibit quite similar write reduction capabilities. In order to explain that, first note that there are many different aspects involved in the system performance delivered. Among others, one key aspect is that reducing the amount of writes to the LLC is not sufficient in itself to guarantee performance improvements: although the main goals when bypassing blocks from the LLC to main memory 
%--based on the reuse exhibited-- 
are both to save energy and improve performance by increasing the hit rate in the LLC, obviously the bypassing may fail in the sense that a bypassed block could be referenced again soon, leading to a LLC miss and even a performance drop with respect to the case where bypassing is not carried out. Thus, for all these three benchmarks, the experimental data reveal that with our proposal the amount of hits in the LLC clearly outperforms both the baseline and the DASCA mechanism. Notably, the amount of LLC hits experienced in the \emph{cactusADM} and \emph{mcf} programs are 7.23x and 2x the values obtained in the baseline, while DASCA obtains 1.89x and 0.89x, respectively. Also, the amount of misses in the LLC is lower than that of the baseline and DASCA, with values ranging between 0.77-0.87x those obtained in the baseline. Considering all the evaluated benchmarks, RD is able to improve the amount of hits around 31\% with respect to the baseline (106\% if we only consider the write-intensive applications) while DASCA experiments only 5\% increment when considering all the benchmarks and 31\% for the \emph{high} applications. 

At a first glance, the behavior of the \emph{libquantum} application may seem somehow strange: Neither RD nor DASCA are able to significantly reduce the amount of writes to the LLC, but however this benchmark running under RD reports a performance improvement of 7\% with respect to the baseline while the performance remains largely unchanged under DASCA. In addition, and as one would expect since the number of bypasses is low, the number of hits in the LLC is practically the same in the three cases. The reason to explain the performance improvement lies in the LLC bank contention due to the write activity: this application is by far the most stalled one due to write contention. Thus, although the write reduction is very limited with our scheme, it is enough to reduce stalls with respect to the baseline by around 8\%, which in absolute numbers implies various millions of these kind of situations avoided, which leads to the performance improvement obtained.  

Conversely, although other benchmarks such as \emph{gromacs}, \emph{calculix} or \emph{wrf} exhibit moderate LLC writes reduction with RD and DASCA, they all perform worse than in the baseline. For these three programs the amount of hits experienced in the LLC is, in RD and DASCA, lower than in the baseline, which suggests that the bypassing performed is not efficient for these benchmarks. Recall that the energy savings achieved in the LLC as a consequence of the reduction in the number of writes performed in this cache level may be partially offset with the performance drop derived from the increment in the amount of LLC misses, as in these three programs occurs. Note also that, although the write operations are outside the critical path, the performance improvement derived from avoiding the long write operations may be mitigated if bank contention exists between the writes effectively performed.




%\subsubsection{Sensitivity to Reuse Detector size}
%\label{subsubsec:sense}

%One key aspect in designing the Reuse Detector is to decide the \emph{expulsion coverage} it provides. In other words, the RD size is an important issue in the implementation of our proposal. In order to evaluate the real impact that this design parameter has over our approach operation we show in Figure~\ref{fig:sense_sc} the amount of writes to the LLC, the execution time and the energy savings in the LLC and the main memory that our proposal obtains for different RD sizes (8K, 16K, 32K and 64K entries). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Sensibilidad a tamaño detector reuso
%\begin{figure*}
%		\begin{tikzpicture} 
%		\centering
%			\begin{axis}[ 
%				small,
%				height=15em,width=40em,
%				ybar, 
%				ymin=0.35,
	%			ymax=1,
%				enlargelimits=0.1, 
%				legend style={font=\scriptsize,at={(0.5,-0.5)}, 
%				anchor=north,legend columns=5}, 
%				symbolic x coords={Writes LLC,Execution time,Eng. STT-RAM,Eng. DRAM}, 
%				xtick=data, 
 %			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
	%			bar width=0.5em,
	%			ymajorgrids,
	%			] 
	%			\addplot [LineFillRedTiny]coordinates {(Writes LLC,0.3815712192) (Execution time,0.9868404568) (Eng. STT-RAM,0.8785844706) (Eng. DRAM,0.97962)};
	%			\addplot [LineFillBlueTiny]coordinates {(Writes LLC,0.4267534086) (Execution time,0.9833294454) (Eng. STT-RAM,0.8865538883) (Eng. DRAM,0.97484)};
	%			\addplot [LineFillOrangeTiny]coordinates {(Writes LLC,0.4610461448) (Execution time,0.9848443445) (Eng. STT-RAM,0.8937317659) (Eng. DRAM,0.97575)};
	%			\addplot [LineFillGreenTiny]coordinates {(Writes LLC,0.5129674339) (Execution time,0.9865762562) (Eng. STT-RAM,0.9029528596) (Eng. DRAM,0.97979)};
	%			\legend{8K,16K,32K,64K} 
	%		\end{axis}
	%	\end{tikzpicture}	
%\caption{Writes to LLC, execution time, and energy savings in both LLC and main memory normalized to the baseline for different RD sizes: SPEC CPU2006 suite.}
%\label{fig:sense_sc}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As shown, the major impact is observed on the capability to reduce the number of writes in the LLC, ranging from the 38\% of the writes the baseline perform when a RD of 8K is employed until the 51\% when a 64K RD is used. Note that maybe these data might appear contradictory at first sight. However, they are not: As the size of the RD increases, it also augments the probability that a block finds its tag in the RD, so the probability of bypass decreases, leading to minor amount of writes to the LLC. We can also observe a slight impact on the energy consumed in the LLC, with values in the range 87.8-90.3\% when increasing the size of the RD: again, note that these numbers follow the same trend exhibited by the amount of writes. Finally, the impact over the performance and the energy consumption of the main memory is almost negligible, showing both almost constant numbers.    





\subsection{Evaluation in a 4-core CMP system}
\label{subsec:mc}

In this section we extend the previous single-core analysis to a more up-to-date environment: a multi-core scenario where the LLC is shared among different cores. 
%We now evaluate the same policies that in the single-core environment --our Reuse Detector and the DASCA approach-- using multiprogrammed workloads. 
For this purpose, we measure again the number of writes to the SLLC, the performance and the energy consumption in both the STT-RAM SLLC and the DRAM main memory for RD and DASCA and report results normalized to the baseline. However, due to the inherent non-determinism that all simulators exhibit (especially in multi-core environments, where the number of instructions executed across different schemes are not stable owing to the random interleaving among memory accesses of different programs) and for the sake of higher accuracy, we employ in this scenario, as well as in the 8 and 16-core CMP systems, the arithmetic mean of the number of writes and energy consumption (per application) but \emph{divided by the total number of instructions executed}. 
%(as well as the geometric mean of the IPC to compute the performance). 
Note that, conversely, in the single-core scenario both kind of metrics match, since all the benchmarks execute the same amount of instructions (1B) in all the runs. %Finally, in Section~\ref{subsubsec:other} we further explore other insightful metrics in order to clarify the real contribution of the evaluated policies. 

We employ 28 mixes made up of applications from the SPEC CPU2006 suite chosen accordingly to the WPKI categories illustrated in Table~\ref{tab:writeperinst}. First, we randomly compose three groups of 4 mixes made up of applications belonging to just one WPKI category (mixes referred to as H$i$, M$i$ and L$i$ for high, medium and low WPKI respectively). Then, we build other 16 mixes merging applications with WPKI corresponding to different categories and trying to construct them in a balanced and homogeneous fashion. Again, the workload name encodes the WPKI categories of the applications. For example, HL2 is the third mix we build consisting of applications with high WPKI (2 in this case) and applications with low WPKI (other two). The detailed mixes are illustrated in Table~\ref{tab:mix4C}. Most graphs in this section report individual results for each mix, the arithmetic mean (AVG) considering all the mixes, just the 4 H$i$ mixes (HIGH), the 4 H$i$ and the 4 HM$i$ mixes together (H+HM), the 4 H$i$, the 4 HM$i$ and the 4 HML$i$ mixes together (H+HM+HML) and all the mixes including at least a high program (SomeH). Again, in the case of the performance metric we employ the geometric mean instead of the arithmetic one.


\subsubsection{Write filtering}
\label{subsubsec:wr_mc}

Figure~\ref{fig:writes_mc} illustrates the number of writes to the STT-RAM SLLC generated by using DASCA and an 8K-entry RD per core normalized to a baseline STT-RAM without any write reduction mechanism. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Writes mc
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.05,
				ymax=0.87,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.7,0.98)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				%\addplot [LineFillRedTiny]coordinates {(H0,) (H1,) (H2,) (H3,) (HL0,) (HL1,) (HL2,) (HL3,) (HM0,) (HM1,) (HM2,) (HM3,) (HML0,) (HML1,) (HML2,) (HML3,) (L0,) (L1,) (L2,) (L3,) (M0,) (M1,) (M2,) (M3,) (ML0,) (ML1,) (ML2,) (ML3,) (GMEAN,)(HIGH,)(H+HM,)(H+HM+HML,)(SomeH,)};
				%\addplot [LineFillYellowTiny]coordinates {(H0,0.71) (H1,0.21) (H2,0.79) (H3,0.11) (HL0,0.09) (HL1,0.82) (HL2,0.16) (HL3,0.44) (HM0,0.41) (HM1,0.79) (HM2,0.40) (HM3,0.19) (HML0,0.44) (HML1,0.82) (HML2,0.55) (HML3,0.15) (L0,0.27) (L1,0.88) (L2,0.52) (L3,0.65) (M0,0.57) (M1,0.40) (M2,0.72) (M3,0.28) (ML0,0.49) (ML1,0.70) (ML2,0.20) (ML3,0.76) (GMEAN,0.40509)(HIGH,0.3395846574)(H+HM,0.3672987076)(H+HM+HML,0.3831090566)(SomeH,0.3507990488)};
				\addplot [LineFillYellowTiny]coordinates {(H0,0.71) (H1,0.21) (H2,0.79) (H3,0.11) (HL0,0.09) (HL1,0.82) (HL2,0.16) (HL3,0.44) (HM0,0.41) (HM1,0.79) (HM2,0.40) (HM3,0.19) (HML0,0.44) (HML1,0.82) (HML2,0.55) (HML3,0.15) (L0,0.27) (L1,0.88) (L2,0.52) (L3,0.65) (M0,0.57) (M1,0.40) (M2,0.72) (M3,0.28) (ML0,0.49) (ML1,0.70) (ML2,0.20) (ML3,0.76) (AVG,0.48387)(HIGH,0.4578)(H+HM,0.45322)(H+HM+HML,0.46599)(SomeH,0.444010)};
%				\addplot [LineFillBlueTiny]coordinates {(H0,0.75) (H1,0.18) (H2,0.75) (H3,0.14) (HL0,0.11) (HL1,0.82) (HL2,0.15) (HL3,0.17) (HM0,0.32) (HM1,0.79) (HM2,0.25) (HM3,0.28) (HML0,0.42) (HML1,0.50) (HML2,0.32) (HML3,0.17) (L0,0.21) (L1,0.78) (L2,0.36) (L3,0.60) (M0,0.58) (M1,0.41) (M2,0.71) (M3,0.37) (ML0,0.44) (ML1,0.68) (ML2,0.20) (ML3,0.69) (GMEAN,0.36722)(HIGH,0.3461276381)(H+HM,0.3561446329)(H+HM+HL,0.3457862128)(SomeH,0.3102827744)};  RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.74) (H1,0.09) (H2,0.73) (H3,0.08) (HL0,0.06) (HL1,0.82) (HL2,0.12) (HL3,0.09) (HM0,0.22) (HM1,0.78) (HM2,0.18) (HM3,0.25) (HML0,0.39) (HML1,0.45) (HML2,0.25) (HML3,0.12) (L0,0.13) (L1,0.76) (L2,0.27) (L3,0.59) (M0,0.52) (M1,0.31) (M2,0.66) (M3,0.27) (ML0,0.39) (ML1,0.67) (ML2,0.16) (ML3,0.64) (GMEAN,0.29273)(HIGH,0.2512276929)(H+HM,0.2737899067)(H+HM+HL,0.2732734405)(SomeH,0.2362530442)}; RD 0.5x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.75) (H1,0.07) (H2,0.71) (H3,0.07) (HL0,0.04) (HL1,0.82) (HL2,0.10) (HL3,0.05) (HM0,0.16) (HM1,0.78) (HM2,0.13) (HM3,0.34) (HML0,0.59) (HML1,0.44) (HML2,0.23) (HML3,0.10) (L0,0.12) (L1,0.75) (L2,0.19) (L3,0.56) (M0,0.52) (M1,0.29) (M2,0.67) (M3,0.24) (ML0,0.36) (ML1,0.63) (ML2,0.11) (ML3,0.61) (GMEAN,0.26170)(HIGH,0.2263099303)(H+HM,0.2493137381)(H+HM+HML,0.2587826632)(SomeH,0.2099018837)}; %RD 0.25x
				\addplot [LineFillBlueTiny]coordinates {(H0,0.75) (H1,0.07) (H2,0.71) (H3,0.07) (HL0,0.04) (HL1,0.82) (HL2,0.10) (HL3,0.05) (HM0,0.16) (HM1,0.78) (HM2,0.13) (HM3,0.34) (HML0,0.59) (HML1,0.44) (HML2,0.23) (HML3,0.10) (L0,0.12) (L1,0.75) (L2,0.19) (L3,0.56) (M0,0.52) (M1,0.29) (M2,0.67) (M3,0.24) (ML0,0.36) (ML1,0.63) (ML2,0.11) (ML3,0.61) (AVG,0.37310)(HIGH,0.4011)(H+HM,0.377347)(H+HM+HML,0.364747)(SomeH,0.33658)}; %RD 0.25x
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Number of writes to the STT-RAM SLLC normalized to the baseline in the 4-core CMP system.}
\label{fig:writes_mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The experimental results reveal that the RD and DASCA performs similarly in decreasing the amount of writes to the SLCC. Overall, our technique makes just around 36\% of the writes the baseline does, while DASCA performs around 40\%. These percentages decrease even slightly more for the mixes with write-intensive applications under both schemes. %Notably, in 21 out of 28 mixes evaluated the Reuse Detector exhibits higher ability in cutting the write traffic to the STT-RAM LLC.

The experimental results reveal that RD exhibits a significantly greater ability to decrease the amount of writes to the SLLC than DASCA. Notably, in 25 out of the 28 mixes evaluated RD outperforms DASCA. Overall, the number of writes in the baseline system gets reduced to 37\% by using RD, in contrast with DASCA which only achieves a 48\%. As for the write-intensive mixes the RD and DASCA makes around 40\% and 46\% of the writes the baseline performs, respectively.



\subsubsection{Performance}
\label{subsubsec:perf_mc}

In order to evaluate performance when executing multiprogrammed workloads, we analyze the \emph{Instruction Throughput} (IT) and the \emph{Weighted Speedup} (WS) metrics. The IT metric is defined as the sum of all instructions committed per cycle in the entire chip ($\sum_{i=1}^{n} IPC_i$, being \emph{n} the number of threads), while the WS is defined as the slowdown experienced by each application in a mix, compared to its run under the same configuration when no other application is running on other cores ($\sum_{i=1}^{n} (IPC_{i}^{shared}/IPC_{i}^{alone})$). For the sake of simplicity and since in our context the WS does not constitute a metric as significant as IT, we do not show the WS results obtained. Anyway, these results follow an analogous trend to those obtained when we evaluate the instruction throughput.
Figure~\ref{fig:perf_mc} illustrates the IT that each evaluated policy delivers normalized to the baseline. %Note that, unlike in the case of execution time metrics, now values higher than 1 imply performance improvements with respect to the baseline.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Throughput%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.95,
				%ymax=1.14,
				ymax=1.1,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.89,0.98)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				\addplot [LineFillYellowTiny]coordinates {(H0,1.01857) (H1,1.02080) (H2,1.00091) (H3,1.02689) (HL0,1.01471) (HL1,1.00755) (HL2,1.01565) (HL3,1.00194) (HM0,1.01827) (HM1,1.01771) (HM2,1.01718) (HM3,1.05025) (HML0,1.04537) (HML1,0.96201) (HML2,0.98627) (HML3,1.01996) (L0,1.00196) (L1,0.99804) (L2,1.00242) (L3,0.99932) (M0,1.01543) (M1,1.01520) (M2,1.02813) (M3,1.03876) (ML0,1.00020) (ML1,1.01218) (ML2,1.00875) (ML3,1.00454) (GMEAN,1.01232)(HIGH,1.0167475297)(H+HM,1.0212414208)(H+HM+HML,1.0150904998)(SomeH,1.0138022338)};
			%	\addplot [LineFillBlueTiny]coordinates {(H0,1.05825) (H1,1.13895) (H2,1.05085) (H3,1.17208) (HL0,1.12582) (HL1,1.01302) (HL2,1.02099) (HL3,1.01339) (HM0,1.05904) (HM1,1.02530) (HM2,1.04997) (HM3,1.06787) (HML0,1.06060) (HML1,1.02984) (HML2,1.03786) (HML3,1.03155) (L0,1.00066) (L1,0.99689) (L2,0.99846) (L3,0.99930) (M0,1.02746) (M1,1.02408) (M2,1.03079) (M3,1.06066) (ML0,0.99873) (ML1,1.01980) (ML2,0.96218) (ML3,1.00374) (GMEAN,1.03757)(HIGH,1.1038163119)(H+HM,1.0767902358)(H+HM+HL,1.0643475087)(SomeH,1.0587793992)}; RD 1x
			%	\addplot [LineFillBlueTiny]coordinates {(H0,1.04036) (H1,1.07012) (H2,1.05262) (H3,1.08448) (HL0,1.02299) (HL1,1.01318) (HL2,1.01933) (HL3,1.00816) (HM0,1.06447) (HM1,1.02202) (HM2,1.04654) (HM3,1.08542) (HML0,1.07735) (HML1,1.03366) (HML2,1.03547) (HML3,1.03193) (L0,1.00148) (L1,0.99579) (L2,0.99802) (L3,0.99956) (M0,1.02435) (M1,1.02223) (M2,1.03526) (M3,1.05505) (ML0,0.99999) (ML1,1.01616) (ML2,1.00956) (ML3,1.00490) (GMEAN,1.03075)(HIGH,1.0617592884)(H+HM,1.0580508321)(H+HM+HL,1.0534915634)(SomeH,1.0439650806)}; RD 0.5x
				\addplot [LineFillBlueTiny]coordinates {(H0,1.03670) (H1,1.12092) (H2,1.04394) (H3,1.08512) (HL0,1.01851) (HL1,1.01306) (HL2,1.01676) (HL3,1.00664) (HM0,1.04620) (HM1,1.01778) (HM2,1.03095) (HM3,1.08355) (HML0,1.07683) (HML1,1.03149) (HML2,1.01569) (HML3,1.02893) (L0,1.00199) (L1,0.99996) (L2,1.01299) (L3,0.99749) (M0,1.01784) (M1,1.02147) (M2,1.03071) (M3,1.04738) (ML0,0.99755) (ML1,1.01323) (ML2,1.00809) (ML3,1.00363) (GMEAN,1.02907)(HIGH,1.0711356597)(H+HM,1.057649046)(H+HM+HML,1.0510526827)(SomeH,1.041595001)}; %RD 0.25x

				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Instruction throughput normalized to the baseline in the 4-core CMP system.}
\label{fig:perf_mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As shown, RD moderately outperforms DASCA. This is a key contribution of RD, since our approach, managing to reduce the amount of writes to the SLLC to a greater extent than DASCA, is also able to deliver higher performance (which also allows to report higher energy savings in both the SLLC and the main memory as shown later). The data reveal that, overall, RD improves performance by around 3\% compared to the baseline, while DASCA just improves it by around 1.2\%. Moreover, we can observe that, in almost all of the 28 mixes evaluated (except mainly those mixes made up of benchmarks with a reduced WPKI, those labeled as \emph{low}, where the performance of both techniques essentially matches that of the baseline), our technique performs better. %Just in 2 of the studied mixes the DASCA scheme manages to perform slightly better than our approach. Also, zooming into particular workloads, we see that in many of them the RD significantly outperforms DASCA: For example, HL3 (26\% vs 9\%), HM1 (48\% vs 14\%) or HM3 (24\% vs 5\%).
Zooming into particular mixes, the results reveal that RD performs especially better than DASCA in those mixes made up of write-intensive applications. Thus, our approach reports a performance improvement of more than 7\% when considering just the H$_i$ mixes while DASCA just reports 1.7\% IT improvement with respect to the baseline. Also, RD delivers significantly higher performance than DASCA and the baseline for those mixes which contain any application with high WPKI. 




\subsubsection{Energy savings}
\label{subsubsec:energy_mc}

Figure~\ref{fig:energy_mc} illustrates the energy savings in the SLLC. As in the single-core scenario, the graph follows a similar relative trend between our approach and DASCA to that observed in the write reduction numbers (Figure~\ref{fig:writes_mc}), just slightly modulated with the performance numbers since, as shown in Figure~\ref{fig:energy_llc_break}, the dynamic contribution to the energy consumption in the SLLC is higher than the static part (except in the mixes made up of applications with low WPKI only), so that the ability to reduce the amount of writes to the SLLC (dynamic contribution) impacts the total energy consumption more than the ability to improve performance, which mainly affects the static contribution. Overall, our proposal reports around 37\% energy reduction in the STT-RAM SLLC compared to the baseline while DASCA reduces it by around 31\%. If we zoom into the write-intensive mixes, both RD and DASCA are able to save around 45\% and 39\% of SLLC energy consumption, respectively. If we break the SLLC energy numbers down into the static and dynamic contributions, 
%we obtain the Figure~\ref{fig:energy_break_mc}, which 
our results reveal that, overall, RD is able to reduce --considering all mixes-- the static energy part by around 2.7\% with respect to the baseline (around 6\% for the write-intensive mixes) while DASCA reduces the static contribution by 1.2\% (1.7\% for the \emph{high} mixes). In addition, our approach reports dynamic energy savings of around 50\% (51\% for the \emph{high} mixes) while DASCA numbers are 42\% (46\% for the \emph{high} mixes).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy STT
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.3,
				ymax=0.98,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.705,0.98)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
%				\addplot [LineFillYellowTiny]coordinates {(H0,0.82859) (H1,0.53729) (H2,0.86918) (H3,0.48613) (HL0,0.53250) (HL1,0.89905) (HL2,0.59969) (HL3,0.73079) (HM0,0.68606) (HM1,0.87807) (HM2,0.68673) (HM3,0.60790) (HML0,0.72432) (HML1,0.92331) (HML2,0.78712) (HML3,0.64104) (L0,0.87359) (L1,0.97907) (L2,0.93043) (L3,0.93178) (M0,0.84761) (M1,0.80694) (M2,0.88082) (M3,0.74649) (ML0,0.87089) (ML1,0.87811) (ML2,0.76132) (ML3,0.93665) (GMEAN,0.76766)(HIGH,0.6585730467)(H+HM,0.6829145233)(H+HM+HML,0.7083719571)(SomeH,0.7003416111)};
%				\addplot [LineFillYellowTiny]coordinates {(H0,) (H1,) (H2,) (H3,) (HL0,) (HL1,) (HL2,) (HL3,) (HM0,) (HM1,) (HM2,) (HM3,) (HML0,) (HML1,) (HML2,) (HML3,) (L0,) (L1,) (L2,) (L3,) (M0,) (M1,) (M2,) (M3,) (ML0,) (ML1,) (ML2,) (ML3,) (GMEAN,)(HIGH,)(H+HM,)(H+HM+HML,)(SomeH,)};
				%\addplot [LineFillYellowTiny]coordinates {(H0,0.78) (H1,0.43) (H2,0.84) (H3,0.36) (HL0,0.39) (HL1,0.86) (HL2,0.45) (HL3,0.64) (HM0,0.59) (HM1,0.84) (HM2,0.59) (HM3,0.45) (HML0,0.62) (HML1,0.90) (HML2,0.71) (HML3,0.47) (L0,0.77) (L1,0.96) (L2,0.87) (L3,0.88) (M0,0.76) (M1,0.68) (M2,0.82) (M3,0.61) (ML0,0.78) (ML1,0.82) (ML2,0.62) (ML3,0.89) (GMEAN,0.66758)(HIGH,0.5637257099)(H+HM,0.5839259095)(H+HM+HML,0.6072292805)(SomeH,0.5941499685)};
				\addplot [LineFillYellowTiny]coordinates {(H0,0.78) (H1,0.43) (H2,0.84) (H3,0.36) (HL0,0.39) (HL1,0.86) (HL2,0.45) (HL3,0.64) (HM0,0.59) (HM1,0.84) (HM2,0.59) (HM3,0.45) (HML0,0.62) (HML1,0.90) (HML2,0.71) (HML3,0.47) (L0,0.77) (L1,0.96) (L2,0.87) (L3,0.88) (M0,0.76) (M1,0.68) (M2,0.82) (M3,0.61) (ML0,0.78) (ML1,0.82) (ML2,0.62) (ML3,0.89) (AVG,0.69164)(HIGH,0.6019280356)(H+HM,0.6107521864)(H+HM+HML,0.6319234379)(SomeH,0.6201476595)};
		%		\addplot [LineFillBlueTiny]coordinates {(H0,0.85801) (H1,0.51200) (H2,0.85399) (H3,0.49029) (HL0,0.53960) (HL1,0.89724) (HL2,0.60553) (HL3,0.60472) (HM0,0.63448) (HM1,0.87713) (HM2,0.61019) (HM3,0.66396) (HML0,0.74332) (HML1,0.77428) (HML2,0.67579) (HML3,0.65341) (L0,0.86103) (L1,0.96715) (L2,0.91212) (L3,0.92438) (M0,0.84673) (M1,0.81039) (M2,0.88073) (M3,0.77690) (ML0,0.86238) (ML1,0.87075) (ML2,0.76328) (ML3,0.91413) (GMEAN,0.75044)(HIGH,0.6548887237)(H+HM,0.6717688533)(H+HM+HL,0.6842824663)(SomeH,0.6752551993)}; RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.84976) (H1,0.46317) (H2,0.84088) (H3,0.46505) (HL0,0.51288) (HL1,0.89706) (HL2,0.57906) (HL3,0.56911) (HM0,0.57837) (HM1,0.87224) (HM2,0.56875) (HM3,0.64764) (HML0,0.72344) (HML1,0.74552) (HML2,0.63855) (HML3,0.63048) (L0,0.84627) (L1,0.96326) (L2,0.89790) (L3,0.92117) (M0,0.82396) (M1,0.77669) (M2,0.86005) (M3,0.74003) (ML0,0.84158) (ML1,0.86418) (ML2,0.74629) (ML3,0.90156) (GMEAN,0.72576)(HIGH,0.6263528984)(H+HM,0.6412771004)(H+HM+HL,0.6547737472)(SomeH,0.646943375)}; RD 0.5 x
%				\addplot [LineFillBlueTiny]coordinates {(H0,0.85493) (H1,0.44983) (H2,0.83045) (H3,0.45869) (HL0,0.49642) (HL1,0.89526) (HL2,0.58151) (HL3,0.54746) (HM0,0.55642) (HM1,0.88234) (HM2,0.54764) (HM3,0.69141) (HML0,0.81504) (HML1,0.73861) (HML2,0.62668) (HML3,0.61807) (L0,0.84347) (L1,0.97018) (L2,0.88796) (L3,0.92037) (M0,0.82774) (M1,0.76538) (M2,0.86471) (M3,0.73405) (ML0,0.83936) (ML1,0.85364) (ML2,0.73374) (ML3,0.91700) (GMEAN,0.72362)(HIGH,0.6186626176)(H+HM,0.6373607474)(H+HM+HML,0.6559892547)(SomeH,0.6450477008)}; %RD 0.25x
%\addplot [LineFillBlueTiny]coordinates {(H0,0.81) (H1,0.32) (H2,0.78) (H3,0.32) (HL0,0.34) (HL1,0.86) (HL2,0.42) (HL3,0.38) (HM0,0.42) (HM1,0.83) (HM2,0.40) (HM3,0.56) (HML0,0.72) (HML1,0.63) (HML2,0.49) (HML3,0.44) (L0,0.71) (L1,0.93) (L2,0.78) (L3,0.85) (M0,0.73) (M1,0.62) (M2,0.80) (M3,0.59) (ML0,0.72) (ML1,0.78) (ML2,0.57) (ML3,0.83) (GMEAN,0.59910)(HIGH,0.5048902032)(H+HM,0.5171554316)(H+HM+HML,0.5312114002)(SomeH,0.5139849621)}; %RD 0.25x nueva celda
			\addplot [LineFillBlueTiny]coordinates {(H0,0.81) (H1,0.32) (H2,0.78) (H3,0.32) (HL0,0.34) (HL1,0.86) (HL2,0.42) (HL3,0.38) (HM0,0.42) (HM1,0.83) (HM2,0.40) (HM3,0.56) (HML0,0.72) (HML1,0.63) (HML2,0.49) (HML3,0.44) (L0,0.71) (L1,0.93) (L2,0.78) (L3,0.85) (M0,0.73) (M1,0.62) (M2,0.80) (M3,0.59) (ML0,0.72) (ML1,0.78) (ML2,0.57) (ML3,0.83) (AVG,0.62993)(HIGH,0.5572038011)(H+HM,0.5553389599)(H+HM+HML,0.5606663465)(SomeH,0.5456462651)}; %RD 0.25x nueva celda
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Energy consumption in the STT-RAM SLLC normalized to the baseline in the 4-core CMP system.}
\label{fig:energy_mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				%height=15em,width=40em,
				height=15em,width=28em,
				ybar stacked, 
				ymin=0,
				ymax=1,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.2)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.35em,
				ymajorgrids,
				] 
				%\addplot [LineFillOrangeTiny]coordinates {(H0,) (H1,) (H2,) (H3,) (HL0,) (HL1,) (HL2,) (HL3,) (HM0,) (HM1,) (HM2,) (HM3,) (HML0,) (HML1,) (HML2,) (HML3,) (L0,) (L1,) (L2,) (L3,) (M0,) (M1,) (M2,) (M3,) (ML0,) (ML1,) (ML2,) (ML3,) (AVG,)};
			%	\addplot [LineFillOrangeTiny]coordinates {(H0,0.1069615018) (H1,0.3003637176) (H2,0.1052560516) (H3,0.3198223341) (HL0,0.369791511) (HL1,0.1197104341) (HL2,0.3973856416) (HL3,0.388472699) (HM0,0.305374527) (HM1,0.1152463138) (HM2,0.3108988198) (HM3,0.2617843244) (HML0,0.3108680329) (HML1,0.3744491975) (HML2,0.3571170264) (HML3,0.3488694863) (L0,0.7747538635) (L1,0.6536725021) (L2,0.7805431398) (L3,0.6584482362) (M0,0.3115498335) (M1,0.3615679394) (M2,0.3394152136) (M3,0.4736860266) (ML0,0.5437705416) (ML1,0.3992941945) (ML2,0.559310475) (ML3,0.3929526785) (AVG,0.3836191523)};
			%	\addplot [LineFillGreenTiny]coordinates {(H0,0.8930384982) (H1,0.6996362824) (H2,0.8947439484) (H3,0.6801776659) (HL0,0.630208489) (HL1,0.8802895659) (HL2,0.6026143584) (HL3,0.611527301) (HM0,0.694625473) (HM1,0.8847536862) (HM2,0.6891011802) (HM3,0.7382156756) (HML0,0.6891319671) (HML1,0.6255508025) (HML2,0.6428829736) (HML3,0.6511305137) (L0,0.2252461365) (L1,0.3463274979) (L2,0.2194568602) (L3,0.3415517638) (M0,0.6884501665) (M1,0.6384320606) (M2,0.6605847864) (M3,0.5263139734) (ML0,0.4562294584) (ML1,0.6007058055) (ML2,0.440689525) (ML3,0.6070473215) (AVG,0.6163808477)};
				\addplot [LineFillOrangeTiny]coordinates {(H0,0.0619427583) (H1,0.1622439114) (H2,0.0606291134) (H3,0.1748128821) (HL0,0.2117569329) (HL1,0.0711839078) (HL2,0.2368209709) (HL3,0.2290220572) (HM0,0.1731064075) (HM1,0.0680206784) (HM2,0.1786222668) (HM3,0.1548876188) (HML0,0.1892045379) (HML1,0.2349018674) (HML2,0.2153141768) (HML3,0.2162143336) (L0,0.6206672433) (L1,0.5465837959) (L2,0.6545243501) (L3,0.5324957932) (M0,0.2142895397) (M1,0.2515777633) (M2,0.2252295519) (M3,0.324168571) (ML0,0.4090330711) (ML1,0.266552559) (ML2,0.3957713827) (ML3,0.2939385964) (AVG,0.26333988)};
				\addplot [LineFillGreenTiny]coordinates {(H0,0.9380572417) (H1,0.8377560886) (H2,0.9393708866) (H3,0.8251871179) (HL0,0.7882430671) (HL1,0.9288160922) (HL2,0.7631790291) (HL3,0.7709779428) (HM0,0.8268935925) (HM1,0.9319793216) (HM2,0.8213777332) (HM3,0.8451123812) (HML0,0.8107954621) (HML1,0.7650981326) (HML2,0.7846858232) (HML3,0.7837856664) (L0,0.3793327567) (L1,0.4534162041) (L2,0.3454756499) (L3,0.4675042068) (M0,0.7857104603) (M1,0.7484222367) (M2,0.7747704481) (M3,0.675831429) (ML0,0.5909669289) (ML1,0.733447441) (ML2,0.6042286173) (ML3,0.7060614036) (AVG,0.73666012)};
				\legend{Static,Dynamic} 
			\end{axis}
		\end{tikzpicture}	
\caption{Breakdown of energy consumption in the SLLC into the static and dynamic contributions for the baseline in the 4-core CMP system.}
\label{fig:energy_llc_break}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy STT Satic-dynamic
%\begin{figure*}
%		\begin{tikzpicture} 
%		\centering
%			\begin{axis}[ 
%				small,
%				height=15em,width=44em,
%				ybar, 
%				ymin=0.45,
%				ymax=1.02,
%				enlargelimits=0.03, 
%				legend style={font=\scriptsize,at={(0.5,-0.5)}, 
%				anchor=north,legend columns=5}, 
				%%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
%			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN}, 
%				xtick=data, 
 %			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
	%			bar width=0.07em,
	%			ymajorgrids,
	%			] 
	%			\addplot [LineFillRedTiny]coordinates {(H0,0.97474) (H1,0.88745) (H2,0.88409) (H3,0.93751) (HL0,0.96525) (HL1,0.99790) (HL2,0.99524) (HL3,0.91397) (HM0,0.96720) (HM1,0.87232) (HM2,0.95301) (HM3,0.95027) (HML0,0.99364) (HML1,0.97874) (HML2,0.98232) (HML3,0.98339) (L0,1.00219) (L1,1.00486) (L2,0.97625) (L3,0.99244) (M0,0.98060) (M1,0.98679) (M2,0.99129) (M3,0.98469) (ML0,1.01795) (ML1,0.99293) (ML2,0.99800) (ML3,0.99182) (GMEAN,0.96914)};
	%			\addplot [LineFillBlueTiny]coordinates {(H0,0.90348) (H1,0.84879) (H2,0.82519) (H3,0.86694) (HL0,0.91841) (HL1,0.97896) (HL2,0.99112) (HL3,0.79100) (HM0,0.93636) (HM1,0.67433) (HM2,0.91561) (HM3,0.80471) (HML0,0.96722) (HML1,0.97735) (HML2,0.96237) (HML3,0.96479) (L0,1.00075) (L1,0.99875) (L2,0.96180) (L3,0.98670) (M0,0.94976) (M1,0.95126) (M2,0.94994) (M3,0.95728) (ML0,0.97824) (ML1,0.94269) (ML2,0.99836) (ML3,0.98276) (GMEAN,0.92459)};
	%			\addplot [LineFillOrangeTiny]coordinates {(H0,0.82148) (H1,0.92521) (H2,0.91691) (H3,0.95484) (HL0,0.90964) (HL1,0.48262) (HL2,0.76555) (HL3,0.92680) (HM0,0.78355) (HM1,0.90400) (HM2,0.75335) (HM3,0.83297) (HML0,0.91425) (HML1,0.82470) (HML2,0.85135) (HML3,0.81896) (L0,0.94640) (L1,0.94350) (L2,0.85964) (L3,0.67651) (M0,0.92369) (M1,0.81160) (M2,0.80310) (M3,0.74383) (ML0,0.86557) (ML1,0.75279) (ML2,0.97419) (ML3,0.90203) (GMEAN,0.83516)};
	%			\addplot [LineFillGreenTiny]coordinates {(H0,0.82066) (H1,0.93740) (H2,0.91258) (H3,0.94549) (HL0,0.85617) (HL1,0.46759) (HL2,0.71094) (HL3,0.88217) (HM0,0.79883) (HM1,0.84322) (HM2,0.83201) (HM3,0.89089) (HML0,0.79316) (HML1,0.78972) (HML2,0.92430) (HML3,0.80993) (L0,0.73210) (L1,0.92514) (L2,0.81202) (L3,0.67849) (M0,0.83537) (M1,0.71247) (M2,0.82542) (M3,0.66686) (ML0,0.76917) (ML1,0.57872) (ML2,0.92891) (ML3,0.93950) (GMEAN,0.79877)};
	%			\legend{DASCA Static, RD Static, DASCA Dynamic, RD Dynamic} 
	%		\end{axis}
	%	\end{tikzpicture}	
%\caption{Energy consumption (static vs dynamic) in the LLC normalized to the baseline: multiprogrammed workloads.}
%\label{fig:energy_break_mc}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

Also, we explore the energy savings obtained in the DRAM main memory, where the leakage contribution has far greater significance than in the STT-RAM SLLC, so that the trends obtained essentially follow those of the IT graph, but inverted (higher performance translates into lower DRAM energy consumption). Figure~\ref{fig:energy_dram_mc} illustrates that RD manages to additionally reduce the energy consumption of the main memory by around 6.2\% on average compared to the baseline (8.3\% for the write-intensive mixes), while DASCA barely reaches a 3.6\% energy reduction (around 2\% for the \emph{high} mixes), mainly due to the higher performance improvement that our proposal exhibits. 

%The reasons to explain this improvement are twofold. First, the RD improves the row buffer read hit rates by 5.3\% on average, around twice the DASCA number. This is because bypassing closing writes has an effect of performing writebacks earlier, which increases the locality between read and write commands to the main memory [34]. Second, DASCA reduces the number of main memory accesses by 3% on average since bypassing dead-on-arrival fills increases the effective capacity of the L2 cache and bypassing closing writes proactively evicts dead blocks from the L2 cache thereby improving the cache efficiency.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy DRAM
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.8,
				ymax=1.06,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.89,0.98)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				%\addplot [LineFillYellowTiny]coordinates {(H0,0.98067) (H1,0.96115) (H2,1.02541) (H3,0.95902) (HL0,0.96742) (HL1,0.93518) (HL2,0.93425) (HL3,0.97972) (HM0,0.95420) (HM1,0.91141) (HM2,0.95091) (HM3,0.90759) (HML0,0.92329) (HML1,1.05726) (HML2,1.00110) (HML3,0.91277) (L0,0.99309) (L1,1.01000) (L2,0.99666) (L3,0.99093) (M0,0.94656) (M1,0.94500) (M2,0.93227) (M3,0.92822) (ML0,0.99327) (ML1,0.94123) (ML2,0.96814) (ML3,0.97232) (GMEAN,0.96288)(HIGH,0.9812070868)(H+HM,0.9556592286)(H+HM+HML,0.9610184892)(SomeH,0.9592427796)};
				\addplot [LineFillYellowTiny]coordinates {(H0,0.98067) (H1,0.96115) (H2,1.02541) (H3,0.95902) (HL0,0.96742) (HL1,0.93518) (HL2,0.93425) (HL3,0.97972) (HM0,0.95420) (HM1,0.91141) (HM2,0.95091) (HM3,0.90759) (HML0,0.92329) (HML1,1.05726) (HML2,1.00110) (HML3,0.91277) (L0,0.99309) (L1,1.01000) (L2,0.99666) (L3,0.99093) (M0,0.94656) (M1,0.94500) (M2,0.93227) (M3,0.92822) (ML0,0.99327) (ML1,0.94123) (ML2,0.96814) (ML3,0.97232) (AVG,0.96354)(HIGH,0.9815644112)(H+HM,0.9562958033)(H+HM+HML,0.9620651728)(SomeH,0.9600845497)};
			%	\addplot [LineFillBlueTiny]coordinates {(H0,0.89106) (H1,0.82888) (H2,0.95308) (H3,0.80582) (HL0,0.82821) (HL1,0.93045) (HL2,0.92296) (HL3,0.95524) (HM0,0.89701) (HM1,0.90170) (HM2,0.91325) (HM3,0.88014) (HML0,0.88605) (HML1,0.92404) (HML2,0.91423) (HML3,0.89445) (L0,0.99621) (L1,1.01001) (L2,1.00626) (L3,0.98529) (M0,0.93279) (M1,0.93661) (M2,0.92889) (M3,0.88962) (ML0,0.99383) (ML1,0.92905) (ML2,0.96074) (ML3,0.97624) (GMEAN,0.92254)(HIGH,0.8678410022)(H+HM,0.8827655468)(H+HM+HL,0.8899735887)(SomeH,0.8944188932)};RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.93343) (H1,0.90130) (H2,0.93858) (H3,0.89515) (HL0,0.95930) (HL1,0.93022) (HL2,0.93002) (HL3,0.96277) (HM0,0.88468) (HM1,0.90849) (HM2,0.91329) (HM3,0.84809) (HML0,0.85364) (HML1,0.91518) (HML2,0.91646) (HML3,0.89403) (L0,0.99514) (L1,1.01285) (L2,1.00605) (L3,0.98672) (M0,0.93648) (M1,0.93377) (M2,0.91949) (M3,0.90127) (ML0,0.99217) (ML1,0.93551) (ML2,0.96345) (ML3,0.97095) (GMEAN,0.93259)(HIGH,0.9169164575)(H+HM,0.9024742951)(H+HM+HL,0.8997955821)(SomeH,0.9109981829)}; RD 0.5x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.92245) (H1,0.90493) (H2,0.94353) (H3,0.89959) (HL0,0.96900) (HL1,0.93029) (HL2,0.93999) (HL3,0.97020) (HM0,0.90369) (HM1,0.91889) (HM2,0.92880) (HM3,0.84714) (HML0,0.85749) (HML1,0.91919) (HML2,0.91501) (HML3,0.90047) (L0,0.99455) (L1,1.01555) (L2,1.01406) (L3,0.99095) (M0,0.94716) (M1,0.93216) (M2,0.92278) (M3,0.91284) (ML0,0.99567) (ML1,0.93940) (ML2,0.96338) (ML3,0.97404) (GMEAN,0.93742)(HIGH,0.9174632506)(H+HM,0.908215995)(H+HM+HML,0.9046974843)(SomeH,0.9163484201)};%RD 0.25x
			\addplot [LineFillBlueTiny]coordinates {(H0,0.92245) (H1,0.90493) (H2,0.94353) (H3,0.89959) (HL0,0.96900) (HL1,0.93029) (HL2,0.93999) (HL3,0.97020) (HM0,0.90369) (HM1,0.91889) (HM2,0.92880) (HM3,0.84714) (HML0,0.85749) (HML1,0.91919) (HML2,0.91501) (HML3,0.90047) (L0,0.99455) (L1,1.01555) (L2,1.01406) (L3,0.99095) (M0,0.94716) (M1,0.93216) (M2,0.92278) (M3,0.91284) (ML0,0.99567) (ML1,0.93940) (ML2,0.96338) (ML3,0.97404) (AVG,0.93833)(HIGH,0.9176232027)(H+HM,0.9086260532)(H+HM+HML,0.9050970236)(SomeH,0.9169156767)};%RD 0.25x
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Energy consumption in the DRAM normalized to the baseline in the 4-core CMP system.}
\label{fig:energy_dram_mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Discussion}
\label{subsubsec:disc_mc}

For the sake of clarity, we next explain where the performance improvements of our technique come from. First, as Figure~\ref{fig:writes_mc} illustrated earlier, the write reductions to the SLLC that RD achieves are greater than those of DASCA. Second, and more importantly, as Figure~\ref{fig:perf_mc} reveals, the bypasses dictated by RD translate into more performance than that of DASCA. As in the single-core scenario, the rationale behind that is related with the hit rate experimented in the SLLC with both schemes. Figure~\ref{fig:hits_mc} illustrates the number of hits in the SLLC per kilo instruction that each mix experiments normalized to the baseline. 
%(it is worth noting that we conservatively show in this case the geomean considering all mixes instead the arithmetic mean to avoid a biased number due to the significantly high write reduction capability that our RD exhibits when running H1 and H3 mixes).


\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.8,
				%ymax=2.2,
				ymax=1.85,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,0.98)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				\addplot [LineFillYellowTiny]coordinates {(H0,0.98) (H1,1.18) (H2,0.94) (H3,1.31) (HL0,1.22) (HL1,0.99) (HL2,1.15) (HL3,0.96) (HM0,1.04) (HM1,0.99) (HM2,1.01) (HM3,1.17) (HML0,1.06) (HML1,0.84) (HML2,0.92) (HML3,1.19) (L0,1.07) (L1,0.98) (L2,1.02) (L3,0.98) (M0,1.02541) (M1,1.06) (M2,1.02) (M3,1.05) (ML0,0.99) (ML1,1.01) (ML2,1.00) (ML3,1.02544) (AVG,1.04174)(HIGH,1.1021036697)(H+HM,1.0777998935)(H+HM+HML,1.0525045951)(SomeH,1.0591338236)};
%				\addplot [LineFillBlueTiny]coordinates {(H0,1.03) (H1,4.39) (H2,1.02) (H3,4.94) (HL0,2.88) (HL1,1.00) (HL2,1.34) (HL3,1.19) (HM0,1.27) (HM1,1.00) (HM2,1.17) (HM3,1.30) (HML0,1.33) (HML1,1.06) (HML2,1.12) (HML3,1.27) (L0,1.06) (L1,1.01) (L2,1.04) (L3,1.00) (M0,1.03253) (M1,1.08) (M2,1.04) (M3,1.16) (ML0,1.01) (ML1,1.02) (ML2,1.06) (ML3,1.01669) (GMEAN,1.26)(HIGH,2.1848032713)(H+HM,1.604367847)(H+HM+HL,1.4522378495)(SomeH,1.4549394302)}; RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,1.02) (H1,2.63) (H2,1.01) (H3,2.98) (HL0,1.24) (HL1,1.00) (HL2,1.11) (HL3,1.17) (HM0,1.23) (HM1,0.99) (HM2,1.08) (HM3,1.34) (HML0,1.33) (HML1,1.03) (HML2,1.04) (HML3,1.24) (L0,0.97) (L1,1.00) (L2,1.02) (L3,0.99) (M0,1.03) (M1,1.07) (M2,1.04) (M3,1.10) (ML0,0.97) (ML1,1.00) (ML2,0.99) (ML3,1.02) (GMEAN,1.15)(HIGH,1.6870853325)(H+HM,1.3943098745)(H+HM+HL,1.3089349484)(SomeH,1.2608045584)}; RD 0.5x
				\addplot [LineFillBlueTiny]coordinates {(H0,1.01) (H1,2.47) (H2,1.01) (H3,2.85) (HL0,1.20) (HL1,1.00) (HL2,1.37) (HL3,1.16) (HM0,1.24) (HM1,1.03) (HM2,1.10) (HM3,1.32) (HML0,1.29) (HML1,1.01) (HML2,1.03) (HML3,1.21) (L0,1.05) (L1,1.07) (L2,1.00) (L3,1.01) (M0,1.02) (M1,1.05) (M2,1.03) (M3,1.07) (ML0,0.98) (ML1,1.02) (ML2,1.02) (ML3,1.09) (AVG,1.20431)(HIGH,1.8335583878)(H+HM,1.5032311204)(H+HM+HML,1.381065675)(SomeH,1.3308892183)}; %RD 0.25x
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Number of STT-RAM SLLC hits per kilo instruction normalized to the baseline in the 4-core CMP system.}
\label{fig:hits_mc}
\end{figure*}

The results reveal that in most of the mixes evaluated the amount of hits in the SLLC is higher under our approach than using DASCA. Again, this is especially evident for the case of the mixes including write-intensive applications such as H1, H3 and HL2 where the number of hits is 2.87x, 2.45x and 1.37x those of the baseline, respectively. This is the key to explain our performance improvements: the efficient management of the SLLC contents by exploiting the reuse locality. In addition, there are other factors that also contribute to the throughput gain such as less write operations to the SLLC, less main memory accesses, and increased row buffer hit rates. In order to perform a deeper comparison between RD and DASCA, Table~\ref{tab:comp} recaps the average values of different metrics involved in the performance delivered by RD and DASCA, normalized to those of the baseline. As shown, our scheme improves DASCA and the baseline (especially in the data from write-intensive mixes) in all the metrics considered.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}
	\begin{center}
		%\scriptsize
		%tiny
		\tbl{Average values of different metrics normalized to the baseline in the 4-core CMP system.\label{tab:comp}}{ 
		\resizebox{0.8\textwidth}{!}{%	
		%\begin{tabular}{|c|c|c|c|c|c|c|}
		\begin{tabular}{|l|C{3.5em}|C{3.5em}|C{7.5em}|C{3.5em}|C{3.5em}|C{8.5em}|}
			\hline
			 \backslashbox{\textbf{Policies}}{\textbf{Metrics}}&\textbf{SLLC Misses}&\textbf{SLLC Hits}&\textbf{Row buffer Read Hit Rate}&\textbf{DRAM reads}&\textbf{DRAM Writes}&\textbf{Bank contention in SLLC}\\
			%\textbf{LLC Misses}&\textbf{LLC Hits}&\textbf{LLC MR}&\textbf{RB RHR}&\textbf{RB WHR}&\textbf{DRAM Reads}&\textbf{DRAM Writes}\\
			%\hline
				\hline
				\textbf{DASCA (All/High)} & 1.01/1.05 & 1.04/1.10 & 1.03/1.00 & 1.01/1.05 & 1.04/1.06 & 0.45/0.16\\
				\hline
				%\textbf{DASCA (High)} & 1.05 & 1.09 & 1.00 & 1.05 & 1.06 & 0.15\\
				%\hline
				%\textbf{RD (All/High)} & 0.93/0.92 & 1.26/2.18 & 1.05/1.07 & 0.95/0.92 & 0.95/0.89 & 0.32/0.15\\ %RD 1x
				%\textbf{RD (All/High)} & 0.94/0.95 & 1.15/1.69 & 1.04/1.01 & 0.97/0.96 & 0.95/0.94 & 0.25/0.09\\ %RD 0.5x
				\textbf{RD (All/High)} & 0.94/0.95 & 1.20/1.83 & 1.05/1.01 & 0.98/0.98 & 0.96/0.94 & 0.29/0.08\\ %RD 0.25x
				\hline
			    %\textbf{RD (High)} & 0.92 & 2.18 & 1.07 & 0.92 & 0.89 & 0.15\\
				%\hline
		\end{tabular}}}
	\end{center}
\end{table*}

As in the single-core scenario, next we zoom into particular mixes that need further detail to get a better understanding. First, in some mixes such as H0, HM3 or HML0 we can observe that the DASCA scheme is able to reduce the amount of writes to the SLLC and also the energy consumption in the STT-RAM more than our scheme does (Figures~\ref{fig:writes_mc} and \ref{fig:energy_mc}). Conversely, the RD manages to deliver more throughput than DASCA (Figure~\ref{fig:perf_mc}). However, these performance improvements our approach achieves are not enough to offset the higher energy savings in the SLLC that the DASCA scheme reports for these mixes as a consequence of the lower number of writes to the STT-RAM. 
%Although for mix HM3, as shown in Figure~\ref{fig:energy_break_mc}, the RD manages to reduce the \emph{static} energy consumption of the SLLC by 20\% with respect to the baseline --due to the higher throughput delivered-- and DASCA just reaches 5\%, the \emph{dynamic} energy consumption the RD manages to reduce is just 11\% vs 19\% of DASCA. Although the difference between the numbers achieved by both policies is greater in the case of the static contribution and favorable to our approach, the net result is more favorable to DASCA for this mix due to the higher weight that the dynamic part has in this mix as shown in Figure~\ref{fig:energy_llc_break}. However, the RD allows to report much higher energy savings in the DRAM main memory (19\% vs 2\% of DASCA) due to the high performance improvement already mentioned and to the higher impact the leakage currents has over DRAM technology compared to STT-RAM.



Second, data for mix L2 reveal that the RD is able to reduce the amount of writes to the SLLC much more than DASCA with respect to the baseline (81\% vs. 48\%). However, this great difference translates into just 22\% of energy savings in RD vs. 13\% of DASCA. As shown, the difference between both policies has been significantly reduced due to the low contribution of the dynamic energy to the total energy consumption in the SLLC that this mix exhibits, as Figure~\ref{fig:energy_llc_break} illustrates.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Second, as shown in Figure~\ref{fig:perf_mc}, the RD delivers significantly higher performance than DASCA. Although it was explained earlier that this improvement comes from the higher number of hits, there are other factors that also contribute to the gain such as less write operations to the SLLC, less main memory accesses, and increased row buffer hit rates. 


%Notably, there are some mixes like H3, HL3, HM1 or HM3, where the RD achieves a very significant throughput improvement with respect to the  baseline (15-25\% and up to 47\%) and also compared to DASCA. In all these mixes but HM3 --as already stated before-- our approach manages to slightly reduce the number of the long and power-hungry writes to the SLLC to a greater extent than DASCA. As evident, this fact in isolation can not justify the performance improvements obtained. But if we deep into detail our data reveal that the miss rate in the SLLC  that our approach exhibits is much lower (39\% in mix HM3 or 9\% in H3) than in the DASCA scheme. In addition, the total amount of misses in the LLC is also much lower with our RD than in DASCA (33\% in mix HM3 or or 10\% in H3) and the number of hits in the LLC is higher too (for example, 10\% higher in mix HM3). Furthermore, in all these four mixes the main memory accesses are significantly lower than in DASCA and the row buffer (RB) hit rates (both read and write) are moderately higher in our scheme than in DASCA and much higher than in the baseline. And last but not least, as a side-effect of the new SLLC management, the miss rate in the private L1 caches is also get reduced moderately for some mixes. Notably, mix HM1 and mix HL3 using our RD reports respectively 7.5\% and 6\% lower miss rate in the L1s than the baseline, vs the 1.5\% and 3\% lower miss rate of DASCA. 

%In order to a deeper comparison between our proposal and DASCA, Table~\ref{tab:comp} recaps the average values of different metrics involved in performance that our Reuse Detector and the DASCA scheme report normalized to those of the baseline. As shown our scheme improves DASCA and the baseline (especially in the data from write-intensive mixes) in all the metrics considered.



\subsubsection{Sensitivity to Reuse Detector size}
\label{subsubsec:sense}

%One key aspect in designing the Reuse Detector is to decide the \emph{expulsion coverage} it provides. In other words, the RD size is an important issue in the implementation of our proposal.
The RD size is a key design aspect of our proposal.  
In order to evaluate its impact we show in Figure~\ref{fig:sense_sc} the amount of writes to the SLLC, the Instruction Throughput, 
%the amount of hits in the SLLC, 
and the energy consumption in both the SLLC and the main memory for different RD sizes per core, namely 8K, 16K, 32K and 64K entries. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Sensibilidad a tamaño detector reuso
\begin{figure*}
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=40em,
				ybar, 
				ymin=0.3,
				ymax=1.2,
				enlargelimits=0.1, 
				legend style={font=\scriptsize,at={(0.5,1)}, 
				anchor=north,legend columns=8}, 
				%symbolic x coords={Writes LLC,IT,Hits LLC,Eng. STT-RAM,Eng. DRAM}, 
				symbolic x coords={Writes SLLC,IT,Eng. SLLC,Eng. DRAM}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize},
				bar width=0.5em,
				ymajorgrids,
				]
				%\addplot [LineFillRedTiny]coordinates {(Writes LLC,0.26170) (IT,1.02907) (Hits LLC,1.16) (Eng. STT-RAM,0.72576) (Eng. DRAM,0.93742)}; %0.25x all
				%\addplot [LineFillBlueTiny]coordinates {(Writes LLC,0.29273) (IT,1.03075) (Hits LLC,1.15) (Eng. STT-RAM,0.72576) (Eng. DRAM,0.93259)}; %0.5x all
				%\addplot [LineFillGreenTiny]coordinates {(Writes LLC,0.36722) (IT,1.03757) (Hits LLC,1.26) (Eng. STT-RAM,0.75044) (Eng. DRAM,0.92254)}; %1x all
				%\addplot [LineFillYellowTiny]coordinates {(Writes LLC,0.43867) (IT,1.03164) (Hits LLC,1.26) (Eng. STT-RAM,0.77430) (Eng. DRAM,0.93060)}; %2x all
				%\addplot [LineFillOrangeTiny]coordinates {(Writes LLC,0.2263099303) (IT,1.0711356597) (Hits LLC,1.6356428123) (Eng. STT-RAM,0.6263528984) (Eng. DRAM,0.9174632506)}; %0.25x high
				%\addplot [LineFillTurquoiseTiny]coordinates {(Writes LLC,0.2512276929) (IT,1.0617592884) (Hits LLC,1.6870853325) (Eng. STT-RAM,0.6263528984) (Eng. DRAM,0.9169164575)}; %0.5x high
				%\addplot [LineFillPurpleTiny]coordinates {(Writes LLC,0.3461276381) (IT,1.1038163119) (Hits LLC,2.1848032713) (Eng. STT-RAM,0.6548887237) (Eng. DRAM,0.8678410022)}; %1x high
				%\addplot [LineFillBrownTiny]coordinates {(Writes LLC,0.408131851) (IT,1.0911438469) (Hits LLC,2.1098386489) (Eng. STT-RAM,0.6839962457) (Eng. DRAM,0.885798249)}; %2x high

				%\addplot [LineFillRedTiny2]coordinates {(Writes SLLC,0.26170) (IT,1.02907) (Eng. SLLC,0.72576) (Eng. DRAM,0.93742)}; %0.25x all
				%\addplot [LineFillBlueTiny2]coordinates {(Writes SLLC,0.29273) (IT,1.03075) (Eng. SLLC,0.72576) (Eng. DRAM,0.93259)}; %0.5x all
				%\addplot [LineFillGreenTiny2]coordinates {(Writes SLLC,0.36722) (IT,1.03757) (Eng. SLLC,0.75044) (Eng. DRAM,0.92254)}; %1x all
				%\addplot [LineFillYellowTiny2]coordinates {(Writes SLLC,0.43867) (IT,1.03164) (Eng. SLLC,0.77430) (Eng. DRAM,0.93060)}; %2x all
				%\addplot [LineFillRedTiny3]coordinates {(Writes SLLC,0.2263099303) (IT,1.0711356597) (Eng. SLLC,0.6263528984) (Eng. DRAM,0.9174632506)}; %0.25x high
				%\addplot [LineFillBlueTiny3]coordinates {(Writes SLLC,0.2512276929) (IT,1.0617592884) (Eng. SLLC,0.6263528984) (Eng. DRAM,0.9169164575)}; %0.5x high
				%\addplot [LineFillGreenTiny3]coordinates {(Writes SLLC,0.3461276381) (IT,1.1038163119) (Eng. SLLC,0.6548887237) (Eng. DRAM,0.8678410022)}; %1x high
				%\addplot [LineFillYellowTiny3]coordinates {(Writes SLLC,0.408131851) (IT,1.0911438469) (Eng. SLLC,0.6839962457) (Eng. DRAM,0.885798249)}; %2x high
				%\addplot [LineFillRedTiny2]coordinates {(Writes SLLC,0.26170) (IT,1.02907) (Eng. SLLC,0.59910) (Eng. DRAM,0.93742)}; %0.25x all nueva celda
				%\addplot [LineFillBlueTiny2]coordinates {(Writes SLLC,0.29273) (IT,1.03075) (Eng. SLLC,0.60481) (Eng. DRAM,0.93259)}; %0.5x all nueva celda
				%\addplot [LineFillGreenTiny2]coordinates {(Writes SLLC,0.36722) (IT,1.03757) (Eng. SLLC,0.63815) (Eng. DRAM,0.92254)}; %1x all nueva celda
				%\addplot [LineFillYellowTiny2]coordinates {(Writes SLLC,0.43867) (IT,1.03164) (Eng. SLLC,0.67351) (Eng. DRAM,0.93060)}; %2x all nueva celda
				%\addplot [LineFillRedTiny3]coordinates {(Writes SLLC,0.2263099303) (IT,1.0711356597) (Eng. SLLC,0.5048902032) (Eng. DRAM,0.9174632506)}; %0.25x high nueva celda
				%\addplot [LineFillBlueTiny3]coordinates {(Writes SLLC,0.2512276929) (IT,1.0617592884) (Eng. SLLC,0.5141259921) (Eng. DRAM,0.9169164575)}; %0.5x high nueva celda
				%\addplot [LineFillGreenTiny3]coordinates {(Writes SLLC,0.3461276381) (IT,1.1038163119) (Eng. SLLC,0.5511938968) (Eng. DRAM,0.8678410022)}; %1x high nueva celda
				%\addplot [LineFillYellowTiny3]coordinates {(Writes SLLC,0.408131851) (IT,1.0911438469) (Eng. SLLC,0.5898149934) (Eng. DRAM,0.885798249)}; %2x high nueva celda
				\addplot [LineFillRedTiny2]coordinates {(Writes SLLC,0.37310) (IT,1.02907) (Eng. SLLC,0.62993) (Eng. DRAM,0.93833)}; %0.25x all nueva celda
				\addplot [LineFillBlueTiny2]coordinates {(Writes SLLC,0.38373) (IT,1.03075) (Eng. SLLC,0.63288) (Eng. DRAM,0.93352)}; %0.5x all nueva celda
				\addplot [LineFillGreenTiny2]coordinates {(Writes SLLC,0.43431) (IT,1.03757) (Eng. SLLC,0.66182) (Eng. DRAM,0.92400)}; %1x all nueva celda
				\addplot [LineFillYellowTiny2]coordinates {(Writes SLLC,0.49340) (IT,1.03164) (Eng. SLLC,0.69414) (Eng. DRAM,0.93181)}; %2x all nueva celda
				\addplot [LineFillRedTiny3]coordinates {(Writes SLLC,0.4011467998) (IT,1.0711356597) (Eng. SLLC,0.5572038011) (Eng. DRAM,0.9176232027)}; %0.25x high nueva celda
				\addplot [LineFillBlueTiny3]coordinates {(Writes SLLC,0.4098223232) (IT,1.0617592884) (Eng. SLLC,0.5636516459) (Eng. DRAM,0.9171154268)}; %0.5x high nueva celda
				\addplot [LineFillGreenTiny3]coordinates {(Writes SLLC,0.4551618405) (IT,1.1038163119) (Eng. SLLC,0.5920286028) (Eng. DRAM,0.8697073801)}; %1x high nueva celda
				\addplot [LineFillYellowTiny3]coordinates {(Writes SLLC,0.4997198361) (IT,1.0911438469) (Eng. SLLC,0.6258035081) (Eng. DRAM,0.8875098742)}; %2x high nueva celda
				%\legend{32-All,64K-All,128K-All,256K-All,32K-High,64K-High,128K-High,256K-High} 
				\legend{8K-All,16K-All,32-All,64K-All,8K-High,16K-High,32K-High,64K-High} 
			\end{axis}
		\end{tikzpicture}	
%\caption{Writes to LLC, IT, amount of hits in the SLLC, and energy consumption in both SLLC and main memory normalized to the baseline for different RD sizes.}
\caption{Writes to SLLC, IT and energy consumption in both SLLC and main memory normalized to the baseline for different RD sizes per core in the 4-core CMP system.}
\label{fig:sense_sc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As shown, the major impact is observed on the capability to reduce the number of writes in the SLLC, ranging from an average reduction of 63\% with respect to the baseline when an 8K-entry RD per core is employed (60\% for the write-intensive mixes) to a reduction of around 51\% for a 64K-entry RD per core (50\% for the \emph{high mixes}). Note that maybe these data might appear contradictory at first sight. However, they are not: As the size of RD increases, it also augments the probability that a block finds its tag in the RD, so the probability of bypassing decreases, leading to minor reduction of writes to the SLLC. We can also observe a moderate impact on the average energy consumed in the SLLC, with values in the range 63-69\% as the size of RD gets increased: again, note that these numbers follow a similar trend to that exhibited by the amount of writes. Finally, the impact over the performance and the energy consumption of the main memory is much reduced, falling the average IT variations into a small range of 1\% (4\% for the write-intensive mixes) and the average DRAM energy variations into a range of 1.5\% (5\% for the write-intensive mixes). 

\subsubsection{Overhead analysis}
\label{subsubsec:overhead}

In Section~\ref{subsubsec:details} we outlined that an 8K-entry RD for a 1MB LLC requires an extra storage of 14KB, which represents a 1.37\% overhead with respect to the LLC size. In this section we previously noted that for the 4-CMP system under evaluation (4MB SLLC) we employ an 8K-entry RD per core. The reason is that we are maintaining for each evaluated system the 1.37\% overhead with respect the SLLC size. 
%Note also that although the RD is a monolithic element (blocks evicted from any L2 private cache access it), actually the amount of entries in the RD is limited for each core. 
%Thus, in the 32K-entry RD used in the 4-CMP system each core has 8K entries available. 
Therefore, in the 8-CMP evaluated later, we also employ an 8K-entry RD per core. Hence, the total extra storage (overhead) of RD is 56KB and 112KB for the 4-CMP and 8-CMP systems respectively, representing in all the cases a 1.37\% overhead with respect to the SLLC size.    

\subsubsection{RD in a two-level cache hierarchy}
\label{subsubsec:2_levels}

We have evaluated the operation of our proposal in a three-level cache hierarchy since most current processors employ this configuration. Furthermore, two private levels are more likely to filter better the temporal locality than using just one private level. However, for a fair comparison, we have also evaluated our proposal and the DASCA scheme in a configuration with just two cache levels. Notably, we reproduce the same configuration (4-CMP) used by the authors in~\cite{dasca_14} when presenting the DASCA technique (32 KB IL1 and DL1 as private caches and a 1MB per core shared L2 cache). Table~\ref{tab:2levels} illustrates the main results. 



\begin{table*}
	\begin{center}
		%\scriptsize
		%tiny
		\tbl{Average values of different metrics normalized to the baseline\label{tab:2levels} in a 4-core CMP system with two cache levels.}{ 
		\resizebox{0.8\textwidth}{!}{%	
		%\begin{tabular}{|c|c|c|c|c|c|c|}
		\begin{tabular}{|l|C{3.5em}|C{7em}|C{8em}|C{8em}|C{3.5em}|}
			\hline
			 \backslashbox{\textbf{Policies}}{\textbf{Metrics}}&\textbf{Writes SLLC}&\textbf{Instr. Throughput}&\textbf{Energy consumpt. SLLC}&\textbf{Energy consumpt. DRAM}&\textbf{SLLC Hits}\\
				\hline
				\textbf{DASCA (All/High)} & 0.70/0.79 & 1.01/1.03 & 0.81/0.86 & 0.97/0.96 & 0.98/1.00\\
				\hline
				%\textbf{RD (All/High)} & 0.61/0.78 & 1.03/1.07 & 0.81/0.88 & 0.93/0.90 & 1.00/1.01\\ 1x
				\textbf{RD (All/High)} & 0.59/0.76 & 1.03/1.04 & 0.75/0.83 & 0.95/0.95 & 0.98/1.00\\ %0.25x
				\hline
		\end{tabular}}}
	\end{center}
\end{table*}

As shown, RD maintains higher capability than DASCA (around 11\% higher) in reducing the amount of writes to the SLLC. However, as expected, the amount of writes avoided (and also the hits experienced in the SLLC) is significantly lower than that exhibited in an scenario with 3 cache levels. Recall that this is due to the fact that with two cache levels only, most temporal locality has not been filtered, so that the reuse locality can not be fully exploitable. Also, as a consequence of this lower capability in cutting the write traffic to the SLLC, the energy savings achieved in the shared L2 are significantly lower than those obtained with three cache levels, although RD still reports better numbers than DASCA. Finally, RD again improves the Instruction Throughput to a greater extent than DASCA, and consequently also delivers higher energy savings in the main memory. Note that we have also evaluated 28 mixes in this configuration following the same criteria explained earlier, but they are not exactly the same as in the three-level cache hierarchy experiments since the WPKI values that the benchmarks exhibit do not match those of the three-level configuration and therefore some programs changed the category (high, medium or low) in which they were classified. 

%Note also that the hits observed in the SLLC under our proposal exhibit the lower values (although higher than DASCA) among all the configurations evaluated. This is due to the fact that, with just two cache levels, most temporal locality has not been filtered, so that the reuse locality is not plenty exploitable.




\subsection{Evaluation in an 8-core CMP system}
\label{subsec:8_mc}

In this section we illustrate and analyze the main results obtained when using RD and DASCA in an 8-core CMP system with an 8MB SLLC. Like in the previous section, in this scenario we create 28 mixes following the same criteria as in a 4-CMP system. The mixes evaluated are shown in Table~\ref{tab:mix8C}. %In this section we will not zoom into the details as we did in the previous section (Section~\ref{subsec:mc}), but will only describe the average results and main trends. 
Given that a detailed analysis of the 8-core system would show similar results as the 4-core scenario, in this section we will not zoom into details but will only describe the average results and main trends.

%In this environment we again made up 28 mixes following the same criteria as with a 4-CMP system. The mixes evaluated are shown in Table~\ref{tab:mix8C}.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%For the sake of brevity, and as the behavior observed is analogous to that of a 4-CMP system, the primary results are recap in Table~\ref{tab:8C}. As shown, the ability to reduce the amount of writes to the SLLC is again moderately higher with our proposal (around 59/44\% write reduction with respect to the baseline, 11/8\% less writes performed than with DASCA, for all mixes and write-intensive mixes, respectively) and the energy consumption is around 65\% of the baseline (6\% lower than that of DASCA). In both cases (amount of writes and energy consumption), the average values of both RD and DASCA are slightly higher than in the case of a 4-CMP system. The main reason for lower energy savings in the SLLC is that, apart from lower write reduction, in an 8-CMP system the static contribution to the total energy consumption in the SLLC is on average slightly higher for the mixes evaluated than in the case of a system with only four cores. As a result, the dynamic part, although still dominant, is lower and the net energy savings also are lower. However, performance improves more than in the 4-core CMP: RD achieves a 7\% increase in IT for all mixes (20\% for the \emph{high} mixes) with respect to the baseline system, whereas DASCA stays behind reporting 4\% and 11\% respectively. Moreover, RD also reports much better numbers for the DRAM energy consumption than DASCA. These results confirm those obtained with 4 cores, in the sense that RD is able to significantly reduce the amount of writes to the SLLC to a greater extent than DASCA, to deliver significantly more performance than DASCA and also to report higher energy savings (both in the SLLC and the main memory), which translates into significant energy consumption reduction in the overall system, since main memory consumption is around 59x and 26x that of the SLLC for the 4-CMP and 8-CMP systems respectively.   


%\begin{table*}
%	\begin{center}
%		%\scriptsize
%		%tiny
%		\tbl{Average (geomean) values of different metrics normalized to the baseline\label{tab:8C} in a 8-core CMP system.}{ 
%		\resizebox{0.8\textwidth}{!}{%	
%		%\begin{tabular}{|c|c|c|c|c|c|c|}
%		\begin{tabular}{|l|C{3.5em}|C{7em}|C{8em}|C{8em}|C{3.5em}|}
%			\hline
%			 \backslashbox{\textbf{Policies}}{\textbf{Metrics}}&\textbf{Writes SLLC}&\textbf{Instr. Throughput}&\textbf{Energy consumpt. SLLC}&\textbf{Energy consumpt. DRAM}&\textbf{Hits SLLC}\\
%				\hline
%				\textbf{DASCA (All/High)} & 0.52/0.64 & 1.04/1.11 & 0.71/0.72 & 0.97/1.06 & 0.92/0.84\\
%				\hline
%				%\textbf{RD (All/High)} & 0.55/0.61 & 1.08/1.22 & 0.83/0.77 & 0.91/0.90 & 1.12/1.03\\1x
%				\textbf{RD (All/High)} & 0.41/0.56 & 1.07/1.20 & 0.65/0.66 & 0.93/0.97 & 1.05/1.01\\%0.125x
%				\hline
%		\end{tabular}}}
%	\end{center}
%\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%De la tesis de Roberto
\subsubsection{Write filtering}
\label{subsubsec:wr_8mc}

Figure~\ref{fig:writes_8mc} illustrates the number of writes to the STT-RAM SLLC generated with DASCA and with RD (assuming an 8K-entry RD per core). Both schemes are normalized to a baseline STT-RAM without any content selection mechanism. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Writes mc
\begin{figure*}[htb]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=38em,
				ybar, 
				ymin=0.05,
				ymax=0.87,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.3)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH}, 
				xtick=data, 
 			    x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				%\addplot [LineFillRedTiny]coordinates {(H0,) (H1,) (H2,) (H3,) (HL0,) (HL1,) (HL2,) (HL3,) (HM0,) (HM1,) (HM2,) (HM3,) (HML0,) (HML1,) (HML2,) (HML3,) (L0,) (L1,) (L2,) (L3,) (M0,) (M1,) (M2,) (M3,) (ML0,) (ML1,) (ML2,) (ML3,) (GMEAN,)(HIGH,)(H+HM,)(H+HM+HML,)(SomeH,)};
				%\addplot [LineFillYellowTiny]coordinates {(H0,0.67) (H1,0.61) (H2,0.66) (H3,0.66) (HL0,0.75) (HL1,0.40) (HL2,0.79) (HL3,0.18) (HM0,0.62) (HM1,0.36) (HM2,0.68) (HM3,0.20) (HML0,0.20) (HML1,0.74) (HML2,0.37) (HML3,0.44) (L0,0.80) (L1,0.79) (L2,0.77) (L3,0.78) (M0,0.49) (M1,0.47) (M2,0.57) (M3,0.34) (ML0,0.60) (ML1,0.57) (ML2,0.59) (ML3,0.66) (GMEAN,0.52) (HIGH,0.65) (H+HM,0.52) (H+HM+HML,0.47) (SomeH,0.47)};
				\addplot [LineFillYellowTiny]coordinates {(H0,0.67) (H1,0.61) (H2,0.66) (H3,0.66) (HL0,0.75) (HL1,0.40) (HL2,0.79) (HL3,0.18) (HM0,0.62) (HM1,0.36) (HM2,0.68) (HM3,0.20) (HML0,0.20) (HML1,0.74) (HML2,0.37) (HML3,0.44) (L0,0.80) (L1,0.79) (L2,0.77) (L3,0.78) (M0,0.49) (M1,0.47) (M2,0.57) (M3,0.34) (ML0,0.60) (ML1,0.57) (ML2,0.59) (ML3,0.66) (AVG,0.56243) (HIGH,0.6474175022) (H+HM,0.5557289061) (H+HM+HML,0.5156605129) (SomeH,0.5200329168)};
%				\addplot [LineFillBlueTiny]coordinates {(H0,0.75) (H1,0.18) (H2,0.75) (H3,0.14) (HL0,0.11) (HL1,0.82) (HL2,0.15) (HL3,0.17) (HM0,0.32) (HM1,0.79) (HM2,0.25) (HM3,0.28) (HML0,0.42) (HML1,0.50) (HML2,0.32) (HML3,0.17) (L0,0.21) (L1,0.78) (L2,0.36) (L3,0.60) (M0,0.58) (M1,0.41) (M2,0.71) (M3,0.37) (ML0,0.44) (ML1,0.68) (ML2,0.20) (ML3,0.69) (GMEAN,0.36722)(HIGH,0.3461276381)(H+HM,0.3561446329)(H+HM+HL,0.3457862128)(SomeH,0.3102827744)};  RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.74) (H1,0.09) (H2,0.73) (H3,0.08) (HL0,0.06) (HL1,0.82) (HL2,0.12) (HL3,0.09) (HM0,0.22) (HM1,0.78) (HM2,0.18) (HM3,0.25) (HML0,0.39) (HML1,0.45) (HML2,0.25) (HML3,0.12) (L0,0.13) (L1,0.76) (L2,0.27) (L3,0.59) (M0,0.52) (M1,0.31) (M2,0.66) (M3,0.27) (ML0,0.39) (ML1,0.67) (ML2,0.16) (ML3,0.64) (GMEAN,0.29273)(HIGH,0.2512276929)(H+HM,0.2737899067)(H+HM+HL,0.2732734405)(SomeH,0.2362530442)}; RD 0.5x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.57) (H1,0.52) (H2,0.58) (H3,0.56) (HL0,0.74) (HL1,0.21) (HL2,0.72) (HL3,0.07) (HM0,0.61) (HM1,0.26) (HM2,0.60) (HM3,0.17) (HML0,0.15) (HML1,0.76) (HML2,0.22) (HML3,0.26) (L0,0.61) (L1,0.54) (L2,0.60) (L3,0.55) (M0,0.44) (M1,0.38) (M2,0.54) (M3,0.35) (ML0,0.43) (ML1,0.44) (ML2,0.40) (ML3,0.58) (GMEAN,0.41) (HIGH,0.56) (H+HM,0.45) (H+HM+HML,0.38) (SomeH,0.36)}; %RD 0.25x
				\addplot [LineFillBlueTiny]coordinates {(H0,0.57) (H1,0.52) (H2,0.58) (H3,0.56) (HL0,0.74) (HL1,0.21) (HL2,0.72) (HL3,0.07) (HM0,0.61) (HM1,0.26) (HM2,0.60) (HM3,0.17) (HML0,0.15) (HML1,0.76) (HML2,0.22) (HML3,0.26) (L0,0.61) (L1,0.54) (L2,0.60) (L3,0.55) (M0,0.44) (M1,0.38) (M2,0.54) (M3,0.35) (ML0,0.43) (ML1,0.44) (ML2,0.40) (ML3,0.58) (AVG,0.46024) (HIGH,0.5577391169) (H+HM,0.4837609357) (H+HM+HML,0.4387748511) (SomeH,0.4381952736)}; %RD 0.25x
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Number of writes to the STT-RAM SLLC normalized to the baseline in the 8-core CMP system.}
\label{fig:writes_8mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The experimental results reveal that the RD and DASCA performs similarly in decreasing the amount of writes to the SLCC. Overall, our technique makes just around 36\% of the writes the baseline does, while DASCA performs around 40\%. These percentages decrease even slightly more for the mixes with write-intensive applications under both schemes. %Notably, in 21 out of 28 mixes evaluated the Reuse Detector exhibits higher ability in cutting the write traffic to the STT-RAM LLC.

Similarly to the results for the 4-core scenario, the experimental results reveal that RD just performs 46\% of the writes made in the baseline scheme, whereas DASCA produces 56\% of the writes that the baseline did. For the write-intensive mixes, RD and DASCA reduce the amount of writes compared to the baseline in 44\% and 35\% respectively.


\subsubsection{Performance}
\label{subsubsec:perf_8mc}

As we did in Section~\ref{subsubsec:perf_mc}, we employ the \emph{Instruction Throughput} (IT) to evaluate the performance when executing multiprogrammed workloads. Figure~\ref{fig:perf_8mc} illustrates the IT that each evaluated policy delivers normalized to the baseline. %Note that, unlike in the case of execution time metrics, now values higher than 1 imply performance improvements with respect to the baseline.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Throughput%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\begin{figure*}[htb]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=38em,
				ybar, 
				ymin=0.9,
				%ymax=1.14,
				ymax=1.30,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.3)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				\addplot [LineFillYellowTiny]coordinates {(H0,1.09) (H1,1.16) (H2,1.10) (H3,1.09) (HL0,1.02) (HL1,1.01) (HL2,1.02) (HL3,0.99) (HM0,1.19) (HM1,1.07) (HM2,1.08) (HM3,0.99) (HML0,1.00) (HML1,1.03) (HML2,0.99) (HML3,1.01) (L0,0.91) (L1,1.00) (L2,1.00) (L3,1.00) (M0,1.05) (M1,1.02) (M2,1.03) (M3,1.09) (ML0,1.12) (ML1,1.01) (ML2,1.01) (ML3,1.00) (GMEAN,1.04) (HIGH,1.11) (H+HM,1.10) (H+HM+HML,1.07) (SomeH,1.05)};
			%	\addplot [LineFillBlueTiny]coordinates {(H0,1.05825) (H1,1.13895) (H2,1.05085) (H3,1.17208) (HL0,1.12582) (HL1,1.01302) (HL2,1.02099) (HL3,1.01339) (HM0,1.05904) (HM1,1.02530) (HM2,1.04997) (HM3,1.06787) (HML0,1.06060) (HML1,1.02984) (HML2,1.03786) (HML3,1.03155) (L0,1.00066) (L1,0.99689) (L2,0.99846) (L3,0.99930) (M0,1.02746) (M1,1.02408) (M2,1.03079) (M3,1.06066) (ML0,0.99873) (ML1,1.01980) (ML2,0.96218) (ML3,1.00374) (GMEAN,1.03757)(HIGH,1.1038163119)(H+HM,1.0767902358)(H+HM+HL,1.0643475087)(SomeH,1.0587793992)}; RD 1x
			%	\addplot [LineFillBlueTiny]coordinates {(H0,1.04036) (H1,1.07012) (H2,1.05262) (H3,1.08448) (HL0,1.02299) (HL1,1.01318) (HL2,1.01933) (HL3,1.00816) (HM0,1.06447) (HM1,1.02202) (HM2,1.04654) (HM3,1.08542) (HML0,1.07735) (HML1,1.03366) (HML2,1.03547) (HML3,1.03193) (L0,1.00148) (L1,0.99579) (L2,0.99802) (L3,0.99956) (M0,1.02435) (M1,1.02223) (M2,1.03526) (M3,1.05505) (ML0,0.99999) (ML1,1.01616) (ML2,1.00956) (ML3,1.00490) (GMEAN,1.03075)(HIGH,1.0617592884)(H+HM,1.0580508321)(H+HM+HL,1.0534915634)(SomeH,1.0439650806)}; RD 0.5x
				\addplot [LineFillBlueTiny]coordinates {(H0,1.17) (H1,1.29) (H2,1.19) (H3,1.17) (HL0,1.01) (HL1,1.03) (HL2,1.02) (HL3,1.00) (HM0,1.24) (HM1,1.13) (HM2,1.19) (HM3,1.09) (HML0,1.00) (HML1,1.04) (HML2,1.02) (HML3,1.04) (L0,1.00) (L1,1.00) (L2,1.00) (L3,1.00) (M0,1.06) (M1,1.03) (M2,1.04) (M3,1.10) (ML0,1.12) (ML1,1.01) (ML2,1.00) (ML3,1.01) (GMEAN,1.07) (HIGH,1.20) (H+HM,1.18) (H+HM+HML,1.13) (SomeH,1.10)}; %RD 0.25x
 				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Instruction throughput normalized to the baseline in the 8-core CMP system.}
\label{fig:perf_8mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Similarly to the results obtained for a 4-core CMP system, RD outperforms DASCA in the 8-core scenario. Moreover, in the 8-core scenario, higher performance improvements are achieved in both schemes over the baseline. The results reveal that RD improves performance by around 7\% compared to the baseline, while DASCA improves it by around 4\%. As for write-intensive mixes, RD improves the baseline by 20\% and DASCA by 11\%. As shown in Figure~\ref{fig:perf_8mc}, RD significantly overcomes DASCA and the baseline scheme in those mixes which contain any application with high WPKI.


\subsubsection{Energy savings}
\label{subsubsec:energy_8mc}

Figure~\ref{fig:energy_8mc} illustrates the energy savings in the shared LLC. In general, the results in the 8-core scenario follow the trend observed for the 4-core environment. Specifically, RD reports around 32.5\% energy reduction in the STT-RAM SLLC compared to the baseline while DASCA reduces energy by around 27\%. In the case of write-intensive mixes, both RD and DASCA reduce the SLLC energy consumption by 34\% and 27.5\%, respectively. Analyzing  the static and dynamic contributions on the SLLC energy consumption, 
%we obtain Figure~\ref{fig:energy_llc_break8c}, which reveals that, 
overall, RD is able to reduce --for all mixes-- the static energy part by around 6\% with respect to the baseline (around 15\% for the write-intensive mixes) while DASCA reduces the static contribution by 3.6\% (9.5\% for the \emph{high} mixes). In addition, our approach reports dynamic energy savings of around 43\% (36\% for the \emph{high} mixes) while DASCA numbers are 36\% (30\% for the \emph{high} mixes).
Note that mixes made up of applications with low WPKI exhibit the lowest energy savings across the board. This is consistent with the modest write reduction they report and especially with the high contribution of the static part to the total SLLC energy consumption that they exhibit, as Figure~\ref{fig:energy_llc_break8c} shows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy STT
\begin{figure*}[htb]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=38em,
				ybar, 
				ymin=0.3,
				ymax=1.04,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.3)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH},		
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
%				\addplot [LineFillYellowTiny]coordinates {(H0,0.82859) (H1,0.53729) (H2,0.86918) (H3,0.48613) (HL0,0.53250) (HL1,0.89905) (HL2,0.59969) (HL3,0.73079) (HM0,0.68606) (HM1,0.87807) (HM2,0.68673) (HM3,0.60790) (HML0,0.72432) (HML1,0.92331) (HML2,0.78712) (HML3,0.64104) (L0,0.87359) (L1,0.97907) (L2,0.93043) (L3,0.93178) (M0,0.84761) (M1,0.80694) (M2,0.88082) (M3,0.74649) (ML0,0.87089) (ML1,0.87811) (ML2,0.76132) (ML3,0.93665) (GMEAN,0.76766)(HIGH,0.6585730467)(H+HM,0.6829145233)(H+HM+HML,0.7083719571)(SomeH,0.7003416111)};
%				\addplot [LineFillYellowTiny]coordinates {(H0,) (H1,) (H2,) (H3,) (HL0,) (HL1,) (HL2,) (HL3,) (HM0,) (HM1,) (HM2,) (HM3,) (HML0,) (HML1,) (HML2,) (HML3,) (L0,) (L1,) (L2,) (L3,) (M0,) (M1,) (M2,) (M3,) (ML0,) (ML1,) (ML2,) (ML3,) (GMEAN,)(HIGH,)(H+HM,)(H+HM+HML,)(SomeH,)};
				%\addplot [LineFillYellowTiny]coordinates {(H0,0.74) (H1,0.69) (H2,0.73) (H3,0.74) (HL0,0.82) (HL1,0.61) (HL2,0.84) (HL3,0.48) (HM0,0.69) (HM1,0.56) (HM2,0.74) (HM3,0.48) (HML0,0.51) (HML1,0.81) (HML2,0.58) (HML3,0.64) (L0,1.03) (L1,0.95) (L2,0.93) (L3,0.95) (M0,0.69) (M1,0.70) (M2,0.75) (M3,0.57) (ML0,0.74) (ML1,0.75) (ML2,0.81) (ML3,0.81) (GMEAN,0.71) (HIGH,0.72) (H+HM,0.66) (H+HM+HML,0.65) (SomeH,0.66) };
				\addplot [LineFillYellowTiny]coordinates {(H0,0.74) (H1,0.69) (H2,0.73) (H3,0.74) (HL0,0.82) (HL1,0.61) (HL2,0.84) (HL3,0.48) (HM0,0.69) (HM1,0.56) (HM2,0.74) (HM3,0.48) (HML0,0.51) (HML1,0.81) (HML2,0.58) (HML3,0.64) (L0,1.03) (L1,0.95) (L2,0.93) (L3,0.95) (M0,0.69) (M1,0.70) (M2,0.75) (M3,0.57) (ML0,0.74) (ML1,0.75) (ML2,0.81) (ML3,0.81) (AVG,0.72674) (HIGH,0.7241789124) (H+HM,0.670773469) (H+HM+HML,0.6591915173) (SomeH,0.666612771) };
		%		\addplot [LineFillBlueTiny]coordinates {(H0,0.85801) (H1,0.51200) (H2,0.85399) (H3,0.49029) (HL0,0.53960) (HL1,0.89724) (HL2,0.60553) (HL3,0.60472) (HM0,0.63448) (HM1,0.87713) (HM2,0.61019) (HM3,0.66396) (HML0,0.74332) (HML1,0.77428) (HML2,0.67579) (HML3,0.65341) (L0,0.86103) (L1,0.96715) (L2,0.91212) (L3,0.92438) (M0,0.84673) (M1,0.81039) (M2,0.88073) (M3,0.77690) (ML0,0.86238) (ML1,0.87075) (ML2,0.76328) (ML3,0.91413) (GMEAN,0.75044)(HIGH,0.6548887237)(H+HM,0.6717688533)(H+HM+HL,0.6842824663)(SomeH,0.6752551993)}; RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.84976) (H1,0.46317) (H2,0.84088) (H3,0.46505) (HL0,0.51288) (HL1,0.89706) (HL2,0.57906) (HL3,0.56911) (HM0,0.57837) (HM1,0.87224) (HM2,0.56875) (HM3,0.64764) (HML0,0.72344) (HML1,0.74552) (HML2,0.63855) (HML3,0.63048) (L0,0.84627) (L1,0.96326) (L2,0.89790) (L3,0.92117) (M0,0.82396) (M1,0.77669) (M2,0.86005) (M3,0.74003) (ML0,0.84158) (ML1,0.86418) (ML2,0.74629) (ML3,0.90156) (GMEAN,0.72576)(HIGH,0.6263528984)(H+HM,0.6412771004)(H+HM+HL,0.6547737472)(SomeH,0.646943375)}; RD 0.5 x
%				\addplot [LineFillBlueTiny]coordinates {(H0,0.85493) (H1,0.44983) (H2,0.83045) (H3,0.45869) (HL0,0.49642) (HL1,0.89526) (HL2,0.58151) (HL3,0.54746) (HM0,0.55642) (HM1,0.88234) (HM2,0.54764) (HM3,0.69141) (HML0,0.81504) (HML1,0.73861) (HML2,0.62668) (HML3,0.61807) (L0,0.84347) (L1,0.97018) (L2,0.88796) (L3,0.92037) (M0,0.82774) (M1,0.76538) (M2,0.86471) (M3,0.73405) (ML0,0.83936) (ML1,0.85364) (ML2,0.73374) (ML3,0.91700) (GMEAN,0.72362)(HIGH,0.6186626176)(H+HM,0.6373607474)(H+HM+HML,0.6559892547)(SomeH,0.6450477008)}; %RD 0.25x
%\addplot [LineFillBlueTiny]coordinates {(H0,0.67) (H1,0.63) (H2,0.68) (H3,0.66) (HL0,0.81) (HL1,0.49) (HL2,0.81) (HL3,0.41) (HM0,0.70) (HM1,0.48) (HM2,0.69) (HM3,0.45) (HML0,0.48) (HML1,0.82) (HML2,0.51) (HML3,0.53) (L0,0.92) (L1,0.90) (L2,0.89) (L3,0.89) (M0,0.66) (M1,0.65) (M2,0.73) (M3,0.57) (ML0,0.67) (ML1,0.68) (ML2,0.73) (ML3,0.76) (GMEAN,0.66) (HIGH,0.66) (H+HM,0.61) (H+HM+HML,0.60) (SomeH,0.60)}; %RD 0.25x nueva celda
\addplot [LineFillBlueTiny]coordinates {(H0,0.67) (H1,0.63) (H2,0.68) (H3,0.66) (HL0,0.81) (HL1,0.49) (HL2,0.81) (HL3,0.41) (HM0,0.70) (HM1,0.48) (HM2,0.69) (HM3,0.45) (HML0,0.48) (HML1,0.82) (HML2,0.51) (HML3,0.53) (L0,0.92) (L1,0.90) (L2,0.89) (L3,0.89) (M0,0.66) (M1,0.65) (M2,0.73) (M3,0.57) (ML0,0.67) (ML1,0.68) (ML2,0.73) (ML3,0.76) (AVG,0.67488) (HIGH,0.6609072692) (H+HM,0.6215506698) (H+HM+HML,0.6094473931) (SomeH,0.6150310049)}; %RD 0.25x nueva celda
				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Energy consumption in the STT-RAM SLLC normalized to the baseline in the 8-core CMP system.}
\label{fig:energy_8mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}[htb]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				%height=15em,width=38em,
				height=15em,width=28em,
				ybar stacked, 
				ymin=0,
				ymax=1,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.2)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.35em,
				ymajorgrids,
				] 
				%\addplot [LineFillOrangeTiny]coordinates {(H0,) (H1,) (H2,) (H3,) (HL0,) (HL1,) (HL2,) (HL3,) (HM0,) (HM1,) (HM2,) (HM3,) (HML0,) (HML1,) (HML2,) (HML3,) (L0,) (L1,) (L2,) (L3,) (M0,) (M1,) (M2,) (M3,) (ML0,) (ML1,) (ML2,) (ML3,) (AVG,)};
			%	\addplot [LineFillOrangeTiny]coordinates {(H0,0.1069615018) (H1,0.3003637176) (H2,0.1052560516) (H3,0.3198223341) (HL0,0.369791511) (HL1,0.1197104341) (HL2,0.3973856416) (HL3,0.388472699) (HM0,0.305374527) (HM1,0.1152463138) (HM2,0.3108988198) (HM3,0.2617843244) (HML0,0.3108680329) (HML1,0.3744491975) (HML2,0.3571170264) (HML3,0.3488694863) (L0,0.7747538635) (L1,0.6536725021) (L2,0.7805431398) (L3,0.6584482362) (M0,0.3115498335) (M1,0.3615679394) (M2,0.3394152136) (M3,0.4736860266) (ML0,0.5437705416) (ML1,0.3992941945) (ML2,0.559310475) (ML3,0.3929526785) (AVG,0.3836191523)};
			%	\addplot [LineFillGreenTiny]coordinates {(H0,0.8930384982) (H1,0.6996362824) (H2,0.8947439484) (H3,0.6801776659) (HL0,0.630208489) (HL1,0.8802895659) (HL2,0.6026143584) (HL3,0.611527301) (HM0,0.694625473) (HM1,0.8847536862) (HM2,0.6891011802) (HM3,0.7382156756) (HML0,0.6891319671) (HML1,0.6255508025) (HML2,0.6428829736) (HML3,0.6511305137) (L0,0.2252461365) (L1,0.3463274979) (L2,0.2194568602) (L3,0.3415517638) (M0,0.6884501665) (M1,0.6384320606) (M2,0.6605847864) (M3,0.5263139734) (ML0,0.4562294584) (ML1,0.6007058055) (ML2,0.440689525) (ML3,0.6070473215) (AVG,0.6163808477)};
				\addplot [LineFillOrangeTinyND]coordinates {(H0,0.11) (H1,0.11) (H2,0.11) (H3,0.11) (HL0,0.12) (HL1,0.23) (HL2,0.12) (HL3,0.25) (HM0,0.11) (HM1,0.19) (HM2,0.11) (HM3,0.23) (HML0,0.26) (HML1,0.12) (HML2,0.21) (HML3,0.23) (L0,0.67) (L1,0.69) (L2,0.59) (L3,0.67) (M0,0.23) (M1,0.23) (M2,0.24) (M3,0.24) (ML0,0.35) (ML1,0.29) (ML2,0.35) (ML3,0.29) (AVG,0.27)};
				\addplot [LineFillGreenTinyND]coordinates {(H0,0.89) (H1,0.89) (H2,0.89) (H3,0.89) (HL0,0.88) (HL1,0.77) (HL2,0.88) (HL3,0.75) (HM0,0.89) (HM1,0.81) (HM2,0.89) (HM3,0.77) (HML0,0.74) (HML1,0.88) (HML2,0.79) (HML3,0.77) (L0,0.33) (L1,0.31) (L2,0.41) (L3,0.33) (M0,0.77) (M1,0.77) (M2,0.76) (M3,0.76) (ML0,0.65) (ML1,0.71) (ML2,0.65) (ML3,0.71) (AVG,0.73) };
				\legend{Static,Dynamic} 
			\end{axis}
		\end{tikzpicture}	
\caption{Breakdown of energy consumption in the SLLC into the static and dynamic contributions for the baseline in the 8-core CMP system.}
\label{fig:energy_llc_break8c}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy STT Satic-dynamic
%\begin{figure*}
%		\begin{tikzpicture} 
%		\centering
%			\begin{axis}[ 
%				small,
%				height=15em,width=44em,
%				ybar, 
%				ymin=0.45,
%				ymax=1.02,
%				enlargelimits=0.03, 
%				legend style={font=\scriptsize,at={(0.5,-0.5)}, 
%				anchor=north,legend columns=5}, 
				%%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
%			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN}, 
%				xtick=data, 
 %			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
	%			bar width=0.07em,
	%			ymajorgrids,
	%			] 
	%			\addplot [LineFillRedTiny]coordinates {(H0,0.97474) (H1,0.88745) (H2,0.88409) (H3,0.93751) (HL0,0.96525) (HL1,0.99790) (HL2,0.99524) (HL3,0.91397) (HM0,0.96720) (HM1,0.87232) (HM2,0.95301) (HM3,0.95027) (HML0,0.99364) (HML1,0.97874) (HML2,0.98232) (HML3,0.98339) (L0,1.00219) (L1,1.00486) (L2,0.97625) (L3,0.99244) (M0,0.98060) (M1,0.98679) (M2,0.99129) (M3,0.98469) (ML0,1.01795) (ML1,0.99293) (ML2,0.99800) (ML3,0.99182) (GMEAN,0.96914)};
	%			\addplot [LineFillBlueTiny]coordinates {(H0,0.90348) (H1,0.84879) (H2,0.82519) (H3,0.86694) (HL0,0.91841) (HL1,0.97896) (HL2,0.99112) (HL3,0.79100) (HM0,0.93636) (HM1,0.67433) (HM2,0.91561) (HM3,0.80471) (HML0,0.96722) (HML1,0.97735) (HML2,0.96237) (HML3,0.96479) (L0,1.00075) (L1,0.99875) (L2,0.96180) (L3,0.98670) (M0,0.94976) (M1,0.95126) (M2,0.94994) (M3,0.95728) (ML0,0.97824) (ML1,0.94269) (ML2,0.99836) (ML3,0.98276) (GMEAN,0.92459)};
	%			\addplot [LineFillOrangeTiny]coordinates {(H0,0.82148) (H1,0.92521) (H2,0.91691) (H3,0.95484) (HL0,0.90964) (HL1,0.48262) (HL2,0.76555) (HL3,0.92680) (HM0,0.78355) (HM1,0.90400) (HM2,0.75335) (HM3,0.83297) (HML0,0.91425) (HML1,0.82470) (HML2,0.85135) (HML3,0.81896) (L0,0.94640) (L1,0.94350) (L2,0.85964) (L3,0.67651) (M0,0.92369) (M1,0.81160) (M2,0.80310) (M3,0.74383) (ML0,0.86557) (ML1,0.75279) (ML2,0.97419) (ML3,0.90203) (GMEAN,0.83516)};
	%			\addplot [LineFillGreenTiny]coordinates {(H0,0.82066) (H1,0.93740) (H2,0.91258) (H3,0.94549) (HL0,0.85617) (HL1,0.46759) (HL2,0.71094) (HL3,0.88217) (HM0,0.79883) (HM1,0.84322) (HM2,0.83201) (HM3,0.89089) (HML0,0.79316) (HML1,0.78972) (HML2,0.92430) (HML3,0.80993) (L0,0.73210) (L1,0.92514) (L2,0.81202) (L3,0.67849) (M0,0.83537) (M1,0.71247) (M2,0.82542) (M3,0.66686) (ML0,0.76917) (ML1,0.57872) (ML2,0.92891) (ML3,0.93950) (GMEAN,0.79877)};
	%			\legend{DASCA Static, RD Static, DASCA Dynamic, RD Dynamic} 
	%		\end{axis}
	%	\end{tikzpicture}	
%\caption{Energy consumption (static vs dynamic) in the LLC normalized to the baseline: multiprogrammed workloads.}
%\label{fig:energy_break_mc}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

Figure~\ref{fig:energy_dram_8mc} illustrates the energy savings obtained in the DRAM main memory, where it is shown that RD reduces the energy consumption of the main memory by around 6\% on average compared to the baseline (3\% for the write-intensive mixes), while DASCA reaches a 2.8\% energy reduction and actually wastes more energy, around 6\%, for the \emph{high} mixes. This energy waste may look surprising, given that DASCA is able to reduce the number of writes with respect to the baseline by 35\% and to deliver a performance improvement higher than 10\%. However, this can be explained by the fact that DASCA suffers a very significant increase in the amount of SLLC misses, which translates into high values of DRAM accesses (as shown in Table~\ref{tab:comp8c}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Energy DRAM
\begin{figure*}[htb]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=38em,
				ybar, 
				ymin=0.8,
				ymax=1.12,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.3)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
%				\addplot [LineFillYellowTiny]coordinates {(H0,1.06) (H1,1.01) (H2,1.09) (H3,1.07) (HL0,1.03) (HL1,0.96) (HL2,0.97) (HL3,1.01) (HM0,0.91) (HM1,0.90) (HM2,1.01) (HM3,0.91) (HML0,1.01) (HML1,0.96) (HML2,1.01) (HML3,0.97) (L0,1.10) (L1,1.01) (L2,1.01) (L3,1.01) (M0,0.89) (M1,0.93) (M2,0.90) (M3,0.84) (ML0,0.85) (ML1,0.92) (ML2,0.96) (ML3,0.96) (GMEAN,0.97) (HIGH,1.06) (H+HM,0.99) (H+HM+HML,0.99) (SomeH,0.99)};
				\addplot [LineFillYellowTiny]coordinates {(H0,1.06) (H1,1.01) (H2,1.09) (H3,1.07) (HL0,1.03) (HL1,0.96) (HL2,0.97) (HL3,1.01) (HM0,0.91) (HM1,0.90) (HM2,1.01) (HM3,0.91) (HML0,1.01) (HML1,0.96) (HML2,1.01) (HML3,0.97) (L0,1.10) (L1,1.01) (L2,1.01) (L3,1.01) (M0,0.89) (M1,0.93) (M2,0.90) (M3,0.84) (ML0,0.85) (ML1,0.92) (ML2,0.96) (ML3,0.96) (AVG,0.97240) (HIGH,1.0568101602) (H+HM,0.9932456566) (H+HM+HML,0.9906625218) (SomeH,0.9908220942)};
			%	\addplot [LineFillBlueTiny]coordinates {(H0,0.89106) (H1,0.82888) (H2,0.95308) (H3,0.80582) (HL0,0.82821) (HL1,0.93045) (HL2,0.92296) (HL3,0.95524) (HM0,0.89701) (HM1,0.90170) (HM2,0.91325) (HM3,0.88014) (HML0,0.88605) (HML1,0.92404) (HML2,0.91423) (HML3,0.89445) (L0,0.99621) (L1,1.01001) (L2,1.00626) (L3,0.98529) (M0,0.93279) (M1,0.93661) (M2,0.92889) (M3,0.88962) (ML0,0.99383) (ML1,0.92905) (ML2,0.96074) (ML3,0.97624) (GMEAN,0.92254)(HIGH,0.8678410022)(H+HM,0.8827655468)(H+HM+HL,0.8899735887)(SomeH,0.8944188932)};RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,0.93343) (H1,0.90130) (H2,0.93858) (H3,0.89515) (HL0,0.95930) (HL1,0.93022) (HL2,0.93002) (HL3,0.96277) (HM0,0.88468) (HM1,0.90849) (HM2,0.91329) (HM3,0.84809) (HML0,0.85364) (HML1,0.91518) (HML2,0.91646) (HML3,0.89403) (L0,0.99514) (L1,1.01285) (L2,1.00605) (L3,0.98672) (M0,0.93648) (M1,0.93377) (M2,0.91949) (M3,0.90127) (ML0,0.99217) (ML1,0.93551) (ML2,0.96345) (ML3,0.97095) (GMEAN,0.93259)(HIGH,0.9169164575)(H+HM,0.9024742951)(H+HM+HL,0.8997955821)(SomeH,0.9109981829)}; RD 0.5x
%				\addplot [LineFillBlueTiny]coordinates {(H0,0.99) (H1,0.89) (H2,1.01) (H3,0.99) (HL0,1.01) (HL1,0.91) (HL2,0.97) (HL3,0.99) (HM0,0.85) (HM1,0.80) (HM2,0.92) (HM3,0.87) (HML0,0.97) (HML1,0.95) (HML2,0.96) (HML3,0.91) (L0,1.11) (L1,1.02) (L2,1.03) (L3,1.02) (M0,0.86) (M1,0.89) (M2,0.88) (M3,0.82) (ML0,0.85) (ML1,0.94) (ML2,0.97) (ML3,0.93) (GMEAN,0.94) (HIGH,0.97) (H+HM,0.91) (H+HM+HML,0.92) (SomeH,0.94)};%RD 0.25x
			\addplot [LineFillBlueTiny]coordinates {(H0,0.99) (H1,0.89) (H2,1.01) (H3,0.99) (HL0,1.01) (HL1,0.91) (HL2,0.97) (HL3,0.99) (HM0,0.85) (HM1,0.80) (HM2,0.92) (HM3,0.87) (HML0,0.97) (HML1,0.95) (HML2,0.96) (HML3,0.91) (L0,1.11) (L1,1.02) (L2,1.03) (L3,1.02) (M0,0.86) (M1,0.89) (M2,0.88) (M3,0.82) (ML0,0.85) (ML1,0.94) (ML2,0.97) (ML3,0.93) (AVG,0.94020) (HIGH,0.9711119021) (H+HM,0.9162480239) (H+HM+HML,0.9266828619) (SomeH,0.9374901385)};%RD 0.25x
 				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Energy consumption in the DRAM normalized to the baseline in the 8-core CMP system.}
\label{fig:energy_dram_8mc}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Discussion}
\label{subsubsec:disc_8mc}

As in the 4-core configuration, in this section we explain the reasons for the higher performance improvement achieved in our technique (RD) against DASCA in the 8-core scenario.

As we already reasoned in the previous section, the better performance of RD is due to several factors, being the most important one the high efficiency achieved from the reuse locality exploitation. For demonstrating that fact, Figure~\ref{fig:hits_8mc} shows the number of hits in the SLLC per kilo instruction that each mix experiments normalized to the baseline. As the figure shows, our approach achieves in most mixes a higher or much higher number of hits than DASCA, which confirms that RD uses a more efficient policy than DASCA.

%For the 8-core configuration the performance improvements came from the same sources the 4-core improvements did, viz. first LLC write reduction greater than those of DASCA, the main effect of LLC write reduction is to reduce the LLC bank contention (the STT-RAM Read/Write latency asymmetry annoys the LLC pipeline, with symetric Read/Write latencies the LLC could serves an access per cycle but the longer Write latency breaks the pipeline and it creates a bank contention i.e. the bank have to finish the write before it can attend another access); second taking advantage of bypassing the non-reused blocks LLC could be filled with blocks that will be reused again eliminating some LLC miss penalties (filling the LLC with non-reused and reused block causes that some reused blocks will be evicted for allocating non-reused blocks this could generates a LLC miss), Figure~\ref{fig:hits_8mc} shows the amount of hits in the LLC per kilo instruction that each mix experiments normalized to the baseline, the hit rate increment could be translated as faster accesses because that hitted blocks was allocated in LLC instead of Main Memory.


\begin{figure*}[h!]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=38em,
				ybar, 
				ymin=0.8,
				%ymax=2.2,
				ymax=1.22,
				enlargelimits=0.03, 
				legend style={font=\scriptsize,at={(0.5,-0.3)}, 
				anchor=north,legend columns=5}, 
				%symbolic x coords={MIX H0, MIX H1, MIX H2, MIX H3,MIX HL0, MIX HL1, MIX HL2, MIX HL3, MIX HM0, MIX HM1, MIX HM2, MIX HM3, MIX HML0, MIX HML1, MIX HML2, MIX HML3, MIX L0, MIX L1, MIX L2, MIX L3, MIX M0, MIX M1, MIX M2, MIX M3, MIX ML0, MIX ML1, MIX ML2, MIX ML3,gmean}, 
			%symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,GMEAN,HIGH,H+HM,H+HM+HML,SomeH},
			symbolic x coords={H0,H1,H2,H3,HL0,HL1,HL2,HL3,HM0,HM1,HM2,HM3,HML0,HML1,HML2,HML3,L0,L1,L2,L3,M0,M1,M2,M3,ML0,ML1,ML2,ML3,AVG,HIGH,H+HM,H+HM+HML,SomeH},
				xtick=data, 
 			   x tick label style={font=\scriptsize,rotate=40,anchor=east},
				bar width=0.25em,
				ymajorgrids,
				] 
				%\addplot [LineFillYellowTiny]coordinates {(H0,0.86) (H1,0.86) (H2,0.80) (H3,0.85) (HL0,0.98) (HL1,0.88) (HL2,0.96) (HL3,0.61) (HM0,0.86) (HM1,0.89) (HM2,0.88) (HM3,1.05) (HML0,0.89) (HML1,0.99) (HML2,0.80) (HML3,0.92) (L0,0.94) (L1,0.94) (L2,0.95) (L3,0.94) (M0,1.03) (M1,1.03) (M2,1.01) (M3,1.05) (ML0,0.89) (ML1,1.04) (ML2,1.01) (ML3,0.96) (GMEAN,0.92) (HIGH,0.84) (H+HM,0.88) (H+HM+HML,0.89) (SomeH,0.87)};
				\addplot [LineFillYellowTiny]coordinates {(H0,0.86) (H1,0.86) (H2,0.80) (H3,0.85) (HL0,0.98) (HL1,0.88) (HL2,0.96) (HL3,0.61) (HM0,0.86) (HM1,0.89) (HM2,0.88) (HM3,1.05) (HML0,0.89) (HML1,0.99) (HML2,0.80) (HML3,0.92) (L0,0.94) (L1,0.94) (L2,0.95) (L3,0.94) (M0,1.03) (M1,1.03) (M2,1.01) (M3,1.05) (ML0,0.89) (ML1,1.04) (ML2,1.01) (ML3,0.96) (AVG,0.92426) (HIGH,0.8428920821) (H+HM,0.8814350865) (H+HM+HML,0.8877769874) (SomeH,0.8805220409)};
%				\addplot [LineFillBlueTiny]coordinates {(H0,1.03) (H1,4.39) (H2,1.02) (H3,4.94) (HL0,2.88) (HL1,1.00) (HL2,1.34) (HL3,1.19) (HM0,1.27) (HM1,1.00) (HM2,1.17) (HM3,1.30) (HML0,1.33) (HML1,1.06) (HML2,1.12) (HML3,1.27) (L0,1.06) (L1,1.01) (L2,1.04) (L3,1.00) (M0,1.03253) (M1,1.08) (M2,1.04) (M3,1.16) (ML0,1.01) (ML1,1.02) (ML2,1.06) (ML3,1.01669) (GMEAN,1.26)(HIGH,2.1848032713)(H+HM,1.604367847)(H+HM+HL,1.4522378495)(SomeH,1.4549394302)}; RD 1x
				%\addplot [LineFillBlueTiny]coordinates {(H0,1.02) (H1,2.63) (H2,1.01) (H3,2.98) (HL0,1.24) (HL1,1.00) (HL2,1.11) (HL3,1.17) (HM0,1.23) (HM1,0.99) (HM2,1.08) (HM3,1.34) (HML0,1.33) (HML1,1.03) (HML2,1.04) (HML3,1.24) (L0,0.97) (L1,1.00) (L2,1.02) (L3,0.99) (M0,1.03) (M1,1.07) (M2,1.04) (M3,1.10) (ML0,0.97) (ML1,1.00) (ML2,0.99) (ML3,1.02) (GMEAN,1.15)(HIGH,1.6870853325)(H+HM,1.3943098745)(H+HM+HL,1.3089349484)(SomeH,1.2608045584)}; RD 0.5x
				%\addplot [LineFillBlueTiny]coordinates {(H0,1.01) (H1,1.02) (H2,1.01) (H3,1.01) (HL0,0.99) (HL1,1.09) (HL2,1.10) (HL3,1.03) (HM0,1.01) (HM1,1.18) (HM2,1.01) (HM3,1.21) (HML0,1.07) (HML1,1.01) (HML2,1.20) (HML3,1.13) (L0,1.09) (L1,1.00) (L2,1.02) (L3,0.99) (M0,1.03) (M1,1.06) (M2,1.00) (M3,1.08) (ML0,0.99) (ML1,1.01) (ML2,1.02) (ML3,1.00) (GMEAN,1.05) (HIGH,1.01) (H+HM,1.06) (H+HM+HML,1.07) (SomeH,1.07)}; %RD 0.25x
				\addplot [LineFillBlueTiny]coordinates {(H0,1.01) (H1,1.02) (H2,1.01) (H3,1.01) (HL0,0.99) (HL1,1.09) (HL2,1.10) (HL3,1.03) (HM0,1.01) (HM1,1.18) (HM2,1.01) (HM3,1.21) (HML0,1.07) (HML1,1.01) (HML2,1.20) (HML3,1.13) (L0,1.09) (L1,1.00) (L2,1.02) (L3,0.99) (M0,1.03) (M1,1.06) (M2,1.00) (M3,1.08) (ML0,0.99) (ML1,1.01) (ML2,1.02) (ML3,1.00) (AVG,1.04918) (HIGH,1.0133938477) (H+HM,1.0579785213) (H+HM+HML,1.0723638909) (SomeH,1.0674963725)}; %RD 0.25x
 				\legend{DASCA,RD} 
			\end{axis}
		\end{tikzpicture}	
\caption{Number of STT-RAM SLLC hits per kilo instruction normalized to the baseline in the 8-core CMP system.}
\label{fig:hits_8mc}
\end{figure*}

%As discussed in Section~\ref{subsubsec:disc_mc}, RD exploits the reuse locality in a efficient way, this can be prove with other metrics namely LLC Misses and Hits, DRAM Reads and Writes, Row buffer Read Hit Rate and Bank contention in LLC, all these metrics are showed in Table~\ref{tab:comp8c}, the results are presented for RD and DASCA also they are showed for all and write-intesive mixes. 
In addition to the hit rate improvement, there are other metrics that also justify achieving a better performance, such as SLLC misses, DRAM reads and writes, row buffer read hit rate and bank contention in the SLLC. All these metrics are shown in Table~\ref{tab:comp8c}, for both RD and DASCA and also for both all and write-intensive mixes. Note that the RD beats DASCA in all the metrics considered. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}
	\begin{center}
		%\scriptsize
		%tiny
		\tbl{Average values of different metrics normalized to the baseline in the 8-core CMP system.\label{tab:comp8c}}{ 
		\resizebox{0.8\textwidth}{!}{%
		%\rowcolors{2}{gray!23}{gray!10}	
		%\begin{tabular}{|c|c|c|c|c|c|c|}
		\begin{tabular}{|l|C{3.5em}|C{3.5em}|C{7.5em}|C{3.5em}|C{3.5em}|C{8.5em}|}
			\hline
			%\rowcolor{gray!40}
			 \backslashbox{\textbf{Policies}}{\textbf{Metrics}}&\textbf{SLLC Misses}&\textbf{SLLC Hits}&\textbf{Row buffer Read Hit Rate}&\textbf{DRAM reads}&\textbf{DRAM Writes}&\textbf{Bank contention in SLLC}\\
			%\textbf{LLC Misses}&\textbf{LLC Hits}&\textbf{LLC MR}&\textbf{RB RHR}&\textbf{RB WHR}&\textbf{DRAM Reads}&\textbf{DRAM Writes}\\
			%\hline
				\hline
				\textbf{DASCA (All/High)} & 1.08/1.30 & 0.92/0.84 & 1.00/0.99 & 1.08/1.30 & 1.09/1.21 & 0.40/0.13 \\
				\hline
				%\textbf{DASCA (High)} & 1.05 & 1.09 & 1.00 & 1.05 & 1.06 & 0.15\\
				%\hline
				%\textbf{RD (All/High)} & 0.93/0.92 & 1.26/2.18 & 1.05/1.07 & 0.95/0.92 & 0.95/0.89 & 0.32/0.15\\ %RD 1x
				%\textbf{RD (All/High)} & 0.94/0.95 & 1.15/1.69 & 1.04/1.01 & 0.97/0.96 & 0.95/0.94 & 0.25/0.09\\ %RD 0.5x
				\textbf{RD (All/High)} & 0.98/1.00 & 1.05/1.01 & 1.02/1.04 & 1.00/1.06 & 1.02/1.05 & 0.24/0.07\\ %RD 0.25x
				\hline
			    %\textbf{RD (High)} & 0.92 & 2.18 & 1.07 & 0.92 & 0.89 & 0.15\\
				%\hline
		\end{tabular}}}
	\end{center}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[h!]
%	\begin{center}
%		%\scriptsize
%		%tiny
%		\tbl{Average (geomean) values of different metrics normalized to the baseline in the 8-core CMP system.}{ 
%		\resizebox{1\textwidth}{!}{%	
%		%\begin{tabular}{|c|c|c|c|c|c|c|}
%		\rowcolors{2}{gray!23}{gray!10}
%		\begin{tabular}{l|C{3.5em}C{7em}C{8em}C{8em}C{3.5em}}
%		\rowcolor{gray!40}
%			%\hline
%			 \backslashbox{\textbf{Policies}}{\textbf{Metrics}}&\textbf{Writes LLC}&\textbf{Instr. Throughput}&\textbf{Energy consumpt. LLC}&\textbf{Energy consumpt. DRAM}&\textbf{Hits LLC}\\
%			%	\hline
%				\textbf{DASCA (All/High)} & 0.52/0.64 & 1.04/1.11 & 0.71/0.72 & 0.97/1.06 & 0.92/0.84\\
%			%	\hline
%				%\textbf{RD (All/High)} & 0.55/0.61 & 1.08/1.22 & 0.83/0.77 & 0.91/0.90 & 1.12/1.03\\1x
%				\textbf{RD (All/High)} & 0.41/0.56 & 1.07/1.20 & 0.65/0.66 & 0.93/0.97 & 1.05/1.01\\%0.125x
%			%	\hline
%		\end{tabular}}}
%		\label{tab:comp8c}
%	\end{center}
%\end{table}

%As in the single-core scenario, next we zoom into particular mixes that need further detail to get a better understanding. First, in some mixes such as H0, HM3 or HML0 we can observe that the DASCA scheme is able to reduce the amount of writes to the SLLC and also the energy consumption in the STT-RAM more than our scheme does (Figures~\ref{fig:writes_8mc} and \ref{fig:energy_8mc}). Conversely, the RD manages to deliver more throughput than DASCA (Figure~\ref{fig:perf_mc}). However, these performance improvements our approach achieves are not enough to offset the higher energy savings in the SLLC that the DASCA scheme reports for these mixes as a consequence of the lower number of writes to the STT-RAM. 
%Although for mix HM3, as shown in Figure~\ref{fig:energy_break_mc}, the RD manages to reduce the \emph{static} energy consumption of the SLLC by 20\% with respect to the baseline --due to the higher throughput delivered-- and DASCA just reaches 5\%, the \emph{dynamic} energy consumption the RD manages to reduce is just 11\% vs 19\% of DASCA. Although the difference between the numbers achieved by both policies is greater in the case of the static contribution and favorable to our approach, the net result is more favorable to DASCA for this mix due to the higher weight that the dynamic part has in this mix as shown in Figure~\ref{fig:energy_llc_break}. However, the RD allows to report much higher energy savings in the DRAM main memory (19\% vs 2\% of DASCA) due to the high performance improvement already mentioned and to the higher impact the leakage currents has over DRAM technology compared to STT-RAM.



%Second, data for mix L2 reveal that the RD is able to reduce the amount of writes to the SLLC much more than DASCA with respect to the baseline (81\% vs. 48\%). However, this great difference translates into just 22\% of energy savings in RD vs. 13\% of DASCA. As shown, the difference between both policies has been significantly reduced due to the low contribution of the dynamic energy to the total energy consumption in the SLLC that this mix exhibits, as Figure~\ref{fig:energy_llc_break8c} illustrates.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Second, as shown in Figure~\ref{fig:perf_mc}, the RD delivers significantly higher performance than DASCA. Although it was explained earlier that this improvement comes from the higher number of hits, there are other factors that also contribute to the gain such as less write operations to the SLLC, less main memory accesses, and increased row buffer hit rates. 


%Notably, there are some mixes like H3, HL3, HM1 or HM3, where the RD achieves a very significant throughput improvement with respect to the  baseline (15-25\% and up to 47\%) and also compared to DASCA. In all these mixes but HM3 --as already stated before-- our approach manages to slightly reduce the number of the long and power-hungry writes to the SLLC to a greater extent than DASCA. As evident, this fact in isolation can not justify the performance improvements obtained. But if we deep into detail our data reveal that the miss rate in the SLLC  that our approach exhibits is much lower (39\% in mix HM3 or 9\% in H3) than in the DASCA scheme. In addition, the total amount of misses in the LLC is also much lower with our RD than in DASCA (33\% in mix HM3 or or 10\% in H3) and the number of hits in the LLC is higher too (for example, 10\% higher in mix HM3). Furthermore, in all these four mixes the main memory accesses are significantly lower than in DASCA and the row buffer (RB) hit rates (both read and write) are moderately higher in our scheme than in DASCA and much higher than in the baseline. And last but not least, as a side-effect of the new SLLC management, the miss rate in the private L1 caches is also get reduced moderately for some mixes. Notably, mix HM1 and mix HL3 using our RD reports respectively 7.5\% and 6\% lower miss rate in the L1s than the baseline, vs the 1.5\% and 3\% lower miss rate of DASCA. 

%In order to a deeper comparison between our proposal and DASCA, Table~\ref{tab:comp} recaps the average values of different metrics involved in performance that our Reuse Detector and the DASCA scheme report normalized to those of the baseline. As shown our scheme improves DASCA and the baseline (especially in the data from write-intensive mixes) in all the metrics considered.



\subsubsection{Sensitivity to Reuse Detector size}
\label{subsubsec:sense8c}

%One key aspect in designing the Reuse Detector is to decide the \emph{expulsion coverage} it provides. In other words, the RD size is an important issue in the implementation of our proposal.
Given that the RD size is a determining factor in our proposal, and as done in the 4-CMP system, in Figure~\ref{fig:sense_sc8c} we show the amount of writes to the SLLC, the Instruction Throughput, and the energy consumption in both the SLLC and the main memory for different RD sizes per core, namely 8K, 16K, 32K and 64K entries. 

The trends are very similar to those observed in the 4-core scenario. Notably, a significant impact is observed on the capability to reduce the number of writes in the SLLC, especially for the All mixes, whereas a moderate (or even negligible in some cases) impact is seen on the average energy consumed in that cache level or main memory and performance of the overall system.
%The RD size is a key design aspect of our proposal.  
%In order to evaluate its impact we show in Figure~\ref{fig:sense_sc8c} the amount of writes to the SLLC, the Instruction Throughput, 
%the amount of hits in the SLLC, 
%and the energy consumption in both the SLLC and the main memory for different RD sizes per core, namely 8K, 16K, 32K and 64K entries. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Sensibilidad a tamaño detector reuso
\begin{figure*}[t!]
		\begin{tikzpicture} 
		\centering
			\begin{axis}[ 
				small,
				height=15em,width=38em,
				ybar, 
				ymin=0.3,
				ymax=1.2,
				enlargelimits=0.15, 
				legend style={font=\scriptsize,at={(0.5,-0.2)}, 
				anchor=north,legend columns=8}, 
				%symbolic x coords={Writes LLC,IT,Hits LLC,Eng. STT-RAM,Eng. DRAM}, 
				symbolic x coords={Writes SLLC,IT,Eng. SLLC,Eng. DRAM}, 
				xtick=data, 
 			   x tick label style={font=\scriptsize},
				bar width=0.7em,
				ymajorgrids,
				]
				%\addplot [LineFillRedTiny]coordinates {(Writes LLC,0.26170) (IT,1.02907) (Hits LLC,1.16) (Eng. STT-RAM,0.72576) (Eng. DRAM,0.93742)}; %0.25x all
				%\addplot [LineFillBlueTiny]coordinates {(Writes LLC,0.29273) (IT,1.03075) (Hits LLC,1.15) (Eng. STT-RAM,0.72576) (Eng. DRAM,0.93259)}; %0.5x all
				%\addplot [LineFillGreenTiny]coordinates {(Writes LLC,0.36722) (IT,1.03757) (Hits LLC,1.26) (Eng. STT-RAM,0.75044) (Eng. DRAM,0.92254)}; %1x all
				%\addplot [LineFillYellowTiny]coordinates {(Writes LLC,0.43867) (IT,1.03164) (Hits LLC,1.26) (Eng. STT-RAM,0.77430) (Eng. DRAM,0.93060)}; %2x all
				%\addplot [LineFillOrangeTiny]coordinates {(Writes LLC,0.2263099303) (IT,1.0711356597) (Hits LLC,1.6356428123) (Eng. STT-RAM,0.6263528984) (Eng. DRAM,0.9174632506)}; %0.25x high
				%\addplot [LineFillTurquoiseTiny]coordinates {(Writes LLC,0.2512276929) (IT,1.0617592884) (Hits LLC,1.6870853325) (Eng. STT-RAM,0.6263528984) (Eng. DRAM,0.9169164575)}; %0.5x high
				%\addplot [LineFillPurpleTiny]coordinates {(Writes LLC,0.3461276381) (IT,1.1038163119) (Hits LLC,2.1848032713) (Eng. STT-RAM,0.6548887237) (Eng. DRAM,0.8678410022)}; %1x high
				%\addplot [LineFillBrownTiny]coordinates {(Writes LLC,0.408131851) (IT,1.0911438469) (Hits LLC,2.1098386489) (Eng. STT-RAM,0.6839962457) (Eng. DRAM,0.885798249)}; %2x high

				%\addplot [LineFillRedTiny2]coordinates {(Writes SLLC,0.26170) (IT,1.02907) (Eng. SLLC,0.72576) (Eng. DRAM,0.93742)}; %0.25x all
				%\addplot [LineFillBlueTiny2]coordinates {(Writes SLLC,0.29273) (IT,1.03075) (Eng. SLLC,0.72576) (Eng. DRAM,0.93259)}; %0.5x all
				%\addplot [LineFillGreenTiny2]coordinates {(Writes SLLC,0.36722) (IT,1.03757) (Eng. SLLC,0.75044) (Eng. DRAM,0.92254)}; %1x all
				%\addplot [LineFillYellowTiny2]coordinates {(Writes SLLC,0.43867) (IT,1.03164) (Eng. SLLC,0.77430) (Eng. DRAM,0.93060)}; %2x all
				%\addplot [LineFillRedTiny3]coordinates {(Writes SLLC,0.2263099303) (IT,1.0711356597) (Eng. SLLC,0.6263528984) (Eng. DRAM,0.9174632506)}; %0.25x high
				%\addplot [LineFillBlueTiny3]coordinates {(Writes SLLC,0.2512276929) (IT,1.0617592884) (Eng. SLLC,0.6263528984) (Eng. DRAM,0.9169164575)}; %0.5x high
				%\addplot [LineFillGreenTiny3]coordinates {(Writes SLLC,0.3461276381) (IT,1.1038163119) (Eng. SLLC,0.6548887237) (Eng. DRAM,0.8678410022)}; %1x high
				%\addplot [LineFillYellowTiny3]coordinates {(Writes SLLC,0.408131851) (IT,1.0911438469) (Eng. SLLC,0.6839962457) (Eng. DRAM,0.885798249)}; %2x high
				%\addplot [LineFillRedTiny2]coordinates {(Writes SLLC,0.41) (IT,1.07) (Eng. SLLC,0.66) (Eng. DRAM,0.94)}; %0.25x all nueva celda
				%\addplot [LineFillBlueTiny2]coordinates {(Writes SLLC,0.46) (IT,1.07) (Eng. SLLC,0.69) (Eng. DRAM,0.94)}; %0.5x all nueva celda
				%\addplot [LineFillGreenTiny2]coordinates {(Writes SLLC,0.52) (IT,1.08) (Eng. SLLC,0.71) (Eng. DRAM,0.91)}; %1x all nueva celda
				%\addplot [LineFillYellowTiny2]coordinates {(Writes SLLC,0.55) (IT,1.08) (Eng. SLLC,0.73) (Eng. DRAM,0.91)}; %2x all nueva celda
				%\addplot [LineFillRedTiny3]coordinates {(Writes SLLC,0.56) (IT,1.20) (Eng. SLLC,0.66) (Eng. DRAM,0.97)}; %0.25x high nueva celda
				%\addplot [LineFillBlueTiny3]coordinates {(Writes SLLC,0.57) (IT,1.21) (Eng. SLLC,0.67) (Eng. DRAM,0.96)}; %0.5x high nueva celda
				%\addplot [LineFillGreenTiny3]coordinates {(Writes SLLC,0.58) (IT,1.23) (Eng. SLLC,0.68) (Eng. DRAM,0.90)}; %1x high nueva celda
				%\addplot [LineFillYellowTiny3]coordinates {(Writes SLLC,0.61) (IT,1.23) (Eng. SLLC,0.70) (Eng. DRAM,0.91)}; %2x high nueva celda
				\addplot [LineFillRedTiny2]coordinates {(Writes SLLC,0.46024) (IT,1.07) (Eng. SLLC,0.67488) (Eng. DRAM,0.94020)}; %0.25x all nueva celda
				\addplot [LineFillBlueTiny2]coordinates {(Writes SLLC,0.49821) (IT,1.07) (Eng. SLLC,0.70049) (Eng. DRAM,0.94043)}; %0.5x all nueva celda
				\addplot [LineFillGreenTiny2]coordinates {(Writes SLLC,0.54379) (IT,1.08) (Eng. SLLC,0.72631) (Eng. DRAM,0.91144)}; %1x all nueva celda
				\addplot [LineFillYellowTiny2]coordinates {(Writes SLLC,0.57066) (IT,1.08) (Eng. SLLC,0.74070) (Eng. DRAM,0.91431)}; %2x all nueva celda
				\addplot [LineFillRedTiny3]coordinates {(Writes SLLC,0.5577391169) (IT,1.20) (Eng. SLLC,0.6609072692) (Eng. DRAM,0.9711119021)}; %0.25x high nueva celda
				\addplot [LineFillBlueTiny3]coordinates {(Writes SLLC,0.5748842483) (IT,1.21) (Eng. SLLC,0.6747333241) (Eng. DRAM,0.9631276293)}; %0.5x high nueva celda
				\addplot [LineFillGreenTiny3]coordinates {(Writes SLLC,0.5850753949) (IT,1.23) (Eng. SLLC,0.6781458801) (Eng. DRAM,0.898559369)}; %1x high nueva celda
				\addplot [LineFillYellowTiny3]coordinates {(Writes SLLC,0.6090648807) (IT,1.23) (Eng. SLLC,0.6964182877) (Eng. DRAM,0.9091556259)}; %2x high nueva celda
				%\legend{32-All,64K-All,128K-All,256K-All,32K-High,64K-High,128K-High,256K-High} 
				\legend{8K-All,16K-All,32-All,64K-All,8K-High,16K-High,32K-High,64K-High} 
			\end{axis}
		\end{tikzpicture}	
%\caption{Writes to LLC, IT, amount of hits in the SLLC, and energy consumption in both SLLC and main memory normalized to the baseline for different RD sizes.}
\caption{Writes to SLLC, IT and energy consumption in both SLLC and main memory normalized to the baseline for different RD sizes per core in the 8-core CMP system.}
\label{fig:sense_sc8c}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As shown, the major impact is observed on the capability to reduce the number of writes in the LLC, ranging from an average reduction of 59\% with respect to the baseline when an 8K-entry RD per core is employed (44\% for the write-intensive mixes) to a reduction of around 35\% for a 64K-entry RD per core (39\% for the \emph{high mixes}). As explained in section~\ref{subsubsec:sense} when the size of RD increases, it also augments the probability that a block finds its tag in the RD, so the probability of bypassing decreases, leading to minor reduction of writes to the LLC. We can also observe a moderate impact on the average energy consumed in the LLC, with values in the range 66-70\% as the size of RD gets increased: again, note that these numbers follow a similar trend to that exhibited by the amount of writes. Finally, the impact over the performance and the energy consumption of the main memory is highly reduced, falling the average IT variations into a range of 1\% (3\% for the write-intensive mixes) and the average DRAM energy variations into a range of 3\% (7\% for the write-intensive mixes). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{RD performance in multi-core scenarios}
\label{subsec:putting}

In this section we briefly inspect the main hints about the performance of RD when we augment the number of cores. So far, we have evaluated the RD in systems with one, four and eight cores. In order to further explore the RD behavior we have also evaluated our proposal in a system with 16 cores, employing the mixes shown in Table~\ref{tab:pmix16C}.



%\begin{table*}[htb]
%	\begin{center}
%%		\small
	%	\tiny
	%	%\footnotesize
	%	%\caption{Proposed SPEC 2006 multiprogrammed mixes 16 cores\label{tab:pmix16C}}{ 
	%	\tbl{Proposed SPEC 2006 multiprogrammed mixes 16 cores.\label{tab:pmix16C}}{
	%	\begin{tabular}{|c|c|}
	%		\hline
	%		%\textbf{Mixes}&\textbf{Applications}&\textbf{Categories}\\
	%		\textbf{Mixes}&\textbf{Applications}\\
	%		\hline
%mix.H0 & 429.mcf, 433.milc, 434.zeusmp, 436.cactusADM, 437.leslie3d, 470.lbm, 410.bwaves, 462.libquantum, \\
%&436.cactusADM, 462.libquantum, 429.mcf, 437.leslie3d, 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc\\
%\hline
%mix.H1 & 429.mcf, 433.milc, 434.zeusmp, 436.cactusADM, 437.leslie3d, 470.lbm, 410.bwaves, 462.libquantum, \\
%&436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, 429.mcf, 433.milc, 434.zeusmp, 462.libquantum\\
%\hline
%mix.H2 & 429.mcf, 433.milc, 434.zeusmp, 436.cactusADM, 437.leslie3d, 470.lbm, 410.bwaves, 462.libquantum, \\
%&429.mcf, 433.milc, 434.zeusmp, 462.libquantum, 470.lbm, 437.leslie3d, 410.bwaves, 436.cactusADM\\
%\hline
%mix.H3 & 436.cactusADM, 462.libquantum, 429.mcf, 437.leslie3d, 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, \\
%&436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, 429.mcf, 433.milc, 434.zeusmp, 462.libquantum\\
%\hline
%mix.H4 & 436.cactusADM, 462.libquantum, 429.mcf, 437.leslie3d, 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, \\
%&429.mcf, 433.milc, 434.zeusmp, 462.libquantum, 470.lbm, 437.leslie3d, 410.bwaves, 436.cactusADM\\
%\hline
%mix.H5 & 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, 429.mcf, 433.milc, 434.zeusmp, 462.libquantum, \\
%&429.mcf, 433.milc, 434.zeusmp, 462.libquantum, 470.lbm, 437.leslie3d, 410.bwaves, 436.cactusADM\\
%\hline
%mix.HM0 & 483.xalancbmk, 445.gobmk, 450.soplex, 473.astar, 403.gcc, 400.perlbench, 456.hmmer, 481.wrf, \\
%&429.mcf, 433.milc, 434.zeusmp, 436.cactusADM, 437.leslie3d, 470.lbm, 410.bwaves, 462.libquantum\\
%\hline
%mix.HM1 & 483.xalancbmk, 400.perlbench, 450.soplex, 401.bzip2, 481.wrf, 483.xalancbmk, 403.gcc, 400.perlbench, \\
%&436.cactusADM, 462.libquantum, 429.mcf, 437.leslie3d, 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc\\
%\hline
%mix.HM2 & 450.soplex, 483.xalancbmk, 403.gcc, 400.perlbench, 445.gobmk, 450.soplex, 456.hmmer, 445.gobmk, \\
%&436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, 429.mcf, 433.milc, 434.zeusmp, 462.libquantum\\
%\hline
%mix.HM3 & 400.perlbench, 445.gobmk, 481.wrf, 473.astar, 481.wrf, 450.soplex, 456.hmmer, 445.gobmk, \\
%&429.mcf, 433.milc, 434.zeusmp, 462.libquantum, 470.lbm, 437.leslie3d, 410.bwaves, 436.cactusADM\\
%\hline
%mix.HM4 & 429.mcf, 433.milc, 434.zeusmp, 462.libquantum, 470.lbm, 437.leslie3d, 410.bwaves, %436.cactusADM,\\
%& 483.xalancbmk, 445.gobmk, 450.soplex, 473.astar, 403.gcc, 400.perlbench, 456.hmmer, 481.wrf\\
%\hline
%mix.HM5 & 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, 429.mcf, 433.milc, 434.zeusmp, 462.libquantum, \\
%&483.xalancbmk, 400.perlbench, 450.soplex, 401.bzip2, 481.wrf, 483.xalancbmk, 403.gcc, 400.perlbench\%\
%\hline
%mix.HM6 & 436.cactusADM, 462.libquantum, 429.mcf, 437.leslie3d, 436.cactusADM, 410.bwaves, 437.leslie3d, 433.milc, \\
%&450.soplex, 483.xalancbmk, 403.gcc, 400.perlbench, 445.gobmk, 450.soplex, 456.hmmer, 445.gobmk\\
%\hline
%mix.HM7 & 429.mcf, 433.milc, 434.zeusmp, 436.cactusADM, 437.leslie3d, 470.lbm, 410.bwaves, 462.libquantum, \\
%&400.perlbench, 445.gobmk, 481.wrf, 473.astar, 481.wrf, 450.soplex, 456.hmmer, 445.gobmk\\
%\hline
%		\end{tabular}}
%	\end{center}
%\end{table*} 

In Table~\ref{tab:cores} we recap the main numbers derived from RD and DASCA evaluation across the different configurations (for the sake of simplicity, we show just the numbers considering all applications or mixes, not those corresponding to the write-intensive ones). Notably, we illustrate the average LLC write reduction capability, energy savings in the LLC, the performance delivered and the energy savings in the DRAM.

\begin{table*}
	\begin{center}
		\scriptsize
		%tiny
		\tbl{Average values of different metrics normalized to the baseline across different configurations.\label{tab:cores}}{ 
		\resizebox{0.8\textwidth}{!}{%
		%\rowcolors{2}{gray!23}{gray!10}	
		%\begin{tabular}{|c|c|c|c|c|c|c|}
		%\begin{tabular}{|l|C{7em}|C{7em}|C{7em}|C{7em}|}
		\begin{tabular}{|l|C{7.5em}|C{7.5em}|C{8em}|C{7.5em}|}
		%\begin{tabular}{|c|c|c|c|c|}
			\hline
			%\rowcolor{gray!40}
			 \backslashbox{\textbf{Scenario}}{\textbf{Metrics}}&\textbf{LLC Write reduction (\%) (DASCA/RD)}&\textbf{LLC Energy Savings (\%) (DASCA/RD)}&\textbf{Performance improvement (\%) (DASCA/RD)}&\textbf{DRAM Energy Savings (\%) (DASCA/RD)}\\
			%\textbf{LLC Misses}&\textbf{LLC Hits}&\textbf{LLC MR}&\textbf{RB RHR}&\textbf{RB WHR}&\textbf{DRAM Reads}&\textbf{DRAM Writes}\\
			%\hline
				\hline
				\textbf{Single core} & 51.8 / 65.2 & 29.5 / 34.5 & 0.3 / 1.9 & 0.2 / 2.0 \\
				\hline
				\textbf{4-core CMP} & 51.6 / 62.7 & 30.8 / 37.0 & 1.2 / 2.9 & 3.6 / 6.2 \\
				\hline
				\textbf{8-core CMP} & 43.8 / 54.0 & 27.3 / 32.5 & 3.7 / 6.7 & 2.8 / 6.0 \\
				\hline
				\textbf{16-core CMP} & 38.6 / 46.7 & 26.0 / 30.5 & 10.2 / 14.5 & 4.0 / 7.9 \\
				\hline
			    %\textbf{RD (High)} & 0.92 & 2.18 & 1.07 & 0.92 & 0.89 & 0.15\\
				%\hline
		\end{tabular}}}
	\end{center}
\end{table*}

As shown, the write reduction capability in percentage terms gets reduced with the number of cores for both RD and DASCA. %Regarding this issue, please note the following aspects: 1) the total number of writes performed to the LLC increases as the number of applications augments (the aggregated number of writes performed by the mixes evaluated in the 16-CMP system is roughly 2x that of the 4-CMP system, 2) The multiprogrammed workloads have been selected to build mixes made up only of applications with high, medium or low WPKI and also by combining applications from different WPKI categories trying to fill most of the combinations high-medium, high-low, medium-low and high-medium-low (see Section~\ref{sec:sim}). As a result, in all the CMP systems evaluated we analyze the behavior of 4 mixes belonging to each of the following categories: H, M, L, HM, HL, ML and HML. Nevertheless, within each of the categories, the applications were randomly selected, not only regarding the specific programs chosen but also regarding the number of applications from each category belonging to the mixes. For example, the four mixes evaluated in the 4-core CMP system within the HL category are made up of: two mixes with 2H and 2L applications and the other two mixes with 3H and 1L applications. By contrast, the four mixes evaluated in the 8-core CMP system within the HL category are all made up of 4H and 4L applications, i.e., the ratio between the number of applications of each type building a mix within a given category is not exactly constant across the explored configurations, and, more importantly 3) The relative impact of those applications exhibiting a significantly high number of writes to the LLC and also a significant write reduction capability when running alone under RD (such as \emph{bwaves}, \emph{lbm} or \emph{milc}, that reduce the number of writes with respect to the baseline by more than 98\%, which explains why the geomean of LLC write reduction in the single core scenario is so high) gets reduced with the number of cores. This also explains that the geomean and the average number of writes performed to the LLC gets closed as the number of cores augments, with both metrics largely matching in the 16-core CMP system. 
However, despite this decrease in the write filtering numbers, the most important consequence derived from this aspect, i.e. the net energy savings in the LLC, essentially remains in the range of 30-37\% for RD, slightly decreasing with the number of cores as a consequence of the increment in the number of writes, but keeping the benefit with respect to DASCA largely unchanged. Moreover, the performance improvement increases as the number of cores augments for both RD and DASCA, reporting significant numbers especially for the 8-core and 16-core system. Indeed, the performance improvement that RD reports with respect to the DASCA scheme also increases with the number of cores (which is especially significant in the case of write-intensive mixes for the 16-CMP system, where RD is able to increase the performance of the baseline by around 38\%, whereas DASCA only achieves 24\% of improvement). This is due to the fact that the difference in LLC misses reported by both approaches increases as the number of cores augments (notably, these numbers are 1\%, 6\%, 10\% and 13\% for 1, 4, 8 and 16-core systems respectively, always reporting RD the best value) and also the difference in other factors as the number of hits in the LLC, the number of DRAM reads and writes or the row buffer hit rate also increase, benefiting RD more with the number of cores. Finally, and derived from the higher performance delivered, the same trend is observed in the energy savings experienced in the main memory (where it is worthy to note that, in the 16-core scenario, RD manages to reduce the energy consumption of the baseline by more than 15\% for the write-intensive mixes, while DASCA hardly achieves 8\%). Overall we can conclude that, as the number of cores increases, RD is able to significantly increase the performance delivered (and also to increase the energy savings achieved in the main memory) at the expense of a slight decrease in the LLC energy savings obtained. 








==> figures/TableExampleProposedPolicies.tex <==
\begin{figure*}
\begin{center}
%\scalebox{0.55}{
\resizebox{1\textwidth}{!}{%
\begin{tabular}[h]{|c|C{9cm}||c|C{9cm}|}

%  \hline

%  \multicolumn{4}{|c|}{ }\\
%  \multicolumn{4}{|c|}{ $\framebox[1.4cm]{$Blk_x$}_{Reuse Bit}$} \\
%  \multicolumn{4}{|c|}{ }\\
%  \hline \hline
%
%
%  \multicolumn{4}{|c|}{ }\\
%	\multicolumn{4}{|c|}{Initial state: All the cache are empty.} \\
%  \multicolumn{4}{|c|}{L1$_0$ $\framebox[0.8cm]{$\phantom{X}_{0,0}$}$ L1$_1$ $\framebox[0.8cm]{$\phantom{X}_{0,0}$}$}\\
%  \multicolumn{4}{|c|}{ }\\ 
%  \multicolumn{4}{|c|}{RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$}\\
%  \multicolumn{4}{|c|}{ }\\ 
%  \multicolumn{4}{|c|}{SLLC $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$}\\
%  \multicolumn{4}{|c|}{ }\\ 
%  \multicolumn{4}{|c|}{Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ }\\  

%  \multicolumn{4}{|c|}{ }\\ \hline \hline

%   & & &\\ 
  %Ref & Memory State & Ref & Memory State\\

  \hline %\hline
  
  
%  & & &\\ 
%  1 & \normalsize{Read Block A, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset} & 2 & \normalsize{Read Block A, it misses in L1$_1$ and SLLC, the block is get from L1$_0$, the Reuse bit set}\\
  & & &\\
  1st& L1$_0$ $\framebox[0.8cm]{$A_{0,0}$}$ L1$_1$ $\framebox[0.8cm]{$\phantom{X}$}$ & 2nd& L1$_0$ $\framebox[0.8cm]{$A_{0,1}$}$ L1$_1$ $\framebox[0.8cm]{$A_{0,1}$}$\\
  Access& &Access &\\
  & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ & & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$\\
  & & &\\
  & SLLC $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ & & SLLC $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ \\  
  & & &\\
  & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$  & & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ \\  
  & & &\\ \hline

%  & & &\\ 
%  Core$_1$ Read A & \footnotesize{Read Block A, it misses in L1$_1$ and SLLC, the block is get from L1$_0$, the Reuse bit set}\\
%  & & &\\
%  & L1$_0$ $\framebox[0.8cm]{$A$}_{1}$ L1$_1$ $\framebox[0.8cm]{$A$}_{1}$\\
%  & & &\\
  %& RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$\\
%  & & &\\
%  & SLLC $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ \\  
%  & & &\\
  %& Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ \\  
%  & & &\\ \hline

  & & &\\ 
%  3 & \normalsize{Read Block B, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block A is filled in the SLLC} & 4 & \normalsize{Read Block C, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block B is bypassed and its address is filled in the RD}\\
%  & & &\\
  3rd & L1$_0$ $\framebox[0.8cm]{$A_{0,1}$}$ L1$_1$ $\framebox[0.8cm]{$B_{0,0}$}$ & 4th & L1$_0$ $\framebox[0.8cm]{$A_{0,1}$}$ L1$_1$ $\framebox[0.8cm]{$C_{0,0}$}$\\
  Access& &Access &\\
  & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ & & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$\phantom{X}$}$\\
  & & &\\
  & SLLC $\framebox[0.8cm]{$A_0$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ & & SLLC $\framebox[0.8cm]{$A_0$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$\\  
  & & &\\
  & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$  & & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ \\  
  & & &\\ \hline

%  & & &\\ 
  %Core$_1$ Read C & \footnotesize{Read Block C, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block B is bypassed and its address is filled in the RD}\\
%  & & &\\
%  & L1$_0$ $\framebox[0.8cm]{$A$}_{1}$ L1$_1$ $\framebox[0.8cm]{$C$}_{0}$\\
%  & & &\\
%  & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$\phantom{X}$}$\\
%  & & &\\
%  & SLLC $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ \\  
%  & & &\\
  %& Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ \\  
%  & & &\\ \hline

  & & &\\ 
%  5 & \normalsize{Read Block B, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block C is bypassed and its address is filled in the RD} & 6 & \normalsize{Read Block D, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block B is filled in the SLLC because its tag is in the RD}\\
%  & & &\\
  5th& L1$_0$ $\framebox[0.8cm]{$A_{0,1}$}$ L1$_1$ $\framebox[0.8cm]{$B_{0,0}$}$ & 6th& L1$_0$ $\framebox[0.8cm]{$A_{0,1}$}$ L1$_1$ $\framebox[0.8cm]{$D_{0,0}$}$\\
  Access& &Access &\\
  & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ & & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$\\
  & & &\\
  & SLLC $\framebox[0.8cm]{$A_0$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ &  & SLLC $\framebox[0.8cm]{$A_0$}$ $\framebox[0.8cm]{$B_0$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$\\  
  & & &\\
  & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$  &  & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ \\  
  & & &\\ \hline

%  & & &\\ 
  %Core$_1$ Read D & \footnotesize{Read Block D, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block B is filled in the SLLC because its tag is in the RD}\\
%  & & &\\
%  & L1$_0$ $\framebox[0.8cm]{$A$}_{1}$ L1$_1$ $\framebox[0.8cm]{$D$}_{0}$\\
%  & & &\\
%  & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$\\
%  & & &\\
%  & SLLC $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ \\  
%  & & &\\
  %& Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ \\  
%  & & &\\ \hline

  & & &\\ 
%  7 & \normalsize{Read Block E, it misses in all L1 and SLLC, the block is get from MM, the Reuse bit unset. The evicted Block A is bypassed because it is clean} & &\\
%  & & &\\
  7th& L1$_0$ $\framebox[0.8cm]{$A_{1,1}$}$ L1$_1$ $\framebox[0.8cm]{$D_{0,0}$}$ & 8th & L1$_0$ $\framebox[0.8cm]{$E_{0,0}$}$ L1$_1$ $\framebox[0.8cm]{$D_{0,0}$}$\\
  Access& &Access &\\
  & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ & & RD$_0$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ RD$_1$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ \\
  & & &\\
  & SLLC $\framebox[0.8cm]{$A_0$}$ $\framebox[0.8cm]{$B_0$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ & & SLLC $\framebox[0.8cm]{$A_1$}$ $\framebox[0.8cm]{$B_0$}$ $\framebox[0.8cm]{$\phantom{X}$}$ $\framebox[0.8cm]{$\phantom{X}$}$ \\  
  & & &\\
  & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$ & & Main Memory $\framebox[0.8cm]{$A$}$ $\framebox[0.8cm]{$B$}$ $\framebox[0.8cm]{$C$}$ $\framebox[0.8cm]{$D$}$ $\framebox[0.8cm]{$E$}$  \\   
  & & &\\ \hline
\end{tabular}}
\caption{Example of the Reuse Detector operation.}
\label{tableExampleReuseDet}
\end{center}
\end{figure*}


==> motivation_original.tex <==
\section{Background and motivation}
\label{sec:motiv}

In this section we first motivate the need of a new SLLC management scheme by describing the main limitations of SRAM technology and conventional management. Then we briefly describe the DASCA scheme, which is the closest approach to our work and the state-of-the-art STT-RAM SLLC management scheme~\cite{dasca_14}.


\subsection{SRAM and STT-RAM technologies}

As stated above, various emerging technologies are currently considered to replace SRAM as the building-block for SLLCs, being STT-RAM the best placed to overcome SRAM constraints, such as energy consumption and read operation latency. 

The main difference between STT-RAM and SRAM is that the information carrier of the former is a Magnetic Tunnel Junction (MTJ) instead of electric charges. An MTJ contains two ferromagnetic layers (denoted as free and fixed layers) and one tunnel barrier layer, see Figure~\ref{fig:stta}. The fixed layer has a fixed magnetic direction while the free layer can change its magnetic direction by passing a current through the MTJ. If the two ferromagnetic layers have different directions, the MTJ resistance is high, indicating a ``1" state; if the two layers have the same direction, the MTJ resistance is low, indicating a ``0" state. A read operation to an MTJ is performed by applying a small voltage difference between two electrodes of the MTJ and sensing the current flow (see Figure~\ref{fig:sttb}, where the STT-RAM cell is represented as a variable resistor). A write operation is performed by applying a large voltage difference between two electrodes for a given duration called write pulse width.

%\begin{figure}
%\centerline{\includegraphics[width=0.45\textwidth]{figures/sttram.png}}
%\caption{Illustration of an STT-RAM cell.}
%\label{fig:stt}
%\end{figure}

%\begin{figure}[H]
%\begin {center}
%\includegraphics[width=0.3\textwidth]{figures/CeldaSTTRAM.png}   
%\caption{STT-RAM memory cell structure.}
%\label{fig:stt}
%\end {center}
%\end{figure}

\begin{figure}
     \begin{center}
        \subfigure[ ]{%
            \label{fig:stta}
            %\fbox{
            \includegraphics[width=0.45\textwidth,natwidth=600,natheight=491]{CeldaSTTRAM}
            %}
        }%
		 %\quad %\quad
        \subfigure[ ]{%
           \label{fig:sttb}
           %\fbox{
           \includegraphics[width=0.25\textwidth,natwidth=374,natheight=271]{STTRAMCircuit}
           %}
        }
    \end{center}
    \caption{%
        (a) STT-RAM memory cell structure. (b) STT-RAM equivalent circuit.}%
\end{figure}


Table~\ref{tab:param} shows the key features of an 1-bank 1MB LLC implemented with SRAM and STT-RAM 22 nm technology, modeled with CACTI 6.5~\cite{cacti65} and NVSim~\cite{nvsim_12}, respectively. As shown, an STT-RAM cache exhibits smaller die footprint and better efficiency in read operations than an SRAM cache. More importantly, an STT-RAM cache consumes almost two orders of magnitude less static power compared to SRAM. Conversely, the STT-RAM cache exhibits a significant drawback that needs to be mitigated: the poor write performance both in terms of latency and energy consumption. 

\begin{table}
\begin{center}
\scriptsize
\tbl{Area, latency and energy consumption for 22 nm SRAM and STT-RAM 1MB caches.\label{tab:param}}{ 
    \resizebox{1\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
%\textbf{Parameter}&\textbf{SRAM}&\textbf{STT-RAM}&\textbf{Difference}\\
\textbf{Parameter}&\textbf{SRAM}&\textbf{STT-RAM}&\textbf{Ratio SRAM/STT-RAM}\\
\hline
Area ($mm^2$) & 0.94 & 0.35 & 2.68\\
\hline
Read Latency (ns) & 8.75 & 5.61 & 1.56\\
\hline
Write Latency (ns) & 8.75 & 16.5 & 0.53\\
\hline
Read Energy (nJ) & 0.56 & 0.32 & 1.75\\
\hline
Write Energy (nJ) & 0.56 & 1.31 & 0.43\\
\hline
Leakage Power (mW) & 190.58 & 3.09 & 61.67\\
\hline
\end{tabular}}}
\end{center}
\end{table}


\subsection{SLLC management techniques}

Regardless of implementation technology, last-level caches usually suffer from the same problem: they keep data assuming that recently referenced lines are likely to appear in the near future (\emph{temporal locality}). Nevertheless, various recent studies point out that the reference stream entered in the SLLC does not usually exhibit temporal locality. Notably, in~\cite{albericio_taco13} the authors observe that this reference stream exhibits \emph{reuse locality} instead of temporal locality. Essentially, that term describes the property that the second reference to a line is a good indicator of forthcoming reuse and also that recently reused lines are more valuable than other lines reused longer.

The studies carried out in ~\cite{albericio_taco13,albericio_micro13,diaz_jp15} demonstrate, considering a large amount of multiprogrammed workloads and different multiprocessor configurations, two important aspects: first, most lines in the SLLC are dead (they will not receive any further hits during their lifetime in the SLLC) and second, most SLLC hits come from a small subset of lines. We have performed our own analysis about the behavior of the blocks evicted from the SLLC, in terms of the amount of accesses they receive before eviction, in the scenario 
%depicted in Figure~\ref{system2Simulate} but, as a starting point, employing just one core (detailed configuration is shown in Table~\ref{tab:cpuSpecs})
%As a starting point, we will employ a scenario with just one core, beingour general 
with the configuration detailed in Table~\ref{tab:cpuSpecs}, but, as a starting point, employing just one core. 
Figure~\ref{motiv_reuso} illustrates this behavior, grouping the blocks into three different categories: no reuse, just one reuse or more than one reuse (multiple reuse). 

\begin{figure}[htb]
%\resizebox{1.01\linewidth}{!}{\input{figuraReuso.tex}}
\resizebox{1.01\linewidth}{!}{\includegraphics{figure2}}
\caption{Breakdown of blocks replaced from the LLC according to the number of accesses they receive before eviction.}
\label{motiv_reuso}
\end{figure}

As shown, our experimental results confirm that most lines in the LLC are dead. Notably, around 70\% of the blocks do not receive any further access since the moment they enter the LLC. Only around 5\% of the blocks just receives one further hit (i.e. one reuse) and around 25\% exhibit more than one reuse. 
 
%Notably, the study in~\cite{albericio_micro13} establishes that on average, depending on the replacement algorithm employed, the percentage of lines stored in the SLLC that do not provide any benefit (dead lines) ranges between 65 and 83\%. In~\cite{diaz_jp15}, apart from emphasizing again that SLLCs do not employ their storage space efficiently since most of the blocks they contain are dead even when using sophisticated replacement policies, it is also highlighted that most hits in SLLC occur on blocks that have experienced \emph{multiple} (more than two) accesses during their lifetime in the SLLC, i.e., the programs exhibit reuse locality at the SLLC. 

%Consequently, implementing a cache management scheme where the blocks with just one use (the block fill) bypass the SLLC when they are evicted from the immediate lower cache level, and that just stores those blocks with reuse (at least two accesses), should allow to hold the small fraction of blocks with multiple reuses, which should translate into a higher hit rate in the SLLC and therefore an improvement of the system performance.  

Consequently, getting blocks with just one use (the block fill, so no reuse) to bypass the LLC when they are evicted from the previous level caches, and just storing blocks with reuse (at least two LLC accesses), should allow to hold the small fraction of blocks with multiple reuses, increasing the LLC hit rate and improving system performance.

Furthermore, Figure~\ref{motiv_Hitreuso} shows that most LLC hits are to blocks having multiple reuses, which together with the aforementioned fact that most blocks inserted in the LLC do not experience any reuse, highly justify the idea of a content selector based on reuse detection between private caches and LLC.

\begin{figure}[htb]
%\resizebox{1.01\linewidth}{!}{\input{figuraHitsReuso.tex}}
\resizebox{1.01\linewidth}{!}{\includegraphics{figure3}}
\caption{Breakdown of block hits at the LLC according to the number of accesses they have received before read.}
%\caption{Breakdown of block hits at the LLC according to the number of accesses they have received before read.}
\label{motiv_Hitreuso}
\end{figure}

\subsection{DASCA scheme}

In~\cite{dasca_14}, the authors propose \emph{Dead Write Prediction Assisted STT-RAM Cache Architecture} (DASCA) to predict and bypass dead writes (writes to data in last level caches not referenced again during the lifetime of corresponding cache blocks) for write energy reduction. In this work dead writes are classified into three categories: dead-on-arrival fills, dead-value fills and closing writes, as a theoretical model for redundant write elimination. On top of that they also present a dead write predictor based on a state-of-the-art dead block predictor~\cite{deadblock_10}. Thus, DASCA bypasses a write operation to the SLLC only if it is predicted not to incur extra cache misses. 

Notably, DASCA adds a specific field to each line at the private levels to store the PC (program counter) of the instructions writing a block, being this PC only updated upon write operations. Also, a PC-signature table (prediction table) is included in the design in order to make the prediction about dead writes (this table is updated according to the mechanism shown in the Table 2 of the paper itself~\cite{dasca_14}). Specifically, the mechanism samples a few cache sets and keeps track of PC information only for those sets. Predictions are made via the predictor table, made up of saturating counters similar to those used in a bimodal branch predictor, being the counters indexed by the signatures stored in the sampler entries. Thus, this PC-based predictor correlates dead blocks with addresses of memory instructions (signatures), so that different signatures are used depending on the kind of dead write predicted. 
%according to the aforementioned dead writes classification.  







==> proposal_original.tex <==
\section{Design}
\label{sec:des}

In this section we first describe the baseline system we start from. Then we describe in detail the proposed design built on top of that. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%DANI%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Propongo la siguiente organización para la Sección 3:
%1) Baseline system.
%2) The Reuse Detector.
%2.1. Reuse Detector operation.
%2.2. Implementation details.


%A continuación se detallan una a una las anteriores secciones. Primero incluyo algunos comentarios, y luego la propuesta de texto para la sección.

\subsection{Baseline system}

%Baseline system:
%Igual podemos añadir una figura estilo la del paper “FlexClusion” en la explicación de nuestra política no-inclusiva.
%En la explicación original creo que hay una errata en “the block may be referenced again from some L1 cache (in this case the block is evicted form the SLLC and sent out to the requiring private cache)”, porque en ese caso no se elimina de SLLC, solo se copia en L1 (si no sería exclusiva).

%Propuesta:
The memory hierarchy used in the baseline multi-core system includes two private levels (L1 and L2) and a last-level cache shared among all the cores (SLLC). All caches are write-back, write-allocate and LRU. L1 and L2 are inclusive while the SLLC is non inclusive. 
%where the last level cache is shared among all the cores in the system (Shared Last Level Cache, or SLLC), whereas the remaining levels are private. All these caches are managed with write-back, write-allocate policies, block replacement is carried out based on an LRU policy, and the caches use a non-inclusive policy.

The baseline management of this memory hierarchy is as follows: When a block is requested to Main Memory (MM), it is copied to the private cache levels of the requester core, but not to the SLLC. During its lifetime at the private levels of the core, the block can be requested by other cores, in which case a copy will be sent from a private L2 cache to the L1-L2 caches of the requesting core, as dictated by the directory-based coherency mechanism (please refer to Section~\ref{sec:sim} for more details on the coherency mechanism).

When a block is evicted from an L2 cache, the SLLC is checked: In case the block is not present there (either because it has not been inserted yet or because it has already been inserted and evicted by the SLLC replacement mechanism), it is inserted in the SLLC, otherwise if the block is already in the SLLC, the block is updated or just discarded, depending respectively on whether the block is dirty or clean. Thus, in our hierarchy, SLLC insertions never come from MM but from an L2, in a similar way to an exclusive policy. Note however that our mechanism differs from an exclusive policy in that, as a result of a hit in the SLLC, the block is copied to the private cache levels of the requester core, but maintained in the SLLC.

\subsection{The Reuse Detector}

%The Reuse Detector:
%Mover figura de Experimental Framework aquí.
%¿Exponer como ventaja el hecho de que solo se accede desde L1 y no desde L1+MM?
%Creo que la frase “Conversely, it does affect the time involved from the eviction of a block from a private cache until its arriving to the SLLC.” puede quitarse.
%Tampoco incluyo el comentario “The buffer is organized in a set-associative … the expulsion coverage of the RD is 64KB.” porque me parece que distrae de la explicación principal.
%El comentario sobre el Reuse Bit lo he reducido, y se amplía en la siguiente sección.

%Propuesta:
As explained earlier, several works have demonstrated that a notable percentage of the blocks inserted/updated in the SLLC are in fact useless, as they are dead-blocks (i.e. blocks which will not be referenced any more during their lifetime in the SLLC)~\cite{dasca_14,deadblock_10}. These useless blocks are harmful, as they evict other blocks which could potentially be useful in the future, and moreover, they increase the amount of writes to the SLLC, which in the context of NVMs (Non-Volatile Memories) is far from convenient, as explained in previous sections.

In this paper we leverage the technique for reducing the amount of dead-blocks inserted/updated in the SLLC~\cite{diaz_jp15} to improve the efficiency of a STT-RAM SLLC. 
In~\cite{diaz_jp15}, the authors present a proposal that, in an exclusive memory hierarchy, reduces the amount of blocks inserted in a conventional SLLC by around 90\%. We apply this technique to a different context, i.e., to a non-inclusive STT-RAM SLLC design within a memory hierarchy where L1-L2 are inclusive. The exclusion policy employed in~\cite{diaz_jp15} implies that, upon a SLLC hit, the block is copied to the private cache levels and removed from the SLLC. In our case, the block is inserted in the SLLC at the end of its usage in the private caches and remains in the SLLC until eviction.
For our purpose, we include an intermediate element between each private L2 cache and the SLLC (Figure~\ref{system2Simulate}). A block evicted from the private L2 caches is targeted to the corresponding element, which we denote as Reuse Detector (RD), instead of accessing directly to the SLLC as it would do in the baseline system. The RD decides whether to send the block to the SLLC or not (i.e. to bypass the shared last-level cache), by means of a prediction about the future usefulness of the block. We must highlight that, being the RD out of the block request path to the SLLC, it does not impact the SLLC hit or miss latencies.


\begin{figure}[htb]
%\resizebox{1\linewidth}{!}{\input{figFramework2.tex}}
%\resizebox{1\linewidth}{!}{\input{figFramework2.tex}}
\includegraphics{figure4}	
\caption{Placement of a Reuse Detector between each private L2 level and STT-RAM SLLC.}
\label{system2Simulate}
\end{figure}

%\begin{figure}[ht!]
%     \begin{center}
%        \subfigure[ ]{%
%            \label{system2Simulate}
%            %\fbox{
%            \resizebox{0.5\linewidth}{!}{\input{figures/figFramework.tex}}
%            %}
%        }%
		 %\quad
%        \subfigure[ ]{%
%           \label{system2Simulate2}
%           %\fbox{
%           \resizebox{0.5\linewidth}{!}{\input{figures/figFramework2.tex}}
%           %}
%        }
%    \end{center}
%    \caption{(a) Placement of a Content Selector (CS) between the private levels and STT-RAM SLLC. The CS is a generic block that represents the algorithm used for filter the blocks to SLLC. (b) The CS in changed by our Reuse Detector.}%
%\end{figure}

For accomplishing the RD prediction, we apply Albericio\textquotesingle s concept of reuse locality~\cite{albericio_taco13,albericio_micro13}. As such, if the evicted block from the L2 has never been requested to the SLLC since the time it entered the cache hierarchy (i.e. it has never been reused at the SLLC), the block is predicted as a dead-block and thus it bypasses the SLLC, directly updating MM (if the block is dirty) or being just discarded (if it is clean). Otherwise, if the block has been reused (i.e. it has been requested to the SLLC at least once since the time it entered the cache hierarchy) and thus it is predicted as a non-dead-block, it is inserted/updated in the SLLC.

The RD consists of a FIFO buffer and some management logic. The buffer stores the tag addresses of the blocks evicted by the private levels in order to maintain their reuse state. Moreover, an extra bit, called \emph{reuse bit}, is added to each cache line in the private levels. This bit distinguishes if the block was inserted at the private cache levels from the SLLC or from another private cache level (\emph{reuse} bit is 1), or main memory (\emph{reuse} bit is 0). In the following sections, we analyze in detail the Reuse Detector operation and implementation.


\subsubsection{Reuse Detector operation}
%Reuse Detector operation:

%Propuesta:
As we said in a previous section, our proposal aims to reduce the amount of writes to the STT-RAM SLLC and to improve the management of SLLC blocks, which translate into system performance improvement and energy consumption reduction on the system.

%Figure~\ref{fig:flow1} shows a flow diagram of a block request to a private cache. In a coherent system like the one we are simulating, a request to a private cache can come from its associated core or from another core due to a coherency request. If the request hits in a private cache and it is performed by a core different to the one associated to this private cache, or a request hits in SLLC, the access is considered an SLLC reuse, and the reuse bit for the block is set. Instead, if a request from a core hits in its associated private cache, the reuse bit is kept unchanged.

Figure~\ref{fig:flow1} shows a flow diagram of a block request from a core to its associated private caches. If the request hits in L1 or L2 the reuse bit is untouched, and the block is copied in L1 if it was not there (inclusive policy). Otherwise, the request is forwarded to the SLLC. If the access hits in the SLLC, the block is provided to the core and copied in the private levels with the reuse bit set. If the access misses in the SLLC but the coherency mechanism informs that the block is present in another private cache, the block is provided by that cache. In this case, the access is recognized as a reuse, so the reuse bits are also set. Finally, if no copy of the block is present in the cache hierarchy, it is requested to MM and copied in L1-L2 with the reuse bit unset.

\begin{figure}[htb]
%%%%%\resizebox{0.8\linewidth}{!}{\input{figures/flowchartDetector2.tex}}
%\resizebox{1\linewidth}{!}{\input{flowchartDetector1.tex}}
\resizebox{\linewidth}{!}{\includegraphics{figure5}}
\caption{Block request and reuse bit management.}
\label{fig:flow1}
\end{figure}

Figure~\ref{fig:flow2} shows a flow diagram of a block eviction from an L2 cache (if required, the corresponding L1 cache is invalidated). When a block is evicted from a last private level cache, its reuse bit is checked. If the reuse bit is set, it means that the block was inserted into the private caches either from the SLLC or from another private cache after checking the SLLC and the coherency mechanism. In any case, the block is considered as having been reused, and it should be inserted in the SLLC (if not present yet) or just updated (if the block is dirty but it is already present in the SLLC). Note that if the block is clean and already present in the SLLC, it can just be discarded. If the reuse bit is unset (i.e. the block was brought into the private caches directly from main memory) but the block\textquotesingle s tag is found in the RD buffer, the block is also considered as having been reused, and thus it is handled as in the previous situation. Finally, if the reuse bit is unset and its tag is not present in the RD buffer, it means that the block is considered as not having been reused yet. Based again on Albericio\textquotesingle s observations~\cite{albericio_taco13,albericio_micro13}, the block should bypass the SLLC, as it is predicted as a dead-block, and it should be sent to MM (if the block is dirty) or just discarded (if it is clean). Note that in all cases the coherency mechanism must be updated.  


\begin{figure}[htb]
%\resizebox{0.8\linewidth}{!}{\input{figures/flowchartDetector2.tex}}
%\resizebox{1\linewidth}{!}{\input{flowchartDetector2.tex}}
\resizebox{\linewidth}{!}{\includegraphics{figure6}}
\caption{Block eviction from a private cache and SLLC insertion.}
\label{fig:flow2}
\end{figure}


\subsubsection{Example}
For the sake of clarifying the Reuse Detector operation, in this subsection we provide a straightforward example illustrating the flow of five memory blocks (A, B, C, D and E) through the different cache levels under a given access pattern. In this example, we consider a dual-core system ($Core_{0}$ and $Core_{1}$) with private first level caches ($L1_{0}$ and $L1_{1}$), a shared second level cache (SLLC), and the corresponding Reuse Detectors between both cache levels. In the example we assume a simplified configuration where: 1) direct-mapped L1s, 2-way set associative RDs and 4-way set associative SLLC are considered; 2) all memory blocks map to the same L1 frame and to the same RD and SLLC set; and 3) initially, all caches and RDs are empty. Next, we detail the access sequence of our example and show the contents of the memory hierarchy after each access in Figure~\ref{tableExampleReuseDet}. Note that we specify as a subindex the dirty bit followed by the reuse bit ($X_{d,r}$) for each block \emph{X} in the private cache levels, and only the dirty bit ($X_d$) for each block \emph{X} in the SLLC.  

\input{TableExampleProposedPolicies.tex}

\begin{enumerate}
\item $Core_0$ requests a word within block A for reading: The access misses in $L1_0$, it is forwarded to the SLLC, and given that the access to SLLC also misses and the block is not present in any other private cache, it is forwarded to MM. According to Figure~\ref{fig:flow1}, block A is copied to $L1_0$ with its reuse bit unset, and the requested word is provided to $Core_0$. 
%\item $Core_0$ requests a word within block A for writing: The access hits in $L1_0$, where the block is marked as dirty. Besides, according to Figure~\ref{fig:flow1}, the reuse bit is kept unchanged.
\item $Core_1$ requests a word within block A for reading: The access misses in $L1_1$ and SLLC. However, the coherency mechanism informs that the block is at $L1_0$, so the request is forwarded to that cache. According to Figure~\ref{fig:flow1}, the block is copied to $L1_1$ and both reuse bits are set, as we recognize this access as an SLLC reuse. 
\item $Core_1$ requests a word within block B for reading: The access misses in $L1_1$ and SLLC, and the block is not present in any other private cache, so the request is forwarded to MM. According to Figure~\ref{fig:flow1}, block B is copied to $L1_1$ (replacing block A) with its reuse bit unset, and the requested word is provided to $Core_1$. According to Figure~\ref{fig:flow2}, given that block A had its reuse bit set, it is inserted into the SLLC. 
\item $Core_1$ requests a word within block C for reading: Block C is inserted in $L1_1$ and block B is replaced. As the reuse bit of block B was unset and its tag was not in $RD_1$, according to Figure~\ref{fig:flow2} the tag is stored in $RD_1$ and, given that the block is clean, it is not inserted in the SLLC but just discarded. 
\item $Core_1$ requests a word within block B for reading: This access is handled analogously to the previous access. 
%Block B is copied to $L1_1$ (replacing another block) with its reuse bit unset.
\item $Core_1$ requests a word within block D for reading: Block D is inserted in $L1_1$ and block B is replaced. As the reuse bit of block B was unset but its tag was present in $RD_1$, according to Figure~\ref{fig:flow2} block B is inserted in the SLLC.
\item $Core_0$ writes to a word within block A: The access hits in $L1_0$. The dirty bit for the block is set.
\item $Core_0$ requests a word within block E for reading: Block E is inserted in $L1_0$ and block A is replaced. As the dirty bit of block A is set and A is already present in the SLLC, the block is updated at this level.
\end{enumerate}


\subsubsection{Implementation details}
\label{subsubsec:details}
%Implementation details:
%He eliminado un comentario sobre los parámetros de diseño y sobre que size era el parámetro principal y que el buffer tiene que ser suficientemente grande. Se puede llevar a entorno o experimentos.
%La Expulsion Coverage (también lo he quitado, con la idea de llevarlo más adelante) no la entiendo muy bien, ¿no es más que el tamaño del buffer en Bytes?
%El Storage Overhead y la Figura 4 los he quitado, me ha parecido mejor llevarlos a la Sección V o la VI.

%Propuesta:
Although a typical set-associative design could be used for the RD implementation, where a whole block tag, a validity bit and some information related with the replacement policy is included for each line, as in~\cite{diaz_jp15} we use two techniques aimed at reducing the required space: sectoring and compression.
A sector is a set of consecutive memory blocks aligned to the sector size. Storing sector tags in the RD allows to merge in a single line of the RD the information related with several blocks. Note that for each entry it is necessary to store a presence bit. For example, with a sector comprising 4-blocks, each line is made up of a tag derived from the sector address, a validity bit, some bits storing the replacement state and 4 presence bits.

The compression of the tags is achieved based on the following process: let \emph{t} be the amount of bits of the full tag and \emph{c} the amount of bits of the compressed tag, being t$>$c. We first divide the full tag into several pieces, each of size \emph{c} (the last piece is filled with \emph{0s} if necessary). Then, we \emph{xor} all the pieces, obtaining the compressed tag. Note that each compressed tag is shared among various sectors, thus false positives are possible where non-reused blocks are delivered to the SLLC. This situation does not cause a functional problem, but it may degrade system performance, so the value of \emph{c} must be chosen carefully.


As for the storage overhead of the RD implementation, i.e., the total amount of extra bits required compared to the baseline, we need the following hardware: The RD has 1024 sets and 16 ways (our simulations reveal that this value provides similar performance to that of higher associativity values), and a sector size of 2 blocks. Each RD entry requires 14 bits (10 for the compressed tag, 2 for the block presence, 1 for the replacement policy and 1 validity bit) as Figure~\ref{fig:rd_block} illustrates. Given that the amount of entries in the RD is 8K, the total extra storage required per core is 14 KB, which represents a negligible 1.3\% of an 1MB last level cache. 

%Note also that although the RD is a monolithic element (blocks evicted from any last private cache access it), actually the amount of entries in the RD is limited for each core

\begin{figure}[htb]
%\resizebox{0.8\linewidth}{!}{\input{detectorBlock.tex}}
\includegraphics{figure8}	
\caption{Reuse Detector entry.}
\label{fig:rd_block}
\end{figure}

Finally, as RD replacement policy we use a 1-bit FIFO. Again based on our simulations, this scheme delivers a similar performance as other policies that would require more storage. In a FIFO policy, age information is updated only when a new address is inserted, and not during subsequent hits. This approach is fully consistent with the main RD buffer goal of detecting the first reuse of a block.


\subsection{Reuse Detector vs DASCA}

In this section we briefly discuss the main differences between the RD approach and the DASCA scheme, which will be further extended and analyzed in the evaluation section. As for the operation of both approaches, note that the DASCA mechanism tries to predict dead writes based on a PC-based predictor. For this purpose, the PC signature of each block that accesses the SLLC must be recorded. Conversely, the RD scheme tries to predict dead-blocks based on their reuse state. Our prediction is based on the addresses of the accessed data instead of the instruction addresses used in DASCA. Also, in our approach we directly store the mentioned addresses while in the DASCA scheme the authors employ a PC-signatures table which is trained by an auxiliary cache that works in parallel with the conventional cache.

Focusing on the specific implementation of the DASCA scheme for the evaluation of this proposal, it is worthy to note that our approach employs a memory hierarchy where L1 and L2 are inclusive while the SLLC (L3) is non inclusive, whereas the original DASCA scheme is evaluated in~\cite{dasca_14} employing a memory hierarchy with just two cache levels and assuming non-inclusive caches by default, although the authors also propose a bypassing scheme that supports both inclusive and non-inclusive caches. Therefore, and looking for a fair comparison between RD and DASCA, we implement DASCA using exactly the same three-level non-inclusive non-exclusive hierarchy employed in the RD approach. As a result of that, the only high-level change with respect to the original version of DASCA lies in that one of the three possible cases they use to classify the dead writes (``dead-value fills'', blocks that receive a writeback request from lower-level caches right after the block is filled, but before any read operation, i.e., the filled block data are overwritten before being read), can not exist since they are removed by the inclusion mechanism we employ in our approach. Notably, this is due to the fact that, in our configuration, all the insertions in the SLLC are motivated by an L2 block eviction, and, as L1 and L2 are inclusive, these evicted blocks are only located in the SLLC after the eviction from L2. If after that the processor generates a write request on one of these blocks, a write hit occurs, and consequently the block is copied to the private cache levels and therefore this block in the SLLC can not be written again in the SLLC before being read. Hence, we consider this evaluation as fair, since this way we are evaluating DASCA under the same conditions as our approach, so that we are not giving an advantage to our RD by the fact that it directly avoids the ``dead-value fills'' with the inclusiveness management. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ANTERIOR FERNANDO%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Overview}

%The starting point is a shared lat-level cache which content is in non-inclusion and non-exclusion with the contents of the private caches (L1) of each processor. In order to maintain the coherence in the memory hierarchy there is a directory in the SLLC (L2, please refer to Section 5 for the detailed experimental framework) that tracks the state and location for each cache block. In our design, those requested blocks arriving from the main memory are copied in the private cache of the requiring processor but not in the SLLC. In the event a block is evicted from a private cache, it is sent out to the SLLC for its storage. Being located at the SLLC the block may be referenced again from some L1 cache (in this case the block is evicted form the SLLC and sent out to the requiring private cache) or it may be replaced by other block that requires space to be filled.

%Our proposal is to include in the aforementioned design an intermediate element at the output of each L1 cache, between each of them and the SLLC. All the blocks evicted from a L1 cache are targeted to this element, that we denote as \emph{Reuse Detector} (RD). We must note that being the RD out of the block request path to the SLLC, the delay added does not impact the hit or miss latencies in the SLLC. Conversely, it does affect the time involved from the eviction of a block from a private cache until its arriving to the SLLC.

%The RD must decide whether to send the block to the SLLC or not, i.e., to bypass the last-level cache. The decision is based on the next criteria: if the evicted block exhibits just one usage, it bypasses the LLC; if it presents one or more reusages, the bypass is not performed.  Note that the SLLC nor the directory requires any structural changes in order to adapt them to the RD mechanism. By contrast, some changes in the coherence protocol and the control logic are required to deal with the eventual bypass.


%\subsection{The Reuse Detector}  

%The RD is formed by a buffer recording blocks addresses and by its management logic. The goal of the buffer is to store the addresses of the blocks that reach the detector, in order to determine for each block if it has been evicted from a L1 cache for the first time or it has been already evicted previously. A first eviction eviction implies that no reuse exists in the L1 cache while next evictions means that reuse is occurring.

%The buffer is organized in an set-associative fashion, and the buffer features like size, associativity and replacement policies are design variables. The buffer size is its most important property, since in order to be effective the buffer must be large enough to contain a significant part of the blocks addresses between their use and reuse. We define the \emph{expulsion coverage} as the overall memory space occupied by the evicted blocks for which the RD is able to track at any given time. For instance, if the RD is able to track 1024 memory blocks, and each block is 64 bytes long, the expulsion coverage of the RD is 64KB.

%In order to detect the reuse, the RD also employs the info about whether the block was sent to a private L1 cache from main memory or it comes from a hit in the SLLC. The provenience from the SLLC also means that a reuse occurs. This information recorded in the L1 cache, using a per line added bit (\emph{reuse bit}), so that when the block is evicted from an L1 cache, this bit is included in the message addressed to the RD. 


%\subsection{Reuse Detector operation} 

%Figure~\ref{fig:flow1} recaps the our proposal flowchart under a block request to a private L1 cache.  


%\begin{figure}[htb]
%\resizebox{0.8\linewidth}{!}{\input{figures/flowchartDetector1.tex}}
%\caption{Simulated system, for all caches a 64 bytes/block is used.}
%\label{fig:flow1}
%\end{figure}

%Figure~\ref{fig:flow2} illustrates the flowchart followed when a block is evicted from an L1 cache.

%\begin{figure}[htb]
%\resizebox{0.8\linewidth}{!}{\input{figures/flowchartDetector2.tex}}
%\caption{Simulated system, for all caches a 64 bytes/block is used.}
%\label{fig:flow2}
%\end{figure}

%Next we detail the various actions the Reuse Detector takes. When a block is evicted from an L1 cache it targets the RD, where the reuse bit is inspected in order to identify if the block comes from the SLLC. If so, this implies that the block exhibits reuse at this level, so it is marked for storage in the SLLC. If the block comes from the main memory, the buffer is checked in order to find the block address: if there is not a match, it implies that it is the first time the block is evicted from the L1, so it does not exhibit reuse and it is marked for bypass the SLLC and its address is inserted in the buffer; if a match occurs, it means that it is the second or more time that the block stayed in an L1 cache, so it presents reuse and therefore the block is marked for storage in the SLLC.

%Finally, if the block is labeled for storage in the SLLC, it is send out to the last-level cache. Otherwise, if it is marked for bypassing the SLLC, the operation depends on the dirtiness of the block, i.e., if the block has been modified during its lifetime in the private L1 cache or not. If it is dirty, the block is directly send to the main memory for its writing, but if the block is clean, a control message is send in order to update the directory.  

%\subsection{Implementation details}

%At first glance, the buffer of the RD can be implemented in a set-associative fashion, including the tag associated to the block address, a validity bit and the info required for the the replacement policy. Each line of the RD cache will store a block address. Although this design is both straightforward and efficient, it has the drawback to require too much storage space. For this reason we  propose to employ two techniques aimed at reduce the required space: to store the tags by sector address instead of by block address, and to compress the tags to store. We refer to a sector as a set of consecutive memory blocks aligned to the sector size. Storing the tags in the RD by sector address allows to record in each line of the RD buffer the information of various addresses corresponding to consecutive memory blocks. For each block it is necessary to hold one presence bit. For example, with a 4-blocks sector, each line consists of a tag (derived from the sector address), one validity bit, the bits corresponding to the replacement policy and 4 bits of presence.    

%The compression of the tags to record pursues to store less bits for the tag present on each line, while maintaining a significant ability to discriminate between sectors. The process works as follows: if we denote as \emph{t} the amount of bits of the full tag and as \emph{c} the amount of bits of the compressed tag, we take the \emph{t} bits and we split them among various pieces of \emph{c} bits. The last piece is filled with \emph{0s}, if necessary, until the corresponding size. Then, the \emph{xor} operation considering all the pieces is performed, obtaining a single value of \emph{c} bits, which is the stored value. Employing compressed tags could lead to \emph{false positives}, since various sectors of the privates L1 caches do share the same compressed tag value. This implies the detection of false reuses, and therefore the delivery to the SLLC of actually non-reused blocks. This blocks do not cause functional problems, but they may degrade the system performance. In order to mitigate this constraint, enough bits must be hold. The particular value depends on the size and associativity of the buffer.  


%\begin{figure}[htb]
%\resizebox{0.8\linewidth}{!}{\input{figures/detectorBlock.tex}}
%\caption{Reuse Detector block.}
%\label{fig:rd_block}
%\end{figure}

   
%The RD buffer employs 1-bit FIFO as replacement policy. Our simulations reveal that this implementation delivers similar RD performance to that of other policies that require more storage space. The FIFO scheme involves that the age information is updated only when an address is inserted, and not during subsequent hits. This approach is fully consistent with the main task of the RD, which is to detect the first reuse of a block. For the following reuses, the key aspect is the information about the block provenience from the SLLC, though the presence in the buffer is also employed in a complementary way for even the block has been evicted from the SLLC.

%In our experimental framework we employ a 16-ways RD buffer. Our simulations reveal that this value provides a  similar performance to that of other high associativity values. 

%\subsection{Storage overhead}

%In this section we compute the storage overhead of the RD implementation, i.e., the total amount of extra bits required compared to the baseline. Recall that the RD implementation also includes its management logic to operate. 

%The chosen RD configuration has a expulsion coverage of 2 MB, with 1024 sets of associativity 16, a sector size of 2 blocks and employs tags of 10 bits. Each RD entry requires 14 bits (10 for the tag, 2 for the block presence, 1 for the replacement policy and 1 validity bit). The amount of entries in the RD is 16K. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> rarr_original.tex <==
\usepackage[cmex10]{amsmath}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

\usepackage{mdwmath}
\usepackage{eqparbox}
\usepackage[tight,footnotesize]{subfigure}
%\PassOptionsToPackage{subfigure}{tocloft}
% *** FLOAT PACKAGES ***
\usepackage{fixltx2e}
\usepackage{dblfloatfix}
\usepackage{lscape,longtable}
% *** PDF, URL AND HYPERLINK PACKAGES ***
\usepackage{url}
\usepackage{balance}
\pdfpageattr {/Group << /S /Transparency /I true /CS /DeviceRGB>>}   
\usepackage{multicol}
%\usepackage{multirow}
\usepackage[x11names,table]{xcolor}
\usepackage{color, colortbl}
%\usepackage{upquote}

%\usepackage{float}
\usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
\newfloatcommand{capbtabbox}{table}[][\FBwidth]
\usepackage{blindtext}
\usepackage{textcomp}
%\usepackage[cmyk]{xcolor}
%\usepackage{longtable}
%\usepackage[section]{placeins}
%\setcounter{topnumber}{2}
%\setcounter{bottomnumber}{2}
%\setcounter{totalnumber}{4}
%\renewcommand{\topfraction}{0.85}
%\renewcommand{\bottomfraction}{0.85}
%\renewcommand{\textfraction}{0.15}
%\renewcommand{\floatpagefraction}{0.7}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{graphicx}
\usepackage{lmodern}
\usepackage{tikz}
\usepackage{pgfplots,pgfplotstable}
%\usepackage{filecontents}
\usepackage{slashbox}

%\usepackage{etoolbox}
%\usepackage{framed}
%\usepackage{enumitem}
\renewcommand\labelenumii{\arabic{enumii}.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%\usetikzlibrary{arrows,decorations.markings}
%\usetikzlibrary{arrows,positioning,chains}
%\usetikzlibrary{shapes,snakes}
%\usetikzlibrary{positioning}
%\usetikzlibrary{shadows}
%\usetikzlibrary{patterns}
%\usetikzlibrary{calc,backgrounds}
%%\usepackage[active,tightpage]{preview}
\usetikzlibrary{chains,calc,backgrounds,arrows,trees,shapes,snakes,shadows,matrix,fit,patterns,positioning,automata,decorations.pathmorphing,decorations.pathreplacing}

\newcolumntype{L}{>{\centering\arraybackslash}m{3cm}}
%***************************Blocks*************************************************
%**********************************************************************************

%ESto es para que solo aparezca un bloque en las leyendas de las figuras
%\pgfplotsset{compat=1.11,
%    /pgfplots/ybar legend/.style={
%    /pgfplots/legend image code/.code={%
%       \draw[##1,/tikz/.cd,yshift=-0.25em]
%        (0cm,0cm) rectangle (3pt,0.8em);},
%   },
%}

\makeatletter
\tikzset{nomorepostaction/.code=\let\tikz@postactions\pgfutil@empty}
\makeatother

\newcommand{\CommonLineTextFormat}[3]
{
  \begin{minipage}{#3}
    \centering
%      {\textbf{#1} \hfill #2}%
    %  \linebreak \linebreak
      {\textbf{#1}}%
      \linebreak \linebreak
      {{#2}}
  \end{minipage}
}
\newcommand{\LineTextFormat}[3]
{
  \CommonLineTextFormat{\LARGE {#1}}{#2}{#3}
} 

\newcommand{\LineTextFormatLarge}[3]
{
  \CommonLineTextFormat{\Large {#1}}{#2}{#3}
} 

\definecolor{Maroon}{rgb}{0.8, 0.0, 0.0}
\definecolor{gray}{rgb}{0.3, 0.3, 0.3}

\definecolor{rrrreducm}{cmyk}{0,1,0.71,0.21}
\definecolor{rrrblue}{cmyk}{0.86,0.33,0,0.50}
\definecolor{rrrgreen}{cmyk}{0.86,0.3,0.86,0.5}
\definecolor{rrrsilver}{cmyk}{0,0,0,0.1}
\definecolor{rrrsilver2}{cmyk}{0,0,0,0.07}
\definecolor{rrrred}{cmyk}{0,0.88,0.94,0.38}
\definecolor{rrrred2}{cmyk}{0,0.80,0.81,0.25}
\definecolor{rrrgreen2}{cmyk}{0.35,0,0.67,0.41}
\definecolor{rrrgreen3}{cmyk}{0.43,0,0.60,0.60}
\definecolor{rrrgray}{cmyk}{0,0,0,0.50}
%\definecolor{rrrorange}{cmyk}{0,0.50,1,0}
%\definecolor{rrrorange}{cmyk}{0,0.66,0.87,0}
\definecolor{rrrorange}{cmyk}{0,0.62,0.99,0}
\definecolor{rrryellow}{cmyk}{0,0.09,0.62,0.11}
\definecolor{rrrturquoise}{cmyk}{0.93,0,0.21,0.13}
\definecolor{rrrpurple}{cmyk}{0.33,0.87,0,0.06}
\definecolor{rrrbrown}{cmyk}{0,0.67,0.67,0.50}
\definecolor{rrrinvisible}{cmyk}{0,0,0,0}
\definecolor{rrrsgilightblue}{cmyk}{0.88,0.44,0,0.45}

\tikzstyle{LineFill} = [top color=rrrsilver2, bottom color=rrrgreen2!70, draw=rrrgreen2!90!black!100, drop shadow]    
\tikzstyle{LineFillSilver} = [top color=rrrsilver2, bottom color=rrrgray!70, draw=rrrgray!90!black!100, drop shadow] 
\tikzstyle{Line} = [draw=rrrgreen2, LineFill, minimum width=2cm, minimum height=2cm, node distance=3cm]  
\tikzstyle{LineSilver} = [draw=rrrgreen2, LineFillSilver, minimum width=2cm, minimum height=2cm, node distance=2cm] 

\tikzstyle{LineLabel} = [font={\sffamily\LARGE}, node distance=3cm]
\tikzstyle{LineLabel2} = [node distance=3cm]

\tikzstyle{LineFillRed} = [preaction={
				top color=rrrsilver2, bottom color=rrrred!70, draw=rrrred!70!black!100, drop shadow},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrred!70!rrrsilver2!100,
            pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrred!70, draw=rrrred!70!black!100, drop shadow]     
\tikzstyle{LineP} = [draw=black, LineBlue2, minimum width=1.75cm, minimum height=1.75cm, node distance=1.75cm]
\tikzstyle{LineFill4} = [top color=white, bottom color=rrrgreen!30, draw=rrrgreen2!60!black!100, drop shadow]     
\tikzstyle{Line4} = [draw=black, LineFill4, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm] 
\tikzstyle{LineP4} = [draw=black, LineFill4, minimum width=1.75cm, minimum height=1.75cm, node distance=1.75cm]


\tikzstyle{LineRed} = [draw=rrrred, LineFillRed, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm]  
\tikzstyle{LineFillRed2} = [top color=rrrsilver2, bottom color=rrrred2!70, draw=rrrred2!70!black!100, drop shadow]     
\tikzstyle{LineRed2} = [draw=rrrred2, LineFillRed2, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm]  
\tikzstyle{LinePRed2} = [draw=rrrred2, LineFillRed2, minimum width=1.75cm, minimum height=1.75cm, node distance=1.75cm]
\tikzstyle{LineFillGreen} = [preaction={
				top color=rrrsilver2, bottom color=rrrgreen!90, draw=rrrgreen!90!black!100, drop shadow},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrgreen!90!black!100,
            pattern=north east lines
        }
    }]%top color=rrrsilver2, bottom color=rrrgreen!90, draw=rrrgreen!90!black!100, drop shadow]     
\tikzstyle{LineGreen} = [draw=rrrGreen, LineFillGreen, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm] 
\tikzstyle{LineFillBlue} = [top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100, drop shadow]     
\tikzstyle{LineBlue} = [draw=rrrblue, LineFillBlue, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm] 
\tikzstyle{LineFillBlue2} = [top color=rrrsilver2, bottom color=rrrblue!30, draw=rrrblue!70!black!100, drop shadow]     
\tikzstyle{LineBlue2} = [draw=rrrblue, LineFillBlue2, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm] 
\tikzstyle{LineFillOrange} = [top color=rrrsilver2, bottom color=rrrorange!90, draw=rrrorange!90!black!100, drop shadow]     
\tikzstyle{LineOrange} = [draw=rrrorange, LineFillOrange, minimum width=2.75cm, minimum height=2.75cm, node distance=2.75cm] 
\tikzstyle{LineFillrrrsgilightblue} = [top color=rrrsilver2, bottom color=rrrsgilightblue!70, draw=rrrsgilightblue!70!black!100, drop shadow]     
\tikzstyle{LineFillBlue} = [top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100, drop shadow]     




\tikzstyle{LineFillRedTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrred2!70, draw=rrrred2!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrred2!70!rrrsilver2!100,
            pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrred2!70, draw=rrrred2!70!black!100]     
\tikzstyle{LineFillGreenTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrgreen!70, draw=rrrgreen!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrgreen!70!black!100,
            pattern=north east lines
        }
    }]%top color=rrrsilver2, bottom color=rrrgreen!70, draw=rrrgreen!70!black!100]     
\tikzstyle{LineFillBlueTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrblue!70!black!100,
            pattern=horizontal lines
        }
    }]%top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100] 
\tikzstyle{LineFillOrangeTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrorange!70, draw=rrrorange!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrorange!70!black!100,
            pattern=north west lines
        }
    }]%top color=rrrsilver2, bottom color=rrrorange!70, draw=rrrorange!70!black!100] 
\tikzstyle{LineFillYellowTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrryellow!70, draw=rrryellow!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrryellow!70!black!100,
            pattern=vertical lines
        }
    }]%top color=rrrsilver2, bottom color=rrryellow!70, draw=rrryellow!70!black!100] 
\tikzstyle{LineFillTurquoiseTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrturquoise!70, draw=rrrturquoise!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrturquoise!70!black!100,
            pattern=grid
        }
    }]%top color=rrrsilver2, bottom color=rrrturquoise!70, draw=rrrturquoise!70!black!100] 
\tikzstyle{LineFillPurpleTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrpurple!70, draw=rrrpurple!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrpurple!70!black!100,
            pattern=dots
        }
    }]%top color=rrrsilver2, bottom color=rrrpurple!70, draw=rrrpurple!70!black!100] 
\tikzstyle{LineFillBrownTiny} = [preaction={
				top color=rrrsilver2, bottom color=rrrbrown!70, draw=rrrbrown!70!black!100},
    every path/.style={
        postaction={
        		nomorepostaction,        
	         draw=rrrbrown!70!black!100,
            pattern=crosshatch
        }
    }]%top color=rrrsilver2, bottom color=rrrbrown!70, draw=rrrbrown!70!black!100]     

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%Figura Politicas PCM todos los benchmarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzstyle{LineFillRedTinyND} = [preaction={
                top color=rrrred2!70, bottom color=rrrred2!70, draw=rrrred2!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrred2!70,
            pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrred2!70, draw=rrrred2!70!black!100]     
\tikzstyle{LineFillGreenTinyND} = [preaction={
                top color=rrrgreen!70, bottom color=rrrgreen!70, draw=rrrgreen!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrgreen!70,
            pattern=north east lines
        }
    }]%top color=rrrsilver2, bottom color=rrrgreen!70, draw=rrrgreen!70!black!100]     
\tikzstyle{LineFillBlueTinyND} = [preaction={
                top color=rrrblue!70, bottom color=rrrblue!70, draw=rrrblue!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrblue!70,
            pattern=horizontal lines
        }
    }]%top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100] 
\tikzstyle{LineFillOrangeTinyND} = [preaction={
                top color=rrrorange!70, bottom color=rrrorange!70, draw=rrrorange!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrorange!70,
            pattern=north west lines
        }
    }]%top color=rrrsilver2, bottom color=rrrorange!70, draw=rrrorange!70!black!100] 
\tikzstyle{LineFillYellowTinyND} = [preaction={
                top color=rrryellow!70, bottom color=rrryellow!70, draw=rrryellow!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrryellow!70,
            pattern=vertical lines
        }
    }]%top color=rrrsilver2, bottom color=rrryellow!70, draw=rrryellow!70!black!100] 
\tikzstyle{LineFillTurquoiseTinyND} = [preaction={
                top color=rrrturquoise!70, bottom color=rrrturquoise!70, draw=rrrturquoise!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrturquoise!70,
            pattern=grid
        }
    }]%top color=rrrsilver2, bottom color=rrrturquoise!70, draw=rrrturquoise!70!black!100] 
\tikzstyle{LineFillPurpleTinyND} = [preaction={
                top color=rrrpurple!70, bottom color=rrrpurple!70, draw=rrrpurple!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrpurple!70,
            pattern=dots
        }
    }]%top color=rrrsilver2, bottom color=rrrpurple!70, draw=rrrpurple!70!black!100] 
\tikzstyle{LineFillBrownTinyND} = [preaction={
                top color=rrrbrown!70, bottom color=rrrbrown!70, draw=rrrbrown!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrbrown!70,
            pattern=crosshatch
        }
    }]%top color=rrrsilver2, bottom color=rrrbrown!70, draw=rrrbrown!70!black!100]     
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ESto para las cuatro tramas que quiere Pablo
\tikzstyle{LineFillRedTiny2} = [preaction={
                top color=rrrred2!70, bottom color=rrrred2!70, draw=rrrred2!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrred2!70!rrrsilver2!100,
            pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrred2!70, draw=rrrred2!70!black!100]     
\tikzstyle{LineFillGreenTiny2} = [preaction={
                top color=rrrgreen!30, bottom color=rrrgreen!30, draw=rrrgreen!30!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrgreen!30!black!100,
            pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrgreen!70, draw=rrrgreen!70!black!100]     
\tikzstyle{LineFillBlueTiny2} = [preaction={
                top color=rrrblue!100, bottom color=rrrblue!100, draw=rrrblue!100!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrblue!100!black!100,
            pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100] 
\tikzstyle{LineFillYellowTiny2} = [preaction={
                top color=rrryellow!5, bottom color=rrryellow!5, draw=rrryellow!5!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrryellow!5!black!100,
            pattern=crosshatch dots %vertical lines
        }
    }]%top color=rrrsilver2, bottom color=rrryellow!70, draw=rrryellow!70!black!100]
\tikzstyle{LineFillRedTiny3} = [preaction={
                top color=rrrred2!70, bottom color=rrrred2!70, draw=rrrred2!70!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrred2!70!rrrsilver2!100,
            %pattern=crosshatch dots
        }
    }]%top color=rrrsilver2, bottom color=rrrred2!70, draw=rrrred2!70!black!100]     
\tikzstyle{LineFillGreenTiny3} = [preaction={
                top color=rrrgreen!30, bottom color=rrrgreen!30, draw=rrrgreen!30!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrgreen!30!black!100,
            %pattern=north east lines
        }
    }]%top color=rrrsilver2, bottom color=rrrgreen!70, draw=rrrgreen!70!black!100]     
\tikzstyle{LineFillBlueTiny3} = [preaction={
                top color=rrrblue!100, bottom color=rrrblue!100, draw=rrrblue!100!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrrblue!100!black!100,
            %pattern=horizontal lines
        }
    }]%top color=rrrsilver2, bottom color=rrrblue!70, draw=rrrblue!70!black!100] 
\tikzstyle{LineFillYellowTiny3} = [preaction={
                top color=rrryellow!5, bottom color=rrryellow!5, draw=rrryellow!5!black!100},
    every path/.style={
        postaction={
                nomorepostaction,        
             draw=rrryellow!5!black!100,
            %pattern=crosshatch dots %vertical lines
        }
    }]%top color=rrrsilver2, bottom color=rrryellow!70, draw=rrryellow!70!black!100]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzstyle{AlertFill} = [top color=white, bottom color=rrrgreen!30, draw=rrrgreen!60!black!100, drop shadow]   

\tikzstyle{blockTagFill} = [top color=white, bottom color=rrrblue!30, draw=rrrblue, node distance=1cm, drop shadow]
\tikzstyle{blockTag} = [ellipse, draw=black, blockTagFill, minimum width=2cm, minimum height=2cm]  
\tikzstyle{blockTagFill2} = [top color=white, bottom color=rrrgreen!30, draw=rrrgreen!60!black!100, node distance=1cm, drop shadow]
\tikzstyle{blockTag2} = [ellipse, draw=rrrgreen!50, blockTagFill2, minimum width=2cm, minimum height=2cm] 
\tikzstyle{blockTagFillGray} = [top color=white, bottom color=rrrgray!30, draw=rrrgray!60!black!100, node distance=1cm, drop shadow]
\tikzstyle{blockTagGray} = [ellipse, draw=rrrgray!50, blockTagFillGray, minimum width=2cm, minimum height=2cm] 

\tikzstyle{blockTagFill22} = [top color=rrrred2!30, bottom color=rrrred2!90, draw=rrrred2!70!black!100, node distance=1cm, drop shadow]
\tikzstyle{blockTag22} = [ellipse, draw=rrrred2!90, blockTagFill22, minimum width=3cm, minimum height=4cm] 
\tikzstyle{link} = [>=triangle 60, draw=gray, thick,fill=gray]

\tikzstyle{vecArrow} = [thick,LineBlue, decoration={markings,mark=at position
   1 with {\arrow[thick,fill=rrrblue,draw=rrrblue]{triangle 60}}},
%   double distance=1.8pt, shorten >= 5.5pt,
	LineBlue,
   preaction = {decorate,LineBlue},
   postaction = {draw=rrrblue,line width=1.4pt, LineBlue,shorten >= 4.5pt}]
 
\tikzstyle{vecDoubleArrow} = [LineBlue, decoration={markings,mark=at position
   0 with {\arrow[thick,fill=rrrblue,draw=rrrblue,rotate=180]{triangle 60}},mark=at position
   1 with {\arrow[thick,fill=rrrblue,draw=rrrblue]{triangle 60}}},
   LineBlue,
   preaction = {decorate,LineBlue},
   postaction = {draw=rrrblue,line width=1.4pt, LineBlue,shorten >= 4.5pt}]    
\tikzstyle{innerWhite} = [semithick, white,line width=1.8pt, shorten >= 4.5pt]
\tikzstyle{innerBlue} = [semithick, LineBlue,line width=1.8pt, shorten >= 4.5pt]

\tikzset{
%    mynode/.style={rectangle,rounded corners,draw=rrrblue,fill=rrrblue, top color=white, bottom color=yellow!50,very thick, inner sep=1em, minimum size=3em, text centered},
    myarrow/.style={<->, >=latex', shorten >=1.5pt, thick,line width=1pt,}%,
%    mylabel/.style={text width=7em, text centered,draw=rrrblue} 
}
%**********************************************************************************
\usepackage{afterpage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




